Alternating minimization for generalized rank one matrix sensing: Sharp predictions from a random initialization

We consider the problem of estimating the factors of a rank-$1$ matrix with i.i.d. Gaussian, rank-$1$ measurements that are nonlinearly transformed and corrupted by noise. Considering two prototypical choices for the nonlinearity, we study the convergence properties of a natural alternating update rule for this nonconvex optimization problem starting from a random initialization. We show sharp convergence guarantees for a sample-split version of the algorithm by deriving a deterministic recursion that is accurate even in high-dimensional problems. Notably, while the infinite-sample population update is uninformative and suggests exact recovery in a single step, the algorithm -- and our deterministic prediction -- converges geometrically fast from a random initialization. Our sharp, non-asymptotic analysis also exposes several other fine-grained properties of this problem, including how the nonlinearity and noise level affect convergence behavior. On a technical level, our results are enabled by showing that the empirical error recursion can be predicted by our deterministic sequence within fluctuations of the order $n^{-1/2}$ when each iteration is run with $n$ observations. Our technique leverages leave-one-out tools originating in the literature on high-dimensional $M$-estimation and provides an avenue for sharply analyzing higher-order iterative algorithms from a random initialization in other high-dimensional optimization problems with random data.

==> Proof-of-convergence-results.tex <==
\section{Auxiliary proofs for convergence results}\label{sec:aux-convergence}
In this section, we provide the proofs of Lemmas~\ref{lem:initialization},~\ref{lemma2-good-region}, and~\ref{lem:h-sgn-properties}.

\subsection{Proof of Lemma~\ref{lem:initialization}}\label{sec:proof-lem-initialization}
We prove the lemma for the linear model and nonlinear model in turn.  For both cases, we first bound the deviation of $\parcompZ_{t+1}$ and $\perpcompZ_{t+1}$ from their deterministic counterparts and use these to then bound the deviation of $\parcompX_{t+1}$ and $\perpcompX_{t+1}$ from their deterministic counterparts.  Throughout, we will use the notation 
\begin{align}
	\label{eq:notation-lem-initialization}
	\rho = \frac{C(\oversamp)}{1+\sigma^{2}}, \quad r_{t} = \frac{\perpcompX_{t}}{\parcompX_{t}}, \quad \Delta_{1} = \sqrt{\frac{\log d}{\oversamp \cdot d}}, \quad \text{ and } \quad\Delta_{2} = \frac{\log^{2}(d)}{\oversamp \cdot \sqrt{d}},
\end{align}
\kaccomment{Add a unified proof sketch?}

\subsubsection{Linear observation model}
Recall the functions $\parmapid$~\eqref{eq:parmapid} and $\perpmapid$~\eqref{eq:perpmapid} and note that by definition
\[
\parcompdetZ_{t+1} = \parmapid(\parcompX_{t}, \perpcompX_{t}) = \frac{\parcompX_{t}}{\parcompX_{t}^{2} + \perpcompX_{t}^{2}} \quad \text{ and } \quad (\perpcompdetZ_{t+1})^2 = \perpmapid(\parcompX_{t}, \perpcompX_{t}) = \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{\perpcompX_{t}^{2}}{(\parcompX_{t}^{2} + \perpcompX_{t}^{2})^{2}} + \frac{\sigma^{2}}{C(\oversamp)} \cdot  \frac{\parcompX_{t}^{2}}{(\parcompX_{t}^{2} + \perpcompX_{t}^{2})^{2}}
\]
Straightforward computation yields the pair of sandwich inequalities 
\begin{align}\label{ineq1-lemma1-initia-linear-proof}
	(1-1/r_{t}^{2}) \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} \leq \parcompZ_{t+1}^{\mathsf{det}} \leq \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} \quad \text{and} \quad 
	\rho^{-1} \cdot  \perpcompX_{t}^{-2} \cdot (1+1/r_{t}^{2})^{-2} \leq (\perpcompZ_{t+1}^{\mathsf{det}})^{2} \leq \rho^{-1} \cdot  \perpcompX_{t}^{-2}.
\end{align}
On event $\mathcal{A}_{t+1}$ and using $\parcompX_{t}^{2} + \perpcompX_{t}^{2} \geq 0.5$, we obtain that
Since by assumption, $\parcompX_{t}^{2} + \perpcompX_{t}^{2} \geq 0.5$, we note the following pair of inequalities, which hold on event $\mathcal{A}_{t+1}$
\begin{align}\label{ineq2-lemma1-initia-linear-proof}
	\bigl\lvert \parcompZ_{t+1} - \parcompZ_{t+1}^{\mathsf{det}} \bigr\rvert \leq C_{1} \cdot \Delta_{1} \quad \text{and} \quad \bigl \lvert \perpcompZ_{t+1}^{2} - (\perpcompZ_{t+1}^{\mathsf{det}})^{2} \bigr\rvert \leq C_{1} \cdot \Delta_{2}.
	\end{align}
We turn now to bounding $\parcompX_{t+1}$ and $\perpcompX_{t+1}$.  Combining inequalities~\eqref{ineq1-lemma1-initia-linear-proof} and~\eqref{ineq2-lemma1-initia-linear-proof} with the numeric inequality $(a + b)^2 \leq 2a^2 + 2b^2$ yields the upper bound
\begin{subequations}
	\label{ineq3-lemma1-initia-linear-proof}
	\begin{align}\label{ineq:ineq3-initia-linear-ub}
		\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2} &\leq 2\parcompX_{t}^{2}\perpcompX_{t}^{-4}  + 2C_{1}^{2}\Delta_{1}^{2} + \rho^{-1} \cdot  \perpcompX_{t}^{-2}  + C_{1}\Delta_{2}\nonumber\\
		 &\leq 
		\perpcompX_{t}^{-2} \cdot (\rho^{-1} + 2/r_{t}^{2}) + 2C_{1}^{2}\Delta_{1}^{2} + C_{1}\Delta_{2}.
	\end{align}
We similarly obtain the lower bound
\begin{align}\label{ineq:ineq3-initia-linear-lb}
		\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2} \geq \perpcompX_{t}^{-2} \cdot \rho^{-1} \cdot 1/(1+1/r_{t}^{2})^{2} - C_{1}\Delta_{2}.
\end{align}
\end{subequations}
Again, by definition of the maps $\parmapid$ and $\perpmapid$, 
\begin{align}\label{eq1-lemma1-initia-linear-proof}
	\parcompX_{t+1}^{\mathsf{det}} = \frac{\parcompZ_{t+1}}{\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2}}\quad \text{and} \quad (\perpcompX_{t+1}^{\mathsf{det}})^{2} = \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{\perpcompZ_{t+1}^{2}}{(\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2})^{2}} + \frac{\sigma^{2}}{C(\oversamp)} \cdot  \frac{\parcompZ_{t+1}^{2}}{(\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2})^{2}}.
\end{align}
Combining the lower bound on $\parcompX_{t+1}$~\eqref{ineq1-lemma1-initia-linear-proof}, the deviation inequality~\eqref{ineq2-lemma1-initia-linear-proof} and the upper bound~\eqref{ineq:ineq3-initia-linear-ub} yields the lower bound 
\[
\parcompX_{t+1}^{\mathsf{det}} \geq \frac{\parcompX_{t}\perpcompX_{t}^{-2}(1-r_{t}^{-2}) - C_{1}\Delta_{1}}{\perpcompX_{t}^{-2} \cdot (\rho^{-1} + 2/r_{t}^{2}) + 2C_{1}^{2}\Delta_{1}^{2} + C_{1}\Delta_{2}} = \frac{\parcompX_{t}(1-r_{t}^{-2}) - C_{1}\Delta_{1}\perpcompX_{t}^{2}}{(\rho^{-1} + 2/r_{t}^{2}) + \perpcompX_{t}^{2} \cdot (2C_{1}^{2}\Delta_{1}^{2} + C_{1}\Delta_{2})}.
\]
Further, note that by assumption, $\parcompX_{t} \geq 1/(50\sqrt{d}), \perpcompX_{t}^2 \leq 2, r_t^2 \geq 20\rho$ and $\oversamp \geq C_0 \log{d}$ yields the pair of inequalities
\[
\parcompX_{t} (1 - r_t^{-2}) - C_1 \Delta_1 \perpcompX_{t}^2 \geq \parcompX_{t}/2 \quad \text{ and } \quad (\rho^{-1} + 2/r_{t}^{2}) + \perpcompX_{t}^{2} \cdot (2C_{1}^{2}\Delta_{1}^{2} + C_{1}^{2}\Delta_{2}) \leq 2\rho^{-1}.
\]
Combining the previous three displays yields the lower bound $\parcompdetX_{t+1} \geq \rho/4 \cdot \parcompX_{t}$.  Similarly, we combine the inequalities~\eqref{ineq1-lemma1-initia-linear-proof},~\eqref{ineq2-lemma1-initia-linear-proof} and~\eqref{ineq:ineq3-initia-linear-lb} yields the upper bound 
\[
\parcompX_{t+1}^{\mathsf{det}} \leq \frac{\parcompX_{t} \perpcompX_{t}^{-2} + C_{1} \Delta_{1}}{ \rho^{-1} \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-2} - C_{1}\Delta_{2}} = 
\frac{\parcompX_{t} + C_{1}\Delta_{1}\perpcompX_{t}^{2} }{ \rho^{-1} \cdot (1+r_{t}^{-2})^{-2} - C_{1}\Delta_{2}\perpcompX_{t}^{2}}.
\]
Again, combining the assumptions yields the pair of inequalities 
\[
\parcompX_{t} + C_{1}\Delta_{1}\perpcompX_{t}^{2} \leq 2 \parcompX_{t} \quad \text{ and } \quad \rho^{-1} \cdot (1+r_{t}^{-2})^{-2} - C_{1}\Delta_{2}\perpcompX_{t}^{2} \geq 0.5 \cdot \rho^{-1},
\]
whence we obtain the inequality $\parcompdetX_{t+1} \leq 4\rho \cdot \parcompX_{t}$.  Taking stock, we have shown the sandwich relation
\begin{align}\label{ineq4-lemma1-initia-linear-proof}
	\frac{\rho}{4} \cdot \parcompX_{t} \leq \parcompX_{t+1}^{\mathsf{det}} \leq 4\rho \cdot \parcompX_{t}.
\end{align}
Towards bounding $\perpcompdetX_{t+1}$, we introduce the parallel notation $\widetilde{r}_{t+1} = \perpcompZ_{t+1}/\parcompZ_{t+1}$.  Similarly to the second inequality~\eqref{ineq1-lemma1-initia-linear-proof}, we note the inequality 
\[
\rho^{-1} \cdot \perpcompZ_{t+1}^{-2} \cdot (1+\widetilde{r}_{t+1}^{-2})^{-2} \leq (\perpcompX_{t+1}^{\mathsf{det}})^{2} \leq \rho^{-1} \cdot \perpcompZ_{t+1}^{-2}.
\]
Combining the inequalities~\eqref{ineq1-lemma1-initia-linear-proof} and~\eqref{ineq2-lemma1-initia-linear-proof} with the above display and the numeric inequalities $(1 + a)^{-1} \geq 1 - a$ and $(1 + a)^{-2} \geq 1 - 2a$, for $a > 0$ yields the lower bound 
\begin{align}\label{ineq:linear-perpdet-lb}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} \geq \rho^{-1} \cdot \perpcompZ_{t+1}^{-2} \cdot (1+\widetilde{r}_{t+1}^{-2})^{-2} &\geq
	\perpcompX_{t}^{2} \cdot (1+C_{1}\Delta_{2} \cdot \rho \cdot \perpcompX_{t}^{2})^{-1} \cdot (1+\widetilde{r}_{t+1}^{-2})^{-2} \\&\geq
	\perpcompX_{t}^{2} \cdot (1-C_{1}\Delta_{2} \cdot \rho \cdot \perpcompX_{t}^{2}) \cdot (1-2\widetilde{r}_{t+1}^{-2}).
\end{align} 
Towards bounding $\widetilde{r}_{t+1}$, note the pair of inequalities 
\[
\perpcompZ_{t+1}^{2} \geq \rho^{-1}\perpcompX_{t}^{-2}(1+r_{t}^{-2})^{2} - C_{1}\Delta_{2} \geq 0.5 \rho^{-1} \perpcompX_{t}^{-2} \quad \text{ and } \quad \parcompZ_{t+1}^{2} \leq 2\parcompX_{t}^{2}\perpcompX_{t}^{-4}+2C_{1}^{2}\Delta_{1}^{2}\leq 3\parcompX_{t}^{2}\perpcompX_{t}^{-4},
\]
whence we deduce the lower bound $\widetilde{r}_{t+1}^{2} \geq (6\rho)^{-1}r_{t}^{2}$.  Putting the pieces together, we obtain the lower bound
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} \geq \perpcompX_{t}^{2} \cdot (1-2C_{1}\Delta_{2} \cdot \rho) \cdot (1-12\rho r_{t}^{-2}) &\geq \perpcompX_{t}^{2} \cdot (1-2C_{1}\Delta_{2}\rho -12 \rho r_{t}^{-2})\\
	&\geq \perpcompX_{t}^{2} - 12\rho \parcompX_{t}^{2}-C_{1}'\frac{\log^{2}(d)}{\sqrt{d}},
\end{align*}
where the first inequality follows by combining the inequality~\eqref{ineq:linear-perpdet-lb} with the lower bound $\perpcompX_{t}^2 \geq 0.5$, and the last inequality follows for some universal constant $C_1'$ since $\oversamp \asymp C(\oversamp)$.  Similarly, we upper bound $\perpcompdetX_{t+1}$ as
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} \leq \rho^{-1} \cdot \perpcompZ_{t+1}^{-2} \leq \rho^{-1} \cdot (\rho^{-1}\perpcompX_{t}^{-2}(1+r_{t}^{-2})^{-2} - C_{1}\Delta_{2})^{-1} &=
	\frac{\perpcompX_{t}^{2} \cdot (1+r_{t}^{-2})^{2}}{1-C_{1}\rho \Delta_{2} \perpcompX_{t}^{2} (1+r_{t}^{-2})^{2}}.
\end{align*}
We further upper bound the RHS 
\begin{align*}
\frac{\perpcompX_{t}^{2} \cdot (1+r_{t}^{-2})^{2}}{1-C_{1}\rho \Delta_{2} \perpcompX_{t}^{2} (1+r_{t}^{-2})^{2}} &\leq
\perpcompX_{t}^{2} \cdot (1+r_{t}^{-2})^{2} \cdot \bigl(1+2C_{1}\rho \Delta_{2} \perpcompX_{t}^{2} (1+r_{t}^{-2})^{2}\bigr) \\
&\leq \perpcompX_{t}^2 (1+r_{t}^{-2})^{2} \Bigl(1 + \frac{C_1' \log^2(d)}{\sqrt{d}}\Bigr),
\end{align*}
where the first inequality follows from the numeric inequality $(1-a)^{-1} \leq 1+2a$ for $0\leq a \leq 0.5$, with $a = C_{1}\rho \Delta_{2} \perpcompX_{t}^{2} (1+r_{t}^{-2})^{2} \leq 0.5$ and the final inequality follows by using the assumptions $r_t^2 \geq 20\rho$ and $\perpcompX_t^2 \leq 2$.  Now, since $r_t > 1$, $(1 + r_t^{-2})^2 \leq 1 + 3r_t^{-2}$, 
\[
(1+r_{t}^{-2})^{2} \Bigl(1 + \frac{C_1' \log^2(d)}{\sqrt{d}}\Bigr) \leq 1 + 3r_t^{-2}  + \frac{C \log^2(d)}{\sqrt{d}},
\]
whence we immediately obtain the upper bound
\[
(\perpcompX_{t+1}^{\mathsf{det}})^{2} \leq \perpcompX_{t}^{2} \cdot (1+3r_{t}^{-2}+\frac{C_{1}''\log^{2}(d)}{\sqrt{d}}) \leq \perpcompX_{t}^{2} + 3\parcompX_{t}^{2} + \frac{2C_{1}''\log^{2}(d)}{\sqrt{d}}.
\]
Summarizing, we have obtained the sandwich inequality
\begin{align}\label{ineq5-lemma1-initia-linear-proof}
	\perpcompX_{t}^{2} - 12\rho \parcompX_{t}^{2}-C_{1}'\frac{\log^{2}(d)}{\sqrt{d}} \leq (\perpcompX_{t+1}^{\mathsf{det}})^{2} \leq \perpcompX_{t}^{2} + 3\parcompX_{t}^{2} + \frac{2C_{1}''\log^{2}(d)}{\sqrt{d}}.
\end{align}
Next, we use the inequality
\[
\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2} \geq \perpcompX_{t}^{-2} \cdot \rho^{-1} \cdot (1+1/r_{t}^{2})^{-2} - C_{1}\Delta_{2} \geq \rho^{-1}/4,
\]
in conjunction with the definition of event $\mathcal{B}_{t+1}$ to obtain the pair of deviation bounds
\begin{align*}
	\bigl\lvert \parcompX_{t+1} - \parcompX_{t+1}^{\mathsf{det}} \bigr\rvert  \leq \frac{C_{1} \Delta_1}{\bigl( \parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2} \bigr)^{1/2}} \leq \frac{C_{1}'\log d}{\sqrt{d}} \quad \text{ and }\quad \bigl\lvert \perpcompX_{t+1}^{2}  - (\perpcompX_{t+1}^{\mathsf{det}})^{2} \bigr\rvert \leq \frac{C_{1} \Delta_2}{\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2}}  \leq \frac{C_{1}'\log^{2}(d)}{\sqrt{d}}.
\end{align*}
Combining this with the inequalities~\eqref{ineq4-lemma1-initia-linear-proof} and~\eqref{ineq5-lemma1-initia-linear-proof} yields the desired result.  \qed

\subsubsection{One-bit observation model}
We first obtain a sandwich relation on $\parcompdetZ_{t+1}$.  Using the functions $\parmapbit$~\eqref{eq:parmapbit} in conjunction with the inequality $\phi(x) = \int_{0}^{x} e^{-t^2/2}\mathrm{d}t \leq x$ yields the upper bound
\[
\parcompdetZ_{t+1} = \parmapbit(\parcompX_{t}, \perpcompX_{t}) \leq \frac{1}{2\pi} \cdot \frac{1}{\sqrt{\parcompX_{t}^2 + \perpcompX_{t}^2}} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}} \leq \frac{2}{\pi} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^2}.
\]
Next, applying Lemma~\ref{f-h-properties-nonlinear}(b) in conjunction with the upper bound $\parcompX_{t} /\perpcompX_{t} \leq 1$ yields the lower bound 
\[
\parcompZ_{t+1}^{\mathsf{det}} \geq \frac{1}{\sqrt{2\pi}} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}} \cdot \frac{1}{\sqrt{\parcompX_{t}^{2} + \perpcompX_{t}^{2}}} = \frac{1}{\sqrt{2\pi}} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} \cdot \frac{1}{(1 + r_{t}^{-2})^{1/2}}.
\]
We next find upper and lower bounds on $(\perpcompdetZ_{t+1})^2 = \perpmapbit(\parcompX_{t}, \perpcompX_{t})$~\eqref{eq:perpmapbit}.  To this end, we note that 
\[
\frac{C_3(\oversamp)}{C_2(\oversamp)} \leq \EE\{W^{4}\} \bigg/ \EE\left\{ \frac{W^{2}}{(1 + W^{2})^{2}}\right\} \leq 20,
\]
where $W \sim \mathsf{N}(0, 1)$.  Straightforward computation thus yields the upper bound
\begin{align*}
	(\perpcompZ_{t+1}^{\mathsf{det}})^{2} \leq \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} + \frac{20(\parcompZ_{t+1}^{\mathsf{det}})^{2}}{C(\oversamp)} &\leq 
	\frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} + \frac{20}{C(\oversamp)} \cdot \frac{4}{\pi^{2}} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}}\cdot \frac{\parcompX_{t}^{2}}{\perpcompX_{t}^{2}} \\&\leq \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} \cdot (1+9r_{t}^{-2}),
\end{align*}
where in the penultimate inequality we have also used the upper bound on $\parcompdetZ_{t+1}$.  We additionally obtain the lower bound
\begin{align*}
	(\perpcompZ_{t+1}^{\mathsf{det}})^{2} \geq  \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} - \frac{4}{\pi} \cdot \frac{\parcompZ_{t+1}^{\mathsf{det}}}{C(\oversamp)\sqrt{\parcompX_{t}^{2} + \perpcompX_{t}^{2}}} \cdot 20 &\geq \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} - \frac{160}{\pi^{2}C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2} + \perpcompX_{t}^{2}} \cdot \frac{\parcompX_{t}^{2}}{\perpcompX_{t}^{2}} \\&\geq\frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} \cdot (1-18r_{t}^{-2}),
\end{align*}
where to obtain the first inequality, we have used 
\[
\EE\biggl\{ \frac{|W|^{3}  \phi(\frac{\parcompX_t}{\perpcompX_t} |W|)}{C_{2}(\oversamp) (C(\oversamp) + W^{2})^{2}} \biggr\} \leq \frac{\parcompX_{t}}{\perpcompX_{t}}\frac{C_3(\oversamp)}{C_2(\oversamp)} \leq 20,
\]
which holds since $\parcompX_{t}/\perpcompX_{t} \leq 1$.  We obtain upper and lower bounds on $\parcompZ_{t+1}$ and $\perpcompZ_{t+1}$ since, on $\mathcal{A}_{t+1}$, 
\begin{align}\label{ineq2-lemma1-init-nonlinear-proof}
	\bigl\lvert \parcompZ_{t+1} - \parcompZ_{t+1}^{\mathsf{det}}\bigr\rvert \leq C_{1}\Delta_{1} \quad \text{and} \quad \bigl \lvert  \perpcompZ_{t+1}^{2} - (\perpcompZ_{t+1}^{\mathsf{det}})^{2} \bigr \rvert \leq C_{1}\Delta_{2},
\end{align}
where we have additionally used the fact that $\parcompX_{t}^{2} + \perpcompX_{t}^{2} \geq 0.5$.  With the bounds on $\parcompZ_{t+1}$ and $\perpcompZ_{t+1}$ in hand, we turn to bounding $\parcompX_{t+1}$ and $\perpcompX_{t+1}$.  We first note the upper bound
\[
\parcompdetX_{t+1} = \parmapbit(\parcompZ_{t+1}, \perpcompZ_{t+1}) \leq \frac{2}{\pi} \cdot \frac{1}{\sqrt{\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2}}} \cdot \frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}} \leq \frac{2}{\pi} \cdot \frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}^{2}}.
\]
Using inequalities~\eqref{ineq1-lemma1-init-nonlinear-proof} and~\eqref{ineq2-lemma1-init-nonlinear-proof} in conjunction with the assumptions $\parcompX_{t} \geq 1/(50\sqrt{d})$, $\perpcompX_{t}^{2}\leq2$, $\Delta_{1} \asymp \sqrt{\log d}/\sqrt{\oversamp \cdot d}$, $\oversamp \geq C\log d$, $r_{t}^{2} \geq 50 \rho$, $\rho \asymp \oversamp$, and $\Delta_2 \asymp \log^{2}(d)/(\oversamp \cdot \sqrt{d})$, we obtain the pair of inequalities
\begin{align}\label{ineq3-lemma1-init-nonlinear-proof}
	\parcompZ_{t+1} &\leq \frac{2}{\pi} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} + C_{1}\cdot \Delta_{1} \leq \frac{3}{\pi} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} \quad \text{ and }\quad \nonumber\\
		\perpcompZ_{t+1}^{2} &\geq \rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-1} \cdot (1-18r_{t}^{-2}) - C_{1}\Delta_{2} \geq 0.5\cdot \rho^{-1}\cdot \perpcompX_{t}^{-2}.
\end{align}
Putting the pieces together yields the upper bound 
\[
\parcompX_{t+1}^{\mathsf{det}} \leq \frac{2}{\pi} \cdot \frac{\frac{3}{\pi} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}}}{0.5\cdot \rho^{-1}\cdot \perpcompX_{t}^{-2}} \leq 2\rho \cdot \parcompX_{t}.
\]
We next derive the lower bound of $\parcompX_{t+1}^{\mathsf{det}}$. Using the parallel notation $\widetilde{r}_{t+1} = \parcompZ_{t+1}/\perpcompZ_{t+1}$ and applying inequality~\eqref{ineq3-lemma1-init-nonlinear-proof} yields the lower bound
\[
\widetilde{r}_{t+1} \geq \frac{\left(0.5\cdot \rho^{-1}\cdot \perpcompX_{t}^{-2}\right)^{1/2}}{\frac{3}{\pi} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}}} \geq \frac{\pi}{6} \cdot \rho^{-1/2} \cdot r_{t}.
\]
Since $r_{t}\geq \sqrt{20\rho}$ by assumption, we conclude that $\widetilde{r}_{t+1} \geq 1$.  Next, we apply Lemma~\ref{f-h-properties-nonlinear}(b) in conjunction with the fact that $\frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}} = 1/\widetilde{r}_{t+1} \leq 1$ to obtain the lower bound
\begin{align}\label{ineq3.5-lemma1-init-nonlinear-proof}
	\parcompX_{t+1}^{\mathsf{det}} \geq \frac{1}{\sqrt{2\pi}}\cdot \frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}} \cdot \frac{1}{(\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2})^{1/2}} = \frac{1}{\sqrt{2\pi}}\cdot \frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}^{2}} \cdot \frac{1}{(1+\widetilde{r}_{t+1}^{-2})^{1/2}} \geq \frac{1}{2\sqrt{\pi}} \cdot \frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}^{2}}.
\end{align}
Once more applying inequalities~\eqref{ineq1-lemma1-init-nonlinear-proof} and~\eqref{ineq2-lemma1-init-nonlinear-proof} in conjunction with the assumptions $\parcompX_{t} \geq 1/(50\sqrt{d})$, $\perpcompX_{t}^{2}\leq2$, $\Delta_{1} \asymp \sqrt{\log d}/\sqrt{\oversamp \cdot d}$, $\oversamp \geq C\log d$, $r_{t}^{2} \geq 50 \rho$, $\rho \asymp \oversamp$ and $\Delta_2 \asymp \log^{2}(d)/(\oversamp \cdot \sqrt{d})$ yields
\begin{align}\label{ineq4-lemma1-init-nonlinear-proof}
	\parcompZ_{t+1} &\geq \frac{1}{\sqrt{2\pi}} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} \cdot \frac{1}{(1 + r_{t}^{-2})^{1/2}} - C_{1}\Delta_{1} \geq \frac{1}{4\sqrt{\pi}} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}}\quad \text{and} \nonumber\\
	\perpcompZ_{t+1}^{2} &\leq \rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-1} \cdot (1+9r_{t}^{-2}) + C_{1}\Delta_{2} \leq2\rho^{-1} \cdot \perpcompX_{t}^{-2}.
\end{align}
Putting the pieces together yields the lower bound
\[
\parcompX_{t+1}^{\mathsf{det}} \geq \frac{1}{2\sqrt{\pi}} \cdot \frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}^{2}} \geq \frac{1}{2\sqrt{\pi}} \cdot \frac{ \frac{1}{4\sqrt{\pi}} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} }{ 2\rho^{-1} \cdot \perpcompX_{t}^{-2} } \geq \frac{\rho}{16\pi} \cdot \parcompX_{t}. 
\]
Proceeding to the perpendicular component $\perpcompdetX_{t+1}$, we obtain the inequality 
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} &\leq \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompZ_{t+1}^{2}+\perpcompZ_{t+1}^{2}} \cdot (1+9\widetilde{r}_{t+1}^{-2}) \leq \rho^{-1} \cdot \perpcompZ_{t+1}^{-2}\cdot (1+9\widetilde{r}_{t+1}^{-2}).
\end{align*}
Further, we apply inequalities~\eqref{ineq1-lemma1-init-nonlinear-proof} and~\eqref{ineq2-lemma1-init-nonlinear-proof} to obtain the lower bound
\[
\perpcompZ_{t+1}^{2} \geq \rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-1} \cdot (1-18r_{t}^{-2}) - C_{1}\Delta_{2}.
\]
Putting the two pieces together yields 
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} \leq \frac{1}{\rho}\cdot \frac{ (1+9\widetilde{r}_{t+1}^{-2})}{\rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-1} \cdot (1-18r_{t}^{-2}) - C_{1}\Delta_{2}} &=
	\frac{\perpcompX_{t}^{2}\cdot (1+r_{t}^{-2})\cdot (1-18r_{t}^{-2})^{-1} \cdot (1+9\widetilde{r}_{t+1}^{-2}) }{ 1-C_{1}\cdot \rho \cdot \perpcompX_{t}^{2}\cdot (1+r_{t}^{-2})\cdot (1-18r_{t}^{-2})^{-1} \cdot \Delta_{2}}.
\end{align*}
Further upper bounding the RHS by applying both $\1$ $\perpcompX_{t}^{2}\cdot (1+r_{t}^{-2})\cdot (1-18r_{t}^{-2})^{-1} \leq 10$ since $\perpcompX_{t}^{2} \leq 2$ and $r_{t}^{2} \geq 50\rho$, and $\2$ $(1-a)^{-1} \leq 1+2a$ for $0 \leq a\leq 0.5$ with $a = 10C_{1}\cdot \rho \cdot \Delta_{2} \asymp \log^{2}(d)/\sqrt{d}$ yields the bound 
\begin{align*}
		(\perpcompX_{t+1}^{\mathsf{det}})^{2}	\leq \perpcompX_{t}^{2}\cdot (1+r_{t}^{-2})\cdot (1-18r_{t}^{-2})^{-1} \cdot (1+9\widetilde{r}_{t+1}^{-2}) \cdot (1+20C_{1}\rho\Delta_{2}).
\end{align*}
Note that $\widetilde{r}_{t+1} \geq \frac{\pi}{6} \cdot \rho^{-1/2} \cdot r_{t}$, whence we deduce the inequality
\begin{align*}
	(1+r_{t}^{-2})\cdot (1-18r_{t}^{-2})^{-1} \cdot (1+9\widetilde{r}_{t+1}^{-2}) \leq (1+r_{t}^{-2})\cdot(1+36r_{t}^{-2})\cdot(1+36\rho r_{t}^{-2}) \leq 1+40\rho r_{t}^{-2}.
\end{align*}
Combining the previous two displays yields the upper bound
\[
(\perpcompX_{t+1}^{\mathsf{det}})^{2} \leq \perpcompX_{t}^{2} \cdot (1+40\rho r_{t}^{-2}) \cdot (1+20C_{1}\rho\Delta_{2}) \leq \perpcompX_{t}^{2} + 40\rho\parcompX_{t}^{2} + \frac{C_{1}'\log^{2}(d)}{\sqrt{d}}.
\]
Next we derive the lower bound of $(\perpcompX_{t+1}^{\mathsf{det}})^{2}$. We obtain that
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} &\geq \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompZ_{t+1}^{2}+\perpcompZ_{t+1}^{2}} - \frac{160}{\pi^{2}C(\oversamp)} \cdot \frac{1}{\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2}} \cdot \frac{\parcompZ_{t+1}^{2}}{\perpcompZ_{t+1}^{2}} \\&\geq \rho^{-1} \cdot \perpcompZ_{t+1}^{-2} \cdot (1+\widetilde{r}_{t+1}^{-2})^{-1} \cdot (1-18\widetilde{r}_{t+1}^{-2}),
\end{align*}
Applying inequalities~\eqref{ineq1-lemma1-init-nonlinear-proof} and~\eqref{ineq2-lemma1-init-nonlinear-proof} yields 
\[
\perpcompZ_{t+1}^{2} \leq \rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-1} \cdot (1+9r_{t}^{-2}) + C_{1}\Delta_{2} \leq \rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+9r_{t}^{-2}) + C_{1}\Delta_{2} .
\]
Putting the two pieces together yields 
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} &\geq \frac{1}{\rho} \cdot \frac{(1+\widetilde{r}_{t+1}^{-2})^{-1} \cdot (1-18\widetilde{r}_{t+1}^{-2})}{\rho^{-1} \cdot \perpcompX_{t}^{-2}  \cdot (1+9r_{t}^{-2}) + C_{1}\Delta_{2}} &= \frac{\perpcompX_{t}^{2}\cdot(1+9r_{t}^{-2})^{-1}\cdot(1+\widetilde{r}_{t+1}^{-2})^{-1} \cdot (1-18\widetilde{r}_{t+1}^{-2})}{1 + C_{1}\perpcompX_{t}^{2}(1+9r_{t}^{-2})^{-1}\rho\Delta_{2}}.,
\end{align*}
Using $\1$ $\perpcompX_{t}^{2}(1+9r_{t}^{-2})^{-1} \leq 10$ since $\perpcompX_{t}^{2} \leq 2$ and $r_{t}^{2}\geq 20\rho$, and $\2$ $(1+a)^{-1} \geq 1-a$ with $a = 10C_{1}\rho\Delta_{2}$ yields 
\begin{align*}
	(1 + C_{1}\perpcompX_{t}^{2}(1+9r_{t}^{-2})^{-1}\rho\Delta_{2})^{-1} \geq 1 - 10C_{1}\rho\Delta_{2}.
\end{align*}
Continuing, using $\widetilde{r}_{t+1} \geq \frac{\pi}{6} \cdot \rho^{-1/2} \cdot r_{t}$, we obtain that
\[
(1+9r_{t}^{-2})^{-1}\cdot(1+\widetilde{r}_{t+1}^{-2})^{-1} \cdot (1-18\widetilde{r}_{t+1}^{-2}) \geq (1-9r_{t}^{-2})\cdot(1-\widetilde{r}_{t+1}^{-2}) \cdot (1-18\widetilde{r}_{t+1}^{-2}) \geq 1-100\rho\cdot r_{t}^{-2}.
\]
Putting the pieces together, we obtain the lower bound
\[
(\perpcompX_{t+1}^{\mathsf{det}})^{2} \geq \perpcompX_{t}^{2}\cdot (1-100\rho\cdot r_{t}^{-2})\cdot (1 - 10C_{1}\rho\Delta_{2}) \geq \perpcompX_{t}^{2} - 100\rho \cdot \parcompX_{t}^{2} - \frac{C_{1}'\log^{2}(d)}{\sqrt{d}}.
\]
Taking stock, we have shown the pair of sandwich relations
\begin{align}\label{ineq:penultimate-nonlinear-random-init}
	\frac{\rho}{16\pi} \cdot \parcompX_{t} &\leq \parcompX_{t+1}^{\mathsf{det}} \leq 2\rho \cdot \parcompX_{t} \quad \text{ and } \nonumber\\
	\perpcompX_{t}^{2} - 100\rho \cdot \parcompX_{t}^{2} - \frac{C_{1}'\log^{2}(d)}{\sqrt{d}} &\leq (\perpcompX_{t+1}^{\mathsf{det}})^{2} \leq \perpcompX_{t}^{2} + 40\rho\parcompX_{t}^{2} + \frac{C_{1}'\log^{2}(d)}{\sqrt{d}}.
\end{align}
To conclude, we lower bound the sum of squares $\parcompZ_{t+1}^2 + \perpcompZ_{t+1}^2$ as 
\[
\parcompZ_{t+1}^{2}+\perpcompZ_{t+1}^{2} \geq \perpcompZ_{t+1}^{2} \geq \rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-1} \cdot (1-18r_{t}^{-2}) - C_{1}\Delta_{2} \geq \rho^{-1}/4 \gtrsim \oversamp^{-1},
\]
where the last step follows since $\rho \asymp \oversamp$.  Finally, by the above inequality, we note that on event $\mathcal{B}_{t+1}$, 
\begin{align*}
	\bigl\lvert \parcompX_{t+1} - \parcompX_{t+1}^{\mathsf{det}}\bigr\rvert \lesssim \sqrt{\frac{\log d}{d}} \quad \text{and} \quad \bigl\lvert \perpcompX_{t+1}^{2} - (\perpcompX_{t+1}^{\mathsf{det}})^{2} \bigr\rvert \lesssim \frac{\log^{2}(d)}{\sqrt{d}}.
\end{align*}
The conclusion follows immediately upon combining the above display with the pair of inequalities~\eqref{ineq:penultimate-nonlinear-random-init}. \qed

\subsection{Proof of Lemma~\ref{lemma2-good-region}}\label{sec:proof-lemma-good-region}
We require the following lemma, deferring its proof to Section~\ref{sec:proof-help-lemma2-GD}.
\begin{lemma}\label{help-lemma2-GD-linear}
	Let $\parcompX > 0$ and $\perpcompX\geq 0 $ satisfy $\perpcompX/\parcompX \leq 50\sqrt{\rho}$, for $\rho = C(\oversamp)/(1 + \sigma^2)$.  Further, suppose that with $\psi \in \{ \mathsf{id}, \sign \}$ and $(\parcompdetX, \perpcompdetX) = \bigl(F_{\psi}(\parcompX, \perpcompX), G_{\psi}(\parcompX, \perpcompX)\bigr)$, $\parcompX', \perpcompX'$ satisfy
	\[
	\bigl \lvert \parcompX' - \parcompdetX \bigr \rvert \lesssim \frac{1}{\sqrt{\parcompX^2 + \perpcompX^2}} \sqrt{\frac{\log{n}}{n}}, \qquad \text{ and } \qquad \bigl \lvert \perpcompX' - \perpcompdetX \bigr \rvert \lesssim \frac{1}{\parcompX^2 + \perpcompX^2} \frac{\sqrt{d}\log^2{n}}{n}. 
	\]	
	Then, there exists a universal, positive constant $C$ such that for $\oversamp \geq C$, 
	\[
	\biggl \lvert \Bigl(\frac{\perpcompX'}{\parcompX'}\Bigr)^2 - \ratiomappsi\Bigl(\frac{\perpcompX^2}{\parcompX^2}\Bigr)\biggl\lvert \lesssim \Bigl(1 \vee \frac{\perpcompX^2}{\parcompX^2}\Bigr)\cdot \frac{\sqrt{d}\log^2{n}}{n} + \Bigl(1 \vee \frac{\perpcompX}{\parcompX}\Bigr)\cdot \sqrt{\frac{\log{n}}{n}}.
	\]
\end{lemma}

\subsubsection{Proof of Lemma~\ref{lemma2-good-region} for the linear observation model}
We begin by showing $\perpcompZ_{t+1}/\parcompZ_{t+1} \leq 51$.  Note that on the event $\mathcal{A}_{t+1}$, 
\[
\bigl \lvert \parcompZ_{t+1} - \parcompdetZ_{t+1} \bigr \rvert \lesssim \frac{1}{\sqrt{\parcompX_{t}^2 + \perpcompX_{t}^2}} \cdot \sqrt{\frac{\log{n}}{n}} \qquad \text{ and } \qquad\bigl \lvert (\perpcompZ_{t+1})^2 - (\perpcompdetZ_{t+1})^2 \bigr \rvert \lesssim \frac{1}{\parcompX_{t}^2 + \perpcompX_{t}^2} \cdot \frac{\sqrt{d} \log^2{n}}{n}.  
\]
By assumption, $\perpcompX_t/\parcompX_t \leq 50 \sqrt{\rho} \lesssim \sqrt{\oversamp}$, whence we apply Lemma~\ref{help-lemma2-GD-linear} to obtain the bound 
\begin{align}\label{ineq1-lemma2-GD-linear}
	\begin{split}
		\biggl\lvert \Bigl( \frac{\perpcompZ_{t+1}}{\parcompZ_{t+1}} \Bigr)^{2} - \ratiomapid\Bigl( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \biggr \rvert &\lesssim \Bigl(1 \vee \frac{\perpcompX^2}{\parcompX^2}\Bigr)\cdot \frac{\sqrt{d}\log^2{n}}{n} + \Bigl(1 \vee \frac{\perpcompX}{\parcompX}\Bigr)\cdot \sqrt{\frac{\log{n}}{n}} \\&\lesssim \oversamp \cdot \frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\oversamp} \cdot  \sqrt{\frac{\log(n)}{n}}.
	\end{split}
\end{align}
Consequently, 
\begin{align*}
	\Bigl( \frac{\perpcompZ_{t+1}}{\parcompZ_{t+1}} \Bigr)^{2} &\leq \ratiomapid\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} = \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{\sigma^{2}}{C(\oversamp)} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq
	50^{2}+1.
\end{align*}
Equipped with this bound, we turn to bounding $\perpcompX_{t+1}/\parcompX_{t+1}$.  Proceeding in a parallel manner to above, we obtain the inequality
\begin{align}\label{ineq2-lemma2-GD-linear}
	\begin{split}
		\biggl\lvert \Bigl( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \Bigr)^{2} - \ratiomapid\Bigl( \frac{\perpcompZ_{t}^{2}}{\parcompZ_{t}^{2}}\Bigr) \biggr \rvert &\lesssim \Bigl(1 \vee \frac{\perpcompX^2}{\parcompX^2}\Bigr)\cdot \frac{\sqrt{d}\log^2{n}}{n} + \Bigl(1 \vee \frac{\perpcompX}{\parcompX}\Bigr)\cdot \sqrt{\frac{\log{n}}{n}} \\&\lesssim \frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\frac{\log(n)}{n}}.
	\end{split}
\end{align}
We thus decompose and apply the triangle inequality to obtain
\begin{align*}
	\biggl\lvert \Bigl( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \Bigr)^{2} - \ratiomapid \circ \ratiomapid\Bigl( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \biggr\rvert &\leq
	\biggl\lvert \Bigl( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \Bigr)^{2} - \ratiomapid\Bigl( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\Bigr) \biggr\rvert + 
	\biggl\lvert \ratiomapid\Bigl( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\Bigr) - \ratiomapid \circ \ratiomapid\Bigl( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \biggr\rvert \\&\overset{\1}{=}
	\biggl\lvert \Bigl( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \Bigr)^{2} - \ratiomapid\Bigl( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\Bigr) \biggr\rvert + 
	\frac{1+\sigma^{2}}{C(\oversamp)} \cdot \biggl\lvert \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}} -  \ratiomapid\Bigl( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \biggr\rvert \\&\overset{\2}{\lesssim}
	\frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\frac{\log(n)}{n}} + \frac{1}{\oversamp} \cdot \Bigl( \oversamp \cdot \frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\oversamp} \cdot  \sqrt{\frac{\log(n)}{n}} \Bigr) \\&\lesssim
	\frac{\log^{2}(n)}{\sqrt{n}},
\end{align*}
where in step $\1$ we use $\ratiomapid(x) = \frac{1+\sigma^{2}}{C(\oversamp)}\cdot x+\frac{\sigma^{2}}{C(\oversamp)}$ and step $\2$ follows from inequalities~\eqref{ineq1-lemma2-GD-linear} and~\eqref{ineq2-lemma2-GD-linear}.  This completes the proof. \qed


\subsubsection{Proof of Lemma~\ref{lemma2-good-region} for the one-bit observation model}
We first state a lemma which provides some properties on the functions $\parmapbit$, $\perpmapbit$, and $\ratiomapbit$.
\kaccomment{Perhaps put this lemma elsewhere}
\begin{lemma}\label{f-h-properties-nonlinear}
	Consider the functions $\parmapbit$~\eqref{eq:parmapbit}, $\perpmapbit$~\eqref{eq:perpmapbit}, and $\ratiomapbit$~\eqref{eq:ratiomaps}.  The following hold.
	\begin{itemize}
		\item[(a)] There exists a universal positive constant $C_1$ such that
		\[
		\bigl \lvert \ratiomapbit'(x) \bigr \rvert \leq C_1 \cdot \frac{1 + x^{3/2}}{C(\oversamp)} \qquad \text{ as long as } \qquad x > 0.
		\]
		\item[(b)] The function $\parmapbit$ is lower bounded as 
		\[
			\parmapbit(\parcompX,\perpcompX) \geq \frac{1}{\sqrt{2}\pi} \cdot \frac{\min\{\frac{\parcompX}{\perpcompX},1\}}{(\parcompX^{2} + \perpcompX^{2})^{1/2}},\qquad \text{ as long as } \qquad \frac{\parcompX}{\perpcompX} \geq 0.
		\]
	\end{itemize}
\end{lemma}
Equipped with this lemma, we continue to the proof.  We begin by estimating $\perpcompZ_{t+1}/\parcompZ_{t+1}$, noting that the inequality~\eqref{ineq1-lemma2-GD-linear} continues to hold, so that
\begin{align}\label{ineq1-lemma2-GD-nonlinear}
	\biggl\lvert \Bigl( \frac{\perpcompZ_{t+1}}{\parcompZ_{t+1}} \Bigr)^{2} - \ratiomapbit\Bigl( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \biggr \rvert \lesssim \oversamp \cdot \frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\oversamp} \cdot  \sqrt{\frac{\log(n)}{n}}.
\end{align}
Applying Lemma~\ref{lem:h-sgn-properties} yields the upper bound 
\[
\ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \leq \max\left\{ \frac{\pi^{2}}{2} \cdot \frac{1}{\rho} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{20}{C(\oversamp)}, \frac{50\pi^{2}}{\rho} \right\} \leq C,
\]
where in the last step we use $\frac{\perpcompX_{t}}{\parcompX_{t}} \leq 50\sqrt{\rho}$.
Combining the previous two displays, we obtain the inequality
\begin{align*}
	\Bigl( \frac{\perpcompZ_{t+1}}{\parcompZ_{t+1}} \Bigr)^{2} &\leq \ratiomapbit\Bigl( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) + C_{1}\oversamp \cdot \frac{\sqrt{d}\log^{2}(n)}{n} + C_{1}\sqrt{\oversamp} \cdot \sqrt{\frac{\log(n)}{n}} \leq C.
\end{align*}
With this estimate of $\perpcompZ_{t+1}\parcompZ_{t+1}$ in hand, we turn to bounding $\perpcompX_{t+1}/\parcompX_{t+1}$.  Proceeding in a parallel manner to above, we obtain the inequality (cf. inequality~\eqref{ineq2-lemma2-GD-linear})
\begin{align}\label{ineq2-lemma2-GD-nonlinear}
\biggl\lvert \Bigl( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \Bigr)^{2} - \ratiomapbit\Bigl( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\Bigr) \biggr \rvert \lesssim \frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\frac{\log(n)}{n}}.
\end{align}
We next note the upper bound
\begin{align*}
	\biggl \lvert \ratiomapbit\Bigl(\frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\Bigr) - \ratiomapbit \circ \ratiomapbit \Bigl(\frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \biggr \rvert \leq \max_{0 \leq \lambda \leq 1}\; \biggl \lvert \ratiomapbit'\Bigl( \lambda \cdot \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}} + (1 - \lambda) \ratiomapbit\Bigl(\frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \Bigr) \biggr \rvert \cdot \biggl \lvert \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}} - \ratiomapbit\Bigl(\frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \biggr \rvert.
\end{align*}
Applying Lemma~\ref{f-h-properties-nonlinear}(a) in conjunction with the bounds $\perpcompZ_{t+1}^2/\parcompZ_{t+1}^2 \leq C$, $\ratiomapbit(\perpcompX_{t}^2/\parcompX_{t}^2) \leq C$, and $C(\oversamp) \asymp \oversamp$ yields the bound 
\[
\max_{0 \leq \lambda \leq 1}\; \biggl \lvert \ratiomapbit'\Bigl( \lambda \cdot \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}} + (1 - \lambda) \ratiomapbit\Bigl(\frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \Bigr) \biggr \rvert \lesssim \oversamp^{-1},
\]
so that 
\begin{align}\label{ineq:final-local-nonlinear}
\biggl \lvert \ratiomapbit\Bigl(\frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\Bigr) - \ratiomapbit \circ \ratiomapbit \Bigl(\frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \biggr \rvert \lesssim \oversamp^{-1} \biggl \lvert \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}} - \ratiomapbit\Bigl(\frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \biggr \rvert.
\end{align}
To conclude, we decompose and apply the triangle inequality to obtain the inequality 
\begin{align*}
	\biggl\lvert \Bigl( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \Bigr)^{2} - \ratiomapbit \circ \ratiomapbit\Bigl( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \biggr\rvert &\leq
	\biggl\lvert \Bigl( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \Bigr)^{2} - \ratiomapbit\Bigl( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\Bigr) \biggr\rvert + 
	\biggl\lvert \ratiomapbit\Bigl( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\Bigr) - \ratiomapbit \circ \ratiomapbit\Bigl( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \biggr\rvert.
\end{align*}
We conclude by applying the inequalities~\eqref{ineq1-lemma2-GD-nonlinear},~\eqref{ineq2-lemma2-GD-nonlinear}, and~\eqref{ineq:final-local-nonlinear} to the RHS in the display above to obtain the inequality
\[
\biggl\lvert \Bigl( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \Bigr)^{2} - \ratiomapbit \circ \ratiomapbit\Bigl( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\Bigr) \biggr\rvert \lesssim
\frac{\log^{2}(n)}{\sqrt{n}},
\]
which concludes the proof.\qed


\subsubsection{Proof of Lemma~\ref{help-lemma2-GD-linear}}\label{sec:proof-help-lemma2-GD}
We separate the two cases, $\psi(x) = x$ and $\psi(x) = \sign(x)$, proving each part in turn.  

\paragraph{Proof of Lemma~\ref{help-lemma2-GD-linear} with $\psi(x) = x$}
Applying the condition of the lemma and re-arranging yields
\begin{align*}
	\parcompX' \geq 
	\frac{\parcompX}{\parcompX^{2}+\perpcompX^{2}} - \frac{C_{1}}{\sqrt{\parcompX^{2}+\perpcompX^{2}}} \cdot\sqrt{\frac{\log(d)}{\oversamp \cdot d}} &=
	\frac{1}{\sqrt{\parcompX^{2}+\perpcompX^{2}}}\cdot \biggl( \frac{1}{\sqrt{1+\perpcompX^{2}/\parcompX^{2}}} - C_{1}\sqrt{\frac{\log(d)}{\oversamp \cdot d}} \biggr) \\&\geq  \frac{0.5}{\sqrt{\parcompX^{2}+\perpcompX^{2}}}\cdot  \frac{1}{\sqrt{1+\perpcompX^{2}/\parcompX^{2}}},
\end{align*}
where in the final inequality, we have used the assumption $\perpcompX/\parcompX \leq 50\sqrt{\rho} \lesssim \sqrt{\oversamp}$, which in turn implies $(1 + \perpcompX^2/\parcompX^2)^{-1/2} \gtrsim \oversamp^{-1/2}$.  Decomposing and applying the triangle inequality, we obtain
\begin{align}\label{ineq1-help-lemma2-GD-linear}
	\biggl \lvert \Bigl(\frac{\perpcompX'}{\parcompX'} \Bigr)^{2} - \Bigl(\frac{\perpcompdetX}{\parcompdetX} \Bigr)^{2} \biggr \rvert &\leq \frac{\left| (\perpcompX')^{2} - (\perpcompdetX)^{2}\right|}{(\parcompX')^{2}} + 
	\biggl\lvert \Bigl( \frac{\perpcompdetX}{\parcompX'} \Bigr)^{2} -\Bigl( \frac{\perpcompdetX}{\parcompdetX}\Bigr)^{2} \biggr\rvert \nonumber\\
	&= \frac{\left| (\perpcompX')^{2} - (\perpcompdetX)^{2}\right|}{(\parcompX')^{2}} + \Bigl(\frac{\perpcompdetX}{\parcompdetX}\Bigr)^2 \cdot \frac{\bigl \lvert (\parcompX')^2 - (\parcompdetX)^2\bigr \rvert}{(\parcompX')^2} \nonumber\\
	&\leq \frac{\left| (\perpcompX')^{2} - (\perpcompdetX)^{2}\right|}{(\parcompX')^{2}} + \Bigl(\frac{\perpcompdetX}{\parcompdetX}\Bigr)^2 \cdot \biggl[\frac{\bigl (\parcompX' - \parcompdetX\bigr)^2}{(\parcompX')^2} + \frac{2\bigl \lvert \parcompX' - \parcompdetX\bigr \rvert}{\parcompX'}\biggr]
\end{align}
Note that 
\[
\Bigl( \frac{\perpcompdetX}{\parcompdetX} \Bigr)^2 = \ratiomapid\Bigl(\frac{\perpcompX^2}{\parcompX^2}\Bigr) = \frac{1 + \sigma^2}{C(\oversamp)} \frac{\perpcompX^2}{\parcompX^2} + \frac{\sigma^2}{C(\oversamp)} \leq 50^2 + 1,
\]
where the final inequality follows from the assumption $\perpcompX/\parcompX \leq 50\sqrt{\rho}$.  Applying the assumption in conjunction with the lower bound on $\parcompX'$ yields the pair of inequalities
\[
\frac{\lvert (\perpcompX')^2 - (\perpcompdetX)^2 \rvert}{(\parcompX')^2} \lesssim \Bigl(1 \vee \frac{\perpcompX^2}{\parcompX^2} \Bigr) \cdot \frac{\sqrt{d}\log^2{n}}{n} \qquad \text{ and } \qquad \frac{\lvert \parcompX' - \parcompdetX \rvert}{\parcompX'} \lesssim \Bigl(1 \vee \frac{\perpcompX^2}{\parcompX^2} \Bigr) \sqrt{\frac{\log{n}}{n}}.
\]
Putting the pieces together yields the inequality 
\[
\biggl \lvert \Bigl( \frac{\perpcompX'}{\parcompX'} \Bigr)^{2} -\Bigl( \frac{\perpcompdetX}{\parcompdetX}\Bigr)^{2} \biggr\rvert \lesssim \Bigl(1 \vee \frac{\perpcompX^2}{\parcompX^2} \Bigr) \cdot \frac{\sqrt{d}\log^{2}(n)}{n} +  \Bigl(1 \vee \frac{\perpcompX^2}{\parcompX^2} \Bigr)\cdot \sqrt{\frac{\log(n)}{n}}.
\]
The result follows since $(\perpcompdetX)^2/(\parcompdetX)^2 = \ratiomapid(\perpcompX^2/\parcompX^2)$. \qed

\paragraph{Proof of Lemma~\ref{help-lemma2-GD-linear} with $\psi(x) = \sign(x)$}
The architecture of the proof is nearly identical to the previous paragraph, so we restrict ourselves to the differences.  First, we lower bound $\parcompX'$ as
\begin{align*}
	\parcompX' \geq \frac{1}{\pi \sqrt{2}} \cdot \frac{ (\parcompX/\perpcompX)\wedge 1}{\sqrt{\parcompX^2 + \perpcompX^2}} - \frac{C_1}{\sqrt{\parcompX^2 + \perpcompX^2}}\sqrt{\frac{\log(d)}{\oversamp \cdot d}} \geq \frac{1}{\sqrt{\parcompX^2 + \perpcompX^2}} \cdot \frac{(\parcompX/\perpcompX) \wedge 1}{2\pi},
\end{align*}
where in the final inequality we have used the assumption $\perpcompX/\parcompX \leq 50\sqrt{\rho} \lesssim \sqrt{\oversamp}$, whence $\parcompX/\perpcompX \gtrsim \oversamp^{-1/2}$.  We then note the inequality~\eqref{ineq1-help-lemma2-GD-linear}, which continues to hold, and apply Lemma~\ref{lem:h-sgn-properties} to obtain the bound 
\[
\Bigl(\frac{\perpcompdetX}{\parcompdetX}\Bigr)^{2} = \ratiomapbit\Bigl(\frac{\perpcompX^{2}}{\parcompX^{2}}\Bigr) \leq \max\left\{ \frac{\pi^{2}}{2} \cdot \frac{1}{\rho} \cdot \frac{\perpcompX^{2}}{\parcompX^{2}} + \frac{20}{C(\oversamp)}, \frac{50\pi^{2}}{\rho} \right\} \leq C,
\]
where in the last step we use $b/a \leq 50\sqrt{\rho}$.  The conclusion follows using identical steps to the proof of Lemma~\ref{help-lemma2-GD-linear}, with $\psi(x) = x$. \qed

\subsection{Properties of the function $\ratiomapbit$}
This section is dedicated to various properties of the function $\ratiomapbit$.  We first state two lemmas before providing their proofs as well as the proof of Lemma~\ref{lem:h-sgn-properties}.  We first define the functions $h_1: \mathbb{R} \rightarrow \mathbb{R}$ and $h_2: \mathbb{R} \rightarrow \mathbb{R}$ as
\begin{align}\label{eq:def-h1-h2}
	h_1(x) = \oversamp \EE \biggl\{ \frac{\lvert W \rvert \phi(x \lvert W \rvert)}{C(\oversamp) + W^2}\biggr\} \qquad \text{ and } \qquad h_2(x) = C_3(\oversamp)^{-1}\EE\biggl\{\frac{\lvert W \rvert^3 \phi(x\lvert W \rvert)}{(C(\oversamp) + W^2)^2}\biggr\},
\end{align}
where $W \sim \mathsf{N}(0, 1)$, $\phi(x) = \int_{0}^{x} e^{-t^2/2}\mathrm{d}t$, and we recall $C_3(\oversamp)$~\eqref{eq:C2-C3}.  We will make use of the following technical lemma, whose proof we provide in Section~\ref{sec:proof-lemma1-proof-f-h-main-properties}.
\begin{lemma}\label{lemma1-proof-f-h-main-properties} 
	Consider the functions $h_1$ and $h_2$~\eqref{eq:def-h1-h2}.  The following hold. 
	\begin{itemize}
		\item[(a)] There is a universal positive constant $C$ such that for $x > 0$, 
		\[
		\frac{x}{(1 + x^2)^{1.5}} \leq h_1(x) \leq x \vee 5, \qquad \text{ and } \qquad h_2(x) \leq x \vee C.  
		\]
		\item[(b)] For $x > 0$, the derivatives satisfy
		\[
		\frac{1}{(1 + x^2)^{1.5}} \leq h_1'(x) \leq \frac{5}{(1 + x^2)^{1.5}} \qquad \text{ and } \qquad 0 \leq h_2'(x) \leq \frac{30}{(1 + x^2)^{2.5}}.
		\]
	\end{itemize}
\end{lemma}

The next lemma bounds the derivative of $\ratiomapbit$ as well as lower bounds the parallel component of the update.  We provide its proof in Section~\ref{sec:proof-f-h-properties-nonlinear}.  
\begin{lemma}\label{f-h-properties-nonlinear}
	Consider the functions $\parmapbit$~\eqref{eq:parmapbit}, $\perpmapbit$~\eqref{eq:perpmapbit}, and $\ratiomapbit$~\eqref{eq:ratiomaps}.  The following hold.
	\begin{itemize}
		\item[(a)] There exists a universal positive constant $C_1$ such that
		\[
		\bigl \lvert \ratiomapbit'(x) \bigr \rvert \leq C_1 \cdot \frac{1 + x^{3/2}}{C(\oversamp)} \qquad \text{ as long as } \qquad x > 0.
		\]
		\item[(b)] The function $\parmapbit$ is lower bounded as 
		\[
		\parmapbit(\parcompX,\perpcompX) \geq \frac{1}{\sqrt{2}\pi} \cdot \frac{\min\{\frac{\parcompX}{\perpcompX},1\}}{(\parcompX^{2} + \perpcompX^{2})^{1/2}},\qquad \text{ as long as } \qquad \frac{\parcompX}{\perpcompX} \geq 0.
		\]
	\end{itemize}
\end{lemma}
\subsubsection{Proof of Lemma~\ref{lemma1-proof-f-h-main-properties}}\label{sec:proof-lemma1-proof-f-h-main-properties}
Taking derivatives yields
\[
h_1'(x) = \oversamp \EE\biggl\{\frac{W^2 e^{-x^2 W^2/2}}{C(\oversamp + W^2)}\biggr\}, \qquad \text{ and } \qquad h_2'(x) = C_3(\oversamp)^{-1}\EE \biggl\{\frac{W^4 e^{-x^2W^2/2}}{(C(\oversamp) + W^2)^2}\biggr\}.
\]
Note that since $e^{-x^2W^2/2} \leq 1$, both $h_1'(x) \leq 1$ and $h_2'(x) \leq 1$.  Towards lower bounding the derivatives, note that 
\begin{align*}
	\EE_{W\sim\mathcal{N}(0,1)}\left\{ \frac{W^{2} e^{-x^{2}W^{2}/2}}{C(\oversamp) + W^{2}} \right\} = \frac{ \EE_{W\sim\mathcal{N}(0,\frac{1}{1+x^{2}})}\left\{ \frac{W^{2}}{C(\oversamp) + W^{2}} \right\} }{\sqrt{1+x^{2}}}  = \frac{ \EE_{W\sim\mathcal{N}(0,1)}\left\{ \frac{W^{2}}{ C(\oversamp) + \frac{W^{2}}{1+x^{2}}} \right\} }{(1+x^{2})^{1.5}}.
\end{align*}
Similarly, 
\[
\EE\left\{ \frac{W^{4}  e^{-x^{2}W^{2}/2}}{(C(\oversamp) + W^{2})^{2}} \right\} = (1+x^{2})^{-2.5}\EE \left\{ \frac{W^{4}}{ (C(\oversamp) + W^{2}/(1+x^{2}) )^{2}} \right\},
\]
whence the derivatives admit the equivalent representations
\begin{align}\label{h1'-h2'}
	h_{1}'(x) = \frac{ \EE\bigl\{ \frac{W^{2}}{ C(\oversamp) + W^{2}/(1+x^{2}) } \bigr\} }{(1+x^{2})^{1.5} \cdot \EE\bigl\{ \frac{W^{2}}{C(\oversamp) + W^{2}}\bigr\} } \qquad \text{ and }\qquad h_{2}'(x) = \frac{ \EE\bigl\{ \frac{W^{4}}{ ( C(\oversamp) + W^{2}/(1+x^{2}))^{2} } \bigr\} }{(1+x^{2})^{2.5} \cdot \EE\bigl\{ \frac{W^{4}}{(C(\oversamp) + W^{2} )^{2}}\bigr\} }.
\end{align}
We thus deduce that $h_1'(x) \geq (1 + x^2)^{-1.5}$ for positive $x$.  Applying the upper and lower bounds on $h_1'(x)$ in conjunction with the fact that $h_1(0) = 0$, we obtain the sandwich relation
\[
\frac{x}{(1 + x^2)^{1.5}} \leq h_1(x) = \int_{0}^{x}h_1'(t) \mathrm{d}t \leq x.
\]
In a similar manner, since $h_2'(x) \leq 1$ and $h_2(0) = 0$, we deduce that $h_2(x) \leq x$ for positive $x$.  Now, using the inequality $\int_{0}^{x \lvert W \rvert} e^{-t^2/2} \mathrm{d}t \leq \sqrt{\pi/2}$ for positive $x$, we obtain the upper bounds
\begin{align*}
	h_1(x) &\leq \oversamp \sqrt{\pi/2} \EE\left\{ \frac{|W|}{C(\oversamp) + W^{2}} \right\} \leq \sqrt{\pi/2} \cdot \EE\{|W|\}\cdot \EE\left\{ \frac{W^{2}}{1 + W^{2}}\right\}^{-1} \leq 5, \qquad \text{ and }\\
	h_2(x) &\leq C_3(\oversamp)^{-1} \sqrt{\pi/2} \EE\left\{ \frac{|W|^{3}}{(C(\oversamp) + W^{2})^{2}} \right\}\leq \sqrt{\pi/2} \cdot \EE\{|W|^{3}\}\cdot \EE\left\{ \frac{W^{4}}{(1 + W^{2})^{2}}\right\}^{-1} \leq C. 
\end{align*}
Finally, we proceed from the relations~\eqref{h1'-h2'} to obtain the upper bounds
\begin{align*}
	h_1'(x) &\leq \frac{ \EE\left\{ W^{2} \right\} }{(1+x^{2})^{1.5} \cdot \EE\bigl\{ \frac{W^{2}}{1 + W^{2}}\bigr\} } \leq \frac{5}{(1+x^{2})^{1.5}} \qquad \text{ and }\\
	h_2'(x) &\leq \frac{ \EE\left\{ W^{4} \right\} }{(1+x^{2})^{2.5} \cdot \EE\bigl\{ \frac{W^{4}}{(1 + W^{2} )^{2}}\bigr\} } \leq \frac{30}{(1+x^{2})^{2.5}},
\end{align*}
which completes the proof. \qed

\subsubsection{Proof of Lemma~\ref{f-h-properties-nonlinear}}\label{sec:proof-f-h-properties-nonlinear}
We prove each part in turn, starting with part (a). 
\paragraph{Proof of Lemma~\ref{f-h-properties-nonlinear}(a)}
Using the functions $h_1$ and $h_2$~\eqref{eq:def-h1-h2}, we write
\begin{align}\label{eq1-proof-f-h-properties-nonlinear}
	\ratiomapbit(x) = \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{h_{1}(1/\sqrt{x})^{2}} + \frac{1}{C(\oversamp)} \cdot \frac{ C_3(\oversamp) }{ C_2(\oversamp) } \cdot \left( 1 - 2\cdot \frac{h_{2}(1/\sqrt{x})}{h_{1}(1/\sqrt{x})} \right).
\end{align}
Since 
\[
\frac{C_3(\oversamp)}{C_2(\oversamp)} \leq \frac{\EE\{W^{4}\} }{ \EE\left\{ \frac{W^{2}}{ (1+W^{2})^{2}} \right\} } \leq 20,
\]
Computing the derivative and applying the triangle inequality in conjunction with the inequality $C_3(\oversamp)/C_2(\oversamp)  \leq 20$ yields the upper bound
\begin{align}\label{ineq1-h'-onebit-property-proof}
	|\ratiomapbit'(x)| \leq &\frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{|h_{1}'(1/\sqrt{x}) \cdot x^{-1.5}|}{h_{1}(1/\sqrt{x})^{3}} \nonumber\\
	&\qquad \qquad \qquad + \frac{20}{C(\oversamp)} \cdot \Bigl( \frac{|h_{2}'(1/\sqrt{x}) \cdot x^{-1.5}|}{h_{1}(1/\sqrt{x})} +  \frac{h_{2}(1/\sqrt{x})|h_{1}'(1/\sqrt{x}) \cdot x^{-1.5}|}{h_{1}(1/\sqrt{x})^{2}} \Bigr).
\end{align}
Applying Lemma~\ref{lemma1-proof-f-h-main-properties} yields 
\begin{align}\label{ineq2-h'-onebit-property-proof}
	(i.)\;\; |h_{1}'(1/\sqrt{x}) &\cdot x^{-1.5}| \leq \frac{5x^{-1.5}}{(1+1/x)^{1.5}} \leq 5, \qquad (ii.)\;\; h_2(x) \leq C \qquad \text{ and } \nonumber \\
	&(iii.)\;\; |h_{2}'(1/\sqrt{x}) \cdot x^{-1.5}| \leq \frac{30x^{-1.5}}{(1+1/x)^{2.5}} \leq 30x. 
\end{align}
We consider two cases: $x \leq 100$ and $x > 100$.

\bigskip
\noindent\underline{Case 1: $x \leq 100$.} Note that $h_{1}(x)$ is a monotone increasing function, whence
\[
h_{1}(1/\sqrt{x}) \geq h_{1}(1/\sqrt{100}) \geq 0.1/1.01^{3/2} \qquad \text{ for } x \leq 100,
\]
 Consequently, substituting the inequalities~\eqref{ineq2-h'-onebit-property-proof}, $h_{1}(1/\sqrt{x}) \geq 0.1/1.01^{3/2}$ and $h_{2}(x) \leq C$ into inequality~\eqref{ineq1-h'-onebit-property-proof}, we obtain that for $x\leq100$
\[
|\ratiomapbit'(x)| \leq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{5}{(0.1/1.01^{3/2})^{3}} + \frac{20}{C(\oversamp)} \cdot \left( \frac{30x}{0.1/1.01^{3/2}} +  \frac{5C}{(0.1/1.01^{3/2})^{2}} \right) \leq \frac{C}{C(\oversamp)},
\]
where the last inequality follows since $x\leq100$ and $C$ a large enough constant.  This concludes the first case.

\bigskip
\noindent\underline{Case 2: $x > 100$.} By Lemma~\ref{lemma1-proof-f-h-main-properties}, $h_{1}(1/\sqrt{x}) \geq 1/(1.01^{1.5}\sqrt{x})$ for $x\geq 100$. Consequently, we obtain that for $x\geq 100$,
\[
|\ratiomapbit'(x)| \leq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{5}{(1/(1.01^{1.5}\sqrt{x}))^{3}} + \frac{20}{C(\oversamp)} \cdot \left( \frac{30x}{1/(1.01^{1.5}\sqrt{x})} +  \frac{5C}{(1/(1.01^{1.5}\sqrt{x}))^{2}} \right) \leq \frac{Cx^{1.5}}{C(\oversamp)},
\]
which concludes the second case. 

Combining the two cases yields part (a), so we turn now to part (b).

\paragraph{Proof of Lemma~\ref{f-h-properties-nonlinear}(b)} Use the function $h_1$ to write
\[
\parmapbit(\parcompX,\perpcompX) = \frac{2}{\pi} \cdot (\parcompX^{2} + \perpcompX^{2})^{-1/2} \cdot h_{1}(\parcompX/\perpcompX).
\]
If $\parcompX/\perpcompX \geq 1$,then applying the monotone increasing nature of  $h_{1}(x)$ in conjunction with Lemma~\ref{lemma1-proof-f-h-main-properties} yields the lower bound $h_{1}(\parcompX/\perpcompX) \geq h_{1}(1) \geq 2^{-1.5}$.  Consequently, 
\[
\parmapbit(\parcompX,\perpcompX) \geq \frac{1}{\sqrt{2}\pi} \cdot (\parcompX^{2} + \perpcompX^{2})^{-1/2}, \qquad \text{ if }\qquad \frac{\parcompX}{\perpcompX} \geq 1.
\]
Conversely, if $0 \leq \parcompX/\perpcompX \leq 1$, then by Lemma~\ref{lemma1-proof-f-h-main-properties}, 
\[
h_{1}(\parcompX/\perpcompX) \geq \frac{\parcompX/\perpcompX}{(1+\parcompX^{2}/\perpcompX^{2})^{1.5}} \geq \parcompX/\perpcompX \cdot 2^{-1.5}.
\]
Consequently in this case, 
\[
\parmapbit(\parcompX,\perpcompX) \geq \frac{1}{\sqrt{2}\pi} \cdot (\parcompX^{2} + \perpcompX^{2})^{-1/2} \cdot \frac{\parcompX}{\perpcompX}, \qquad \text{ if }\qquad 0\leq\frac{\parcompX}{\perpcompX} \leq 1.
\]
Combining the two cases yields the conclusion. \qed


\subsubsection{Proof of Lemma~\ref{lem:h-sgn-properties}}\label{sec:proof-lem-h-sgn-properties}
Using the functions $h_1$ and $h_2$~\eqref{eq:def-h1-h2}, we write
\begin{align*}
	\ratiomapbit(x) = \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{h_{1}(1/\sqrt{x})^{2}} + \frac{1}{C(\oversamp)} \cdot \frac{ C_3(\oversamp) }{ C_2(\oversamp) } \cdot \left( 1 - 2\cdot \frac{h_{2}(1/\sqrt{x})}{h_{1}(1/\sqrt{x})} \right).
\end{align*}
Applying Lemma~\ref{lemma1-proof-f-h-main-properties} yields the pair of inequalities (which hold for $x > 0$)
\[
\frac{1}{\sqrt{x}} \cdot \frac{1}{(1+1/x)^{1.5}} \leq h_{1}\Bigl(\frac{1}{\sqrt{x}}\Bigr) \leq  \frac{1}{\sqrt{x}} \vee 5 \qquad \text{ and }\qquad h_{2}\Bigl(\frac{1}{\sqrt{x}}\Bigr) \leq \frac{1}{\sqrt{x}} \vee C
\]
Consequently, we note the lower bound $h_{1}(1/\sqrt{x}) \geq \frac{1}{1.01^{1.5}\sqrt{x}}$ for $x\geq 100$.  Note additionally that
\[
\frac{C_3(\oversamp)}{C_2(\oversamp)} \leq \frac{\EE\{W^{4}\} }{ \EE\left\{ \frac{W^{2}}{ (1+W^{2})^{2}} \right\} } \leq 20.
\]
Thus, we deduce the upper bound
\[
\ratiomapbit(x) \leq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot 1.01^{3} \cdot x + \frac{20}{C(\oversamp)} \leq \frac{\pi^{2}}{2} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot x + \frac{20}{C(\oversamp)}, \qquad \text{ for } x \geq 100,
\]
as well as the lower bound
\begin{align*}
	\ratiomapbit(x) \geq  \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot x + \frac{1}{C(\oversamp)} \cdot \frac{ C_3(\oversamp) }{ C_2(\oversamp)}\cdot (1-2\cdot1.01^{3/2}) &\geq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot x - \frac{25}{C(\oversamp)} \\&\overset{\1}{\geq} \frac{\pi^{2}}{8}\cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot x + \frac{20}{C(\oversamp)} \quad \text{ for } x \geq 100,
\end{align*}
where we note that step $\1$ follows since $x \geq 100$.  This proves part (a) and we turn our attention to part (b).  To this end,  note that $h_{1}(x)$ is a monotone increasing function. Thus,
\[
h_{1}(1/\sqrt{x}) \geq h_{1}(1/\sqrt{100}) \geq 0.1/1.01^{3/2} \qquad \text{ for } x \leq 100,
\]
where the final inequality follows upon applying Lemma~\ref{lemma1-proof-f-h-main-properties}.  Finally, we note that when $x \leq 100$,
\[
h(x) \leq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{h_{1}(1/\sqrt{x})^{2}} + \frac{20}{C(\oversamp)} \leq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1.01^{3}}{0.01} + \frac{20}{C(\oversamp)} \leq 50 \pi^{2} \cdot \frac{1+\sigma^{2}}{C(\oversamp)}.
\]
This concludes the proof.  \qed





\newpage
\kaccomment{Older}
\section{Proof of convergence results}
In this section, we present the proofs of Theorem~\ref{thm:global-conv-linear} and Theorem~\ref{thm:global-conv-nonlinear}.

\subsection{General strategy}
We define four bivariate functions $\parmapid, \perpmapid, \parmapbit,\perpmapbit: \mathbb{R}^2 \rightarrow \mathbb{R}$ that capturing the deterministic updates. 
\begin{definition}\label{F-G-definition}
	We define
	\begin{align*}
		\parmapid(\parcompX,\perpcompX) = \frac{\parcompX}{\parcompX^{2}+\perpcompX^{2}} \;\; \text{ and } \;\;
		\perpmapid(\parcompX,\perpcompX) =  \frac{1+\sigma^2}{C(\oversamp)} \cdot \frac{\perpcompX^2}{(\parcompX^2 + \perpcompX^2)^2} + \frac{\sigma^2}{C(\oversamp)} \cdot \frac{\parcompX^2}{(\parcompX^2 + \perpcompX^2)^2}. 
	\end{align*} 
	Let $W \sim \mathcal{N}(0, 1)$, $\phi(x) = \int_{0}^{x}e^{-\frac{t^{2}}{2}}dt$ and define
	\[
		C_{1}(\oversamp) = \EE\left\{ \frac{W^{2}}{C(\oversamp) + W^{2}}\right\}, C_{2}(\oversamp) = \EE\left\{ \frac{W^{2}}{(C(\oversamp) + W^{2})^{2}}\right\} \;\;\text{and}\;\; C_{3}(\oversamp) = \EE\left\{ \frac{W^{4}}{(C(\oversamp) + W^{2})^{2}} \right\}.
	\]
	\begin{align*}\label{F-G-nonlinear}
		\parmapbit(\parcompX, \perpcompX) &= \frac{2}{\pi} \cdot \frac{1}{\sqrt{\parcompX^{2} + \perpcompX^{2}}} \cdot \EE\left\{ \frac{|W| \cdot \phi\left(\frac{\parcompX}{\perpcompX} \cdot |W|\right)}{C(\oversamp) + W^{2}} \right\} \cdot \frac{1}{C_{1}(\oversamp)}   \;\; \text{ and } \;\; \\
		\perpmapbit(\parcompX, \perpcompX) &= \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX^{2} + \perpcompX^{2}} + \frac{\parmapbit(\parcompX, \perpcompX)^{2}}{C(\oversamp)}  \cdot \frac{C_{3}(\oversamp)}{C_{2}(\oversamp)}
		- \frac{4}{\pi} \cdot \frac{\parmapbit(\parcompX, \perpcompX)}{C(\oversamp)\sqrt{\parcompX^{2} + \perpcompX^{2}}} \cdot \EE\left\{ \frac{|W|^{3} \cdot \phi\left(\frac{\parcompX}{\perpcompX} \cdot |W|\right)}{C_{2}(\oversamp) \cdot (C(\oversamp) + W^{2})^{2}} \right\}.
	\end{align*}
\end{definition}
\begin{definition}\label{definition-of-map1}
Define the deterministic operators $\statemapid, \statemapbit : \mathbb{R}^2 \rightarrow \mathbb{R}^2$ as
\[
\statemapid(\parcompX,\perpcompX) = \left(\parmapid(\parcompX,\perpcompX), \perpmapid(\parcompX,\perpcompX)^{1/2} \right)\;\;\text{and}\;\;
\statemapbit(\parcompX,\perpcompX) = \left(\parmapbit(\parcompX,\perpcompX), \perpmapbit(\parcompX,\perpcompX)^{1/2} \right).
\]
\end{definition}
We next define two functions $\ratiomapid,\ratiomapbit: \mathbb{R} \rightarrow \mathbb{R}$ such that $\ratiomapid,\ratiomapbit$ capture how the ratio changes under the mapping $\statemapid,\statemapbit$ respectively.

\begin{definition}\label{definition-f-h}
Let $W \sim \mathcal{N}(0, 1)$, $\phi(x) = \int_{0}^{x}e^{-\frac{t^{2}}{2}}dt$ and recall $C_{1}(\oversamp),C_{2}(\oversamp)$ and $C_{3}(\oversamp)$ from definition~\ref{F-G-definition}. Define the functions $\ratiomapid,\ratiomapbit : \mathbb{R} \rightarrow \mathbb{R}$ as
\begin{align*}
\ratiomapid(x) &= \frac{1+\sigma^{2}}{C(\oversamp)} \cdot x + \frac{\sigma^{2}}{C(\oversamp)} \quad \text{and}\\
\ratiomapbit(x) &= \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot C_{1}(\oversamp)^{2} \bigg/ \EE\left\{ \frac{|W| \cdot \phi\left(\frac{|W|}{\sqrt{x}}\right)}{C(\oversamp) + W^{2}} \right\}^{2} + \frac{1}{C(\oversamp)} \cdot \frac{ C_{3}(\oversamp)}{C_{2}(\oversamp)} -
 \frac{2C_{1}(\oversamp)}{C(\oversamp)C_{2}(\oversamp)} \cdot \frac{ \EE\left\{ \frac{|W|^{3} \cdot \phi\left(\frac{|W|}{\sqrt{x}}\right) }{(C(\oversamp) + W^{2})^{2}} \right\} }{  \EE\left\{ \frac{|W| \cdot \phi\left(\frac{|W|}{\sqrt{x}}\right)}{C(\oversamp) + W^{2}} \right\} }.
\end{align*}
\end{definition}
The following lemma collects some properties of the functions $\ratiomapid$ and $\ratiomapbit$.
\begin{lemma}\label{f-h-main-properties}
Let $\ratiomapid$ and $\ratiomapbit$ be the functions in definition~\ref{definition-f-h}.
\renewcommand{\theenumi}{\roman{enumi}}
\begin{enumerate}
	\item We have that
	\begin{align*}
	&\text{if}\;(\parcompX',\perpcompX') = \statemapid(\parcompX,\perpcompX),\;\text{then}\; \left(\frac{\perpcompX'}{\parcompX'}\right)^{2} = \ratiomapid\left(\frac{\perpcompX^{2}}{\parcompX^{2}}\right)\quad \text{and}\\
	&\text{if}\;(\parcompX',\perpcompX') = \statemapbit(\parcompX,\perpcompX),\;\text{then}\; \left(\frac{\perpcompX'}{\parcompX'}\right)^{2} = \ratiomapbit\left(\frac{\perpcompX^{2}}{\parcompX^{2}}\right)
	\end{align*}
	\item We have that 
		\begin{align*}
			\frac{\pi^{2}}{8} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot x + \frac{20}{C(\oversamp)} \leq &\ratiomapbit(x) \leq \frac{\pi^{2}}{2} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot x + \frac{20}{C(\oversamp)} \;\; \text{for}\; x\geq 100 \; \text{and} \\
			&\ratiomapbit(x) \leq 50 \pi^{2} \cdot \frac{1+\sigma^{2}}{C(\oversamp)}\;\; \text{for}\; x\leq 100.
		\end{align*}
\end{enumerate}
\end{lemma}
For $0 \leq t \leq T$, we define $\parcompX_{t} = \langle \bcoefX_{t} , \bcoefX_{\star} \rangle$ and $\perpcompX_{t} = \left\Vert \bP_{\bcoefX_{\star}}^{\perp} \bcoefX_{t} \right\Vert_{2}$. For $1\leq t\leq T$, we define $\parcompZ_{t} = \langle \bcoefZ_{t} , \bcoefZ_{\star} \rangle$ and $\perpcompZ_{t} = \left\Vert \bP_{\bcoefZ_{\star}}^{\perp} \bcoefZ_{t} \right\Vert_{2}$. When $\psi(x) = x$, let $\parcompZ_{t}^{\mathsf{det}} = \parmapid(\parcompX_{t-1},\perpcompX_{t-1})$, $ \perpcompZ_{t}^{\mathsf{det}} = \perpmapid(\parcompX_{t-1},\perpcompX_{t-1})^{1/2}$, $\parcompX_{t}^{\mathsf{det}} = \parmapid(\parcompZ_{t},\perpcompZ_{t})$ and $\perpcompX_{t}^{\mathsf{det}} = \perpmapid(\parcompZ_{t},\perpcompZ_{t})^{1/2}$. When $\psi(x) = \mathsf{sign}(x)$, let $\parcompZ_{t}^{\mathsf{det}} = \parmapbit(\parcompX_{t-1},\perpcompX_{t-1})$, $ \perpcompZ_{t}^{\mathsf{det}} = \perpmapbit(\parcompX_{t-1},\perpcompX_{t-1})^{1/2}$, $\parcompX_{t}^{\mathsf{det}} = \parmapbit(\parcompZ_{t},\perpcompZ_{t})$ and $\perpcompX_{t}^{\mathsf{det}} = \perpmapbit(\parcompZ_{t},\perpcompZ_{t})^{1/2}$.\\
For $1 \leq t \leq T$, we define the following events
\begin{align*}
    \mathcal{A}_t &= \left \{ |\parcompZ_{t} - \parcompZ_{t}^{\mathsf{det}} | \leq \frac{C_{1}}{(\parcompX_{t-1}^{2} + \perpcompX_{t-1}^{2})^{1/2}} \cdot \sqrt{\frac{\log(n)}{n}}, |\perpcompZ_{t}^{2} - (\perpcompZ_{t}^{\mathsf{det}})^{2} | \leq \frac{C_{1}}{\parcompX_{t-1}^{2} + \perpcompX_{t-1}^{2}} \cdot \frac{\sqrt{d}\log^{2}(n)}{n} \right \},\\
    \mathcal{B}_t &= \left \{ |\parcompX_{t} - \parcompX_{t}^{\mathsf{det}} | \leq \frac{C_{1}}{(\parcompZ_{t}^{2} + \perpcompZ_{t}^{2})^{1/2}} \cdot \sqrt{ \frac{\log(n)}{n}}, |\perpcompX_{t}^{2} - (\perpcompX_{t}^{\mathsf{det}})^{2} | \leq \frac{C_{1}}{\parcompZ_{t}^{2} + \perpcompZ_{t}^{2}} \cdot \frac{\sqrt{d}\log^{2}(n)}{n} \right \},
\end{align*}
where $C_{1}$ is some universal constant. Having set up all the necessary definitions, we are now ready to state three techinical lemmas.
\begin{lemma}\label{lemma2-good-region}
Suppose $\frac{\perpcompX_{t}}{\parcompX_{t}}\leq 50\sqrt{\rho}$ where $\rho = \frac{C(\oversamp)}{1+\sigma^{2}}$ and and $C \leq \Lambda \leq d$ for some universal constant $C$. On event $\mathcal{A}_{t+1} \cap \mathcal{B}_{t+1}$, we have that
	\begin{align*}
		&\left| \frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} - \ratiomapid \circ \ratiomapid\left(  \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} \right)\right| \lesssim \frac{\log^{2}(n)}{\sqrt{n}},\;\text{if}\;\; \psi(x) = x.\;\; \text{And}\\
		&\left| \frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} - \ratiomapbit \circ \ratiomapbit \left(  \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} \right)\right| \lesssim \frac{\log^{2}(n)}{\sqrt{n}},\;\text{if}\;\; \psi(x) = \mathsf{sign}(x).
	\end{align*}
\end{lemma}

\begin{lemma}\label{lemma2-initialization-linear}
Consider $\psi(x)= x$ in the statistical model~\ref{eq:model}. Suppose $\frac{1}{50\sqrt{d}} \leq \parcompX_{t} \leq 1$, $0.5 \leq \perpcompX_{t}^{2} \leq 2$, $\frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} \geq \frac{20C(\oversamp)}{1+\sigma^{2}}$ and $C\log d \leq \Lambda \leq \sqrt{d}$ for some universal constant $C$. Let $\rho = \frac{C(\oversamp)}{1+\sigma^{2}}$. On event $\mathcal{A}_{t+1} \cap \mathcal{B}_{t+1}$, there exists a universal constant $C_{1}$ such that
	\begin{align*}
		\frac{\rho}{5} \cdot \parcompX_{t} \leq \parcompX_{t+1} &\leq 5\rho \cdot \parcompX_{t} \quad \text{and}\\
		\perpcompX_{t}^{2} - 12\rho \parcompX_{t}^{2}-\frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq \perpcompX_{t+1}^{2} &\leq \perpcompX_{t}^{2} + 3\parcompX_{t}^{2} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}}.
	\end{align*}
\end{lemma}


\begin{lemma}\label{lemma2-initialization-nonlinear}
Consider $\psi(x) = \mathsf{sign}(x)$ in the statistical model~\ref{eq:model}. Suppose $\frac{1}{50\sqrt{d}} \leq \parcompX_{t} \leq 1$, $0.5 \leq \perpcompX_{t}^{2} \leq 2$, $\frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} \geq \frac{50C(\oversamp)}{1+\sigma^{2}}$ and $C\log d \leq \Lambda \leq \sqrt{d}$ for some universal constant $C$. Let $\rho = \frac{C(\oversamp)}{1+\sigma^{2}}$. On event $\mathcal{A}_{t+1} \cap \mathcal{B}_{t+1}$, there exists a universal constant $C_{1}$ such that
	\begin{align*}
		\frac{\rho}{20\pi} \cdot \parcompX_{t} \leq \parcompX_{t+1} &\leq 3\rho \cdot \parcompX_{t} \quad \text{and}\\
		\perpcompX_{t}^{2} - 100\rho \parcompX_{t}^{2}-\frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq \perpcompX_{t+1}^{2} &\leq \perpcompX_{t}^{2} + 40\rho\parcompX_{t}^{2} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}}.
	\end{align*}
\end{lemma}











\subsection{Proof of Theorem~\ref{thm:global-conv-linear}}
Let $T_{0} \geq 0$ be the iteration such that $\parcompX_{t} \leq \frac{1}{30\sqrt{\rho}}$ for $0 \leq t \leq T_{0}$ and $\parcompX_{T_{0}+1} > \frac{1}{30\sqrt{\rho}}$. We first claim that for $0 \leq t \leq T_{0}$
\begin{align}\label{claim1-proof-thm-linear}
	\begin{split}
		\frac{\rho}{5} \cdot \parcompX_{t} \leq \parcompX_{t+1} &\leq 5\rho \cdot \parcompX_{t}, \;\; 0.8 \leq \perpcompX_{t}^{2} \leq 1.2  \quad \text{and}\\
		\perpcompX_{t}^{2} - 12\rho \parcompX_{t}^{2}-\frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq \perpcompX_{t+1}^{2} &\leq \perpcompX_{t}^{2} + 3\parcompX_{t}^{2} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}}.
	\end{split}
\end{align}
We further claim that
\begin{align}\label{claim2-proof-thm-linear}
	\frac{\perpcompX_{t}}{\parcompX_{t}} \leq 50\sqrt{\rho},\quad \forall\; t\geq T_{0}+1.
\end{align}
We defer the proof of claim~\ref{claim1-proof-thm-linear} and claim~\ref{claim2-proof-thm-linear} to the end of this subsection. Now we use claim~\ref{claim1-proof-thm-linear} and claim~\ref{claim2-proof-thm-linear} to prove Theorem~\ref{thm:global-conv-linear}.\\\\
\textbf{Case 1:} $0\leq t \leq T_{0}$.\\
Using cliam~\ref{claim1-proof-thm-linear} yields that $\frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq 0.5 \perpcompX_{t}^{2}$. Consequently, we obtain that
\begin{align*}
	0.5\perpcompX_{t}^{2} - 12\rho \parcompX_{t}^{2} \leq \perpcompX_{t+1}^{2} &\leq 1.5\perpcompX_{t}^{2} + 3\parcompX_{t}^{2}.
\end{align*}
Continuing, we obtain that
\begin{align}\label{ineq1-proof-thm-linear}
	\begin{split}
		\frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} &\leq \frac{1.5\perpcompX_{t}^{2} + 3\parcompX_{t}^{2}}{(\rho/5)^{2} \cdot \parcompX_{t}^{2}} \leq \frac{40}{\rho^{2}}\cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{75}{\rho^{2}} \overset{\1}{\leq} \frac{45}{\rho^{2}}\cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{2\sigma^{2}}{C(\oversamp)} \quad \text{and}\\
		\frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} &\geq \frac{0.5\perpcompX_{t}^{2} - 12\rho \parcompX_{t}^{2}}{(5\rho)^{2} \cdot \parcompX_{t}^{2}} = \frac{1}{50\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} - \frac{12}{25\rho} \overset{\2}{\geq}  \frac{1}{60\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{\sigma^{2}}{C(\oversamp)},
	\end{split}
\end{align}
where in step $\1$ and step $\2$ we use $\frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} \geq 0.8\cdot30^{2}\cdot\rho$.\\\\
\textbf{Case 2:} $t\geq T_{0}+1$.\\
Using Claim~\ref{claim2-proof-thm-linear} yields that $\frac{\perpcompX_{t}}{\parcompX_{t}} \leq 50\sqrt{\rho}$. Now applying Lemma~\ref{lemma2-good-region}, we obtain that there exists some universal constant $C_{1}$ such that
\[
	\left| \frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} - \left(  \left(\frac{1+\sigma^{2}}{C(\oversamp)}\right)^{2} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{\sigma^{2}}{C(\oversamp)} \cdot \left(1+\frac{1+\sigma^{2}}{C(\oversamp)}\right) \right)\right| \leq \frac{C_{1}\log^{2}(d)}{\sqrt{d}}.
\]
Consequently, we obtain that
\begin{align}\label{ineq2-proof-thm-linear}
	\begin{split}
		&\frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} \leq \frac{1}{\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{\sigma^{2}}{C(\oversamp)} \cdot \left(1+\frac{1+\sigma^{2}}{C(\oversamp)}\right) + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq \frac{1}{\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{2\sigma^{2}}{C(\oversamp)}  + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \quad \text{and}\\
		&\frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} \geq \frac{1}{\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{\sigma^{2}}{C(\oversamp)} \cdot \left(1+\frac{1+\sigma^{2}}{C(\oversamp)}\right) - \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \geq \frac{1}{\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{\sigma^{2}}{C(\oversamp)} - \frac{C_{1}\log^{2}(d)}{\sqrt{d}}.
	\end{split} 
\end{align}
Finally, putting the inequalities~\eqref{ineq1-proof-thm-linear} and~\eqref{ineq2-proof-thm-linear} together yields the desired result. 


\paragraph{Proof of claim~\ref{claim1-proof-thm-linear}:} We prove it by induction on $t$.\\
\textbf{Base case:} $t = 0$. The conditions $d^{-1/2}/50 \leq \parcompX_{0} \leq d^{-1/2}$, $\parcompX_{0}^{2} + \perpcompX_{0}^{2} = 1$ and $\oversamp \leq \sqrt{d}$ imply that
\[
	\frac{1}{50\sqrt{d}} \leq \parcompX_{0} \leq 1, 0.8 \leq \perpcompX_{0}^{2} \leq 1.2 \;\text{and}\;\frac{\perpcompX_{0}^{2}}{\parcompX_{0}^{2}} \geq 0.8d \geq \frac{20C(\oversamp)}{1+\sigma^{2}}. 
\]
Now, applying Lemma~\ref{lemma2-initialization-linear} yields the desired result for $t=0$.\\\\
\textbf{Induction step:} Suppose cliam~\ref{claim1-proof-thm-linear} holds for $0 \leq t \leq k$ such that $0 \leq k\leq T_{0}-1$. We need to prove claim~\ref{claim1-proof-thm-linear} for $t = k+1$. Since $k+1 \leq T_{0}$, we have that $\parcompX_{k+1} \leq \frac{1}{30\sqrt{\rho}}$. By induction hypothesis, we obtain that for $0 \leq t\leq k$,
\begin{align*}
	\frac{\rho}{5} \cdot  \parcompX_{t} \leq &\parcompX_{t+1} \leq 5\rho \cdot \parcompX_{t} \quad \text{and}\\
	\perpcompX_{t}^{2} - 12\rho \parcompX_{t}^{2}-\frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq \perpcompX_{t+1}^{2} &\leq \perpcompX_{t}^{2} + 3\parcompX_{t}^{2} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}}.
\end{align*}
Consequently, we obtain that $\parcompX_{k} \geq (\rho/5)^{k-t} \cdot \parcompX_{t}$ for $0 \leq t \leq k$ and also $\parcompX_{k+1} \geq (\rho/5)^{k+1} \cdot \parcompX_{0}$. Using $\parcompX_{k+1}\leq \frac{1}{30\sqrt{\rho}}$ we obtain that
\[
	(\rho/5)^{k+1} \cdot \parcompX_{0} \leq \parcompX_{k+1} \leq \frac{1}{30\sqrt{\rho}}.
\]
Consequently, we obtain that 
\[
	k+1 \leq \log_{\rho/5}\left(\frac{1}{30\sqrt{\rho} \cdot \parcompX_{0}} \right) \overset{\1}{\leq} \log_{\rho/5}\left(\frac{5\sqrt{d}}{3\sqrt{\rho} } \right) \leq \log_{\rho/5}(d),
\]
where in step $\1$ we use $\parcompX_{0} \geq d^{-1/2}/50$. Using $\parcompX_{k} \geq (\rho/5)^{k-t} \cdot \parcompX_{t}$ for $0 \leq t \leq k$, we obtain that
\begin{align*}
	\sum_{t=0}^{k} \parcompX_{t}^{2} \leq \sum_{t=0}^{k} (\rho/5)^{2t-2k}\parcompX_{k}^{2} \leq \parcompX_{k}^{2} \cdot \sum_{t=0}^{k}(\rho/5)^{-2t} \leq 2\parcompX_{k}^{2} \leq \frac{1}{450\rho},
\end{align*}
where in the last step we use $\parcompX_{k} \leq 1/(30\sqrt{\rho})$ since $k\leq T_{0}$. Putting the pieces together, we obtain that
\begin{align*}
	\perpcompX_{k+1}^{2} &\leq \perpcompX_{0}^{2} + 3\sum_{t=0}^{k} \parcompX_{t}^{2} + (k+1) \cdot \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq 1+3\cdot \frac{1}{450\rho} + \log_{\rho/5}(d)  \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq 1.2 \quad \text{and}\\
	\perpcompX_{k+1}^{2} &\geq \perpcompX_{0}^{2} - 12\rho\sum_{t=0}^{k} \parcompX_{t}^{2} - (k+1) \cdot \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \geq 0.9 - \frac{12\rho}{450\rho} - \log_{\rho/5}(d)  \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \geq 0.8.
\end{align*}
Using the condition $\parcompX_{k+1}\leq \frac{1}{30\sqrt{\rho}}$ yields that
\[
	\perpcompX_{k+1}^{2}/\parcompX_{k+1}^{2} \geq 0.8 \cdot 900 \cdot \rho \geq 20\rho = \frac{20C(\oversamp)}{1+\sigma^{2}}.
\]
To this end, we have obtained that
\[
	\frac{1}{50\sqrt{d}} \leq \parcompX_{0} \leq \parcompX_{k+1} \leq \frac{1}{30\sqrt{\rho}} \leq 1, 0.8 \leq \perpcompX_{k+1}^{2} \leq 1.2 \;\;\text{and}\;\; \frac{\perpcompX_{k+1}^{2}}{\parcompX_{k+1}^{2}} \geq \frac{20C(\oversamp)}{1+\sigma^{2}}.
\]
Now applying Lemma~\ref{lemma2-initialization-linear} for $t=k+1$ yields the desired result.\\


\paragraph{Proof of claim~\ref{claim2-proof-thm-linear}:} We prove it by induction on $t$.\\
\textbf{Base case:} $t= T_{0}+1$. Using claim~\ref{claim1-proof-thm-linear} 
\begin{align*}
	\perpcompX_{T_{0}+1}^{2} \leq \perpcompX_{T_{0}}^{2} + 3\parcompX_{T_{0}}^{2} +\frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq 1.2 + \frac{3}{900\rho} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq 1.5
\end{align*}
Using claim~\ref{claim1-proof-thm-linear} yields that
\[
	\frac{\perpcompX_{T_{0}+1}}{\parcompX_{T_{0}+1}} \leq \frac{1.5}{\frac{1}{30\sqrt{\rho}}} \leq 50\sqrt{\rho}.
\]
\textbf{Induction step:} Suppose claim~\ref{claim2-proof-thm-linear} holds for $T_{0} + 1\leq t \leq k$ for some $k \geq T_{0}+1$. We need prove claim~\ref{claim2-proof-thm-linear} for $t=k+1$. Using $\frac{\perpcompX_{k}}{\parcompX_{k}} \leq 50\sqrt{rho}$ and applying Lemma~\ref{lemma2-good-region} for $t = k$ yields that
\[
	\frac{\perpcompX_{k+1}^{2}}{\parcompX_{k+1}^{2}} \leq \frac{1}{\rho^{2}} \cdot \frac{\perpcompX_{k}^{2}}{\parcompX_{k}^{2}} + \frac{\sigma^{2}}{C(\oversamp)} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq (50\sqrt{\rho})^{2}.
\]
So we obtain $\frac{\perpcompX_{k+1}}{\parcompX_{k+1}} \leq 50\sqrt{\rho}$.
































\subsection{Proof of Theorem~\ref{thm:global-conv-nonlinear}}
Let $T_{0} \geq 0$ be the iteration such that $\parcompX_{t} \leq \frac{1}{30\sqrt{\rho}}$ for $0 \leq t \leq T_{0}$ and $\parcompX_{T_{0}+1} > \frac{1}{30\sqrt{\rho}}$. We first claim that for $0 \leq t \leq T_{0}$
\begin{align}\label{claim1-proof-thm-nonlinear}
	\begin{split}
		\frac{\rho}{20\pi} \cdot \parcompX_{t} \leq \parcompX_{t+1} &\leq 3\rho \cdot \parcompX_{t}, \;\; 0.8 \leq \perpcompX_{t}^{2} \leq 1.2  \quad \text{and}\\
		\perpcompX_{t}^{2} - 100\rho \parcompX_{t}^{2}-\frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq \perpcompX_{t+1}^{2} &\leq \perpcompX_{t}^{2} + 40\rho\parcompX_{t}^{2} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}}.
	\end{split}
\end{align}
We further claim such that
\begin{align}\label{claim2-proof-thm-nonlinear}
	&\frac{\perpcompX_{t}}{\parcompX_{t}} \leq 50\sqrt{\rho},\quad \forall\; t \geq T_{0}+1.
\end{align}
Let $T_{1}$ be the first iteration such that $\frac{\perpcompX_{T_{1}}}{\parcompX_{T_{1}}} \leq 10$. We claim that
\begin{align}\label{claim3-proof-thm-nonlinear}
	\frac{\perpcompX_{t}}{\parcompX_{t}} \leq 10\quad \forall\; t \geq T_{1}.
\end{align}
We defer the proof of claim~\ref{claim1-proof-thm-nonlinear}, claim~\ref{claim2-proof-thm-nonlinear} and claim~\ref{claim3-proof-thm-nonlinear} to the end of this subsection. Now we use the above claims to prove Theorem~\ref{thm:global-conv-nonlinear}. Using claim~\ref{claim1-proof-thm-nonlinear} yields that for $0 \leq t\leq T_{0}$
\[
	\frac{\perpcompX_{t}}{\parcompX_{t}} \geq \frac{\sqrt{0.8}}{\frac{1}{30\sqrt{\rho}}} = \sqrt{0.8} \cdot 30\sqrt{\rho} >10.
\]
So by definition we obtain that $T_{1}\geq T_{0}+1$.\\\\
\textbf{Case 1:} $0\leq t \leq T_{0}$.\\
Using cliam~\ref{claim1-proof-thm-nonlinear} yields that $\frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq 0.5 \perpcompX_{t}^{2}$. Consequently, we obtain that
\begin{align*}
	0.5\perpcompX_{t}^{2} - 100\rho \parcompX_{t}^{2} \leq \perpcompX_{t+1}^{2} &\leq 1.5\perpcompX_{t}^{2} + 40\rho\parcompX_{t}^{2}.
\end{align*}
Continuing, we obtain that
\begin{align}\label{ineq1-proof-thm-nonlinear}
	\begin{split}
		\frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} &\leq \frac{1.5\perpcompX_{t}^{2} + 40\rho\parcompX_{t}^{2}}{(\rho/(20\pi))^{2} \cdot \parcompX_{t}^{2}} \leq \frac{600\pi^{2}}{\rho^{2}}\cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{(20\pi)^{2}\cdot 40}{\rho} \overset{\1}{\leq} \frac{(30\pi)^{2}}{\rho^{2}}\cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{30}{C(\oversamp)} \quad \text{and}\\
		\frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} &\geq \frac{0.5\perpcompX_{t}^{2} - 100\rho \parcompX_{t}^{2}}{(3\rho)^{2} \cdot \parcompX_{t}^{2}} = \frac{1}{18\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} - \frac{100}{9\rho} \overset{\2}{\geq}  \frac{1}{20\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{20}{C(\oversamp)},
	\end{split}
\end{align}
where in step $\1$ and step $\2$ we use $\frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} \geq 0.8\cdot30^{2}\cdot\rho$.\\\\
\textbf{Case 2:} $T_{0}+1 \leq t \leq T_{1}-2$.\\
Using Claim~\ref{claim2-proof-thm-nonlinear} yields that $\frac{\perpcompX_{t}}{\parcompX_{t}} \leq 50\sqrt{\rho}$. Now applying Lemma~\ref{lemma2-good-region}, we obtain that there exists some universal constant $C_{1}$ such that
\[
	\left| \frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} - \ratiomapbit \circ \ratiomapbit \left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right)\right| \leq \frac{C_{1}\log^{2}(d)}{\sqrt{d}}.
\]
We next show that $\ratiomapbit \left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) > 100$. Assume that $\ratiomapbit \left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \leq 100$. Then applying part $\2$ of Lemma~\ref{f-h-main-properties} yields that
\[
	\ratiomapbit \circ \ratiomapbit \left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \leq \frac{50\pi^{2}(1+\sigma^{2})}{C(\oversamp)}.
\]
Consequently, we obtain that
\[
	\frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} \leq \frac{50\pi^{2}(1+\sigma^{2})}{C(\oversamp)} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq 100.
\]
By definition, $T_{1} \leq t+1$. This contradicts with the fact that $t<T_{1}-1$. So we conclude that $\ratiomapbit \left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \geq 100$. Then using part $\2$ of Lemma~\ref{f-h-main-properties} yields that
\begin{align*}
	 \frac{\pi^{4}}{64} \cdot \frac{1}{\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{20}{C(\oversamp)} \leq \ratiomapbit \circ \ratiomapbit \left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \leq \frac{\pi^{4}}{4} \cdot \frac{1}{\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{30}{C(\oversamp)}.
\end{align*}
Consequently, we obtain that
\begin{align*}
	&\frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} \leq \frac{\pi^{4}}{4} \cdot \frac{1}{\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{30}{C(\oversamp)} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}}\quad \text{and}\\
	&\frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} \geq \frac{\pi^{4}}{64} \cdot \frac{1}{\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{20}{C(\oversamp)} - \frac{C_{1}\log^{2}(d)}{\sqrt{d}}.
\end{align*}\\\\
\textbf{Case 3:} $t\geq T_{1}$.\\
Using claim~\ref{claim3-proof-thm-nonlinear} yields that $\frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} \leq 100$. Applying part $\2$ of Lemma~\ref{f-h-main-properties} yields that
\[
	\ratiomapbit \circ \ratiomapbit \left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \leq \frac{50\pi^{2}(1+\sigma^{2})}{C(\oversamp)}.
\]
Applying Lemma~\ref{lemma2-good-region} yields that
\[
	\frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} \leq \frac{50\pi^{2}(1+\sigma^{2})}{C(\oversamp)} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}}.
\]
Putting the three cases together yields that
\begin{align*}
		\frac{1}{20\rho^{2}} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{20}{C(\oversamp)} - \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq \frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} &\leq  \frac{(30\pi)^{2}}{\rho^{2}}\cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{30}{C(\oversamp)} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}},\;\;\text{for}\;\;0 \leq t \leq T_{1}-2 \;\;\text{and}\\
		\frac{\perpcompX_{t+1}^{2}}{\parcompX_{t+1}^{2}} &\leq \frac{50\pi^{2}(1+\sigma^{2})}{C(\oversamp)} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}}\;\;\text{for}\;\;t\geq T_{1}.
\end{align*}
Consequently, we obtain that $T_{1} = \mathcal{O}\left(\log_{\rho^{2}}\left(\frac{\perpcompX_{0}^{2}}{\parcompX_{0}^{2}}\right)\right) = \mathcal{O}\left(\log_{n/d}\left(d\right)\right)$, where in the lase equality we use $\frac{\perpcompX_{0}^{2}}{\parcompX_{0}^{2}} \asymp d$ and $\rho \asymp \oversamp = n/d$.





\paragraph{Proof of claim~\ref{claim1-proof-thm-nonlinear}:} We prove it by induction on $t$.\\
\textbf{Base case:} $t = 0$. The conditions $d^{-1/2}/50 \leq \parcompX_{0} \leq d^{-1/2}$, $\parcompX_{0}^{2} + \perpcompX_{0}^{2} = 1$ and $\oversamp \leq \sqrt{d}$ imply that
\[
	\frac{1}{50\sqrt{d}} \leq \parcompX_{0} \leq 1, 0.8 \leq \perpcompX_{0}^{2} \leq 1.2 \;\text{and}\;\frac{\perpcompX_{0}^{2}}{\parcompX_{0}^{2}} \geq 0.8d \geq \frac{20C(\oversamp)}{1+\sigma^{2}}. 
\]
Now, applying Lemma~\ref{lemma2-initialization-nonlinear} yields the desired result for $t=0$.\\\\
\textbf{Induction step:} Suppose cliam~\ref{claim1-proof-thm-nonlinear} holds for $0 \leq t \leq k$ such that $0 \leq k\leq T_{0}-1$. We need to prove claim~\ref{claim1-proof-thm-nonlinear} for $t = k+1$. Since $k+1 \leq T_{0}$, we have that $\parcompX_{k+1} \leq \frac{1}{30\sqrt{\rho}}$. By induction hypothesis, we obtain that for $0 \leq t\leq k$,
\begin{align*}
	\frac{\rho}{20\pi} \cdot  \parcompX_{t} \leq &\parcompX_{t+1} \leq 3\rho \cdot \parcompX_{t} \quad \text{and}\\
	\perpcompX_{t}^{2} - 100\rho \parcompX_{t}^{2}-\frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq \perpcompX_{t+1}^{2} &\leq \perpcompX_{t}^{2} + 40\rho\parcompX_{t}^{2} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}}.
\end{align*}
Consequently, we obtain that $\parcompX_{k} \geq (\rho/(20\pi))^{k-t} \cdot \parcompX_{t}$ for $0 \leq t \leq k$ and also $\parcompX_{k+1} \geq (\rho/(20\pi))^{k+1} \cdot \parcompX_{0}$. Using $\parcompX_{k+1}\leq \frac{1}{30\sqrt{\rho}}$ we obtain that
\[
	(\rho/(20\pi))^{k+1} \cdot \parcompX_{0} \leq \parcompX_{k+1} \leq \frac{1}{30\sqrt{\rho}}.
\]
Consequently, we obtain that 
\[
	k+1 \leq \log_{\rho/(20\pi)}\left(\frac{1}{30\sqrt{\rho} \cdot \parcompX_{0}} \right) \overset{\1}{\leq} \log_{\rho/(20\pi)}\left(\frac{5\sqrt{d}}{3\sqrt{\rho} } \right) \leq \log_{\rho/(20\pi)}(d),
\]
where in step $\1$ we use $\parcompX_{0} \geq d^{-1/2}/50$. Using $\parcompX_{k} \geq (\rho/(20\pi))^{k-t} \cdot \parcompX_{t}$ for $0 \leq t \leq k$, we obtain that
\begin{align*}
	\sum_{t=0}^{k} \parcompX_{t}^{2} \leq \sum_{t=0}^{k} (\rho/(20\pi))^{2t-2k}\parcompX_{k}^{2} \leq \parcompX_{k}^{2} \cdot \sum_{t=0}^{k}(\rho/(20\pi))^{-2t} \leq 1.1\parcompX_{k}^{2} \leq \frac{1.1}{900\rho},
\end{align*}
where in the last step we use $\parcompX_{k} \leq 1/(30\sqrt{\rho})$ since $k\leq T_{0}$. Putting the pieces together, we obtain that
\begin{align*}
	\perpcompX_{k+1}^{2} &\leq \perpcompX_{0}^{2} + 40\rho\sum_{t=0}^{k} \parcompX_{t}^{2} + (k+1) \cdot \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq 1+ \frac{40\rho}{450\rho} + \log_{\rho/5}(d)  \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq 1.2 \quad \text{and}\\
	\perpcompX_{k+1}^{2} &\geq \perpcompX_{0}^{2} - 100\rho\sum_{t=0}^{k} \parcompX_{t}^{2} - (k+1) \cdot \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \geq 1 - \frac{1}{d} - \frac{110\rho}{900\rho} - \log_{\rho/5}(d)  \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \geq 0.8.
\end{align*}
Using the condition $\parcompX_{k+1}\leq \frac{1}{30\sqrt{\rho}}$ yields that
\[
	\perpcompX_{k+1}^{2}/\parcompX_{k+1}^{2} \geq 0.8 \cdot 900 \cdot \rho \geq 20\rho = \frac{20C(\oversamp)}{1+\sigma^{2}}.
\]
To this end, we have obtained that
\[
	\frac{1}{50\sqrt{d}} \leq \parcompX_{0} \leq \parcompX_{k+1} \leq \frac{1}{30\sqrt{\rho}} \leq 1, 0.8 \leq \perpcompX_{k+1}^{2} \leq 1.2 \;\;\text{and}\;\; \frac{\perpcompX_{k+1}^{2}}{\parcompX_{k+1}^{2}} \geq \frac{20C(\oversamp)}{1+\sigma^{2}}.
\]
Now applying Lemma~\ref{lemma2-initialization-linear} for $t=k+1$ yields the desired result.\\


\paragraph{Proof of claim~\ref{claim2-proof-thm-nonlinear}:} We prove it by induction on $t$.
\textbf{Base case:} $t= T_{0}+1$. Using claim~\ref{claim1-proof-thm-linear} 
\begin{align*}
	\perpcompX_{T_{0}+1}^{2} \leq \perpcompX_{T_{0}}^{2} + 40\rho\parcompX_{T_{0}}^{2} +\frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq 1.2 + \frac{40\rho}{900\rho} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq 1.5
\end{align*}
Using $\parcompX_{T_{0}+1} \geq \frac{1}{30\sqrt{\rho}}$ yields that
\[
	\frac{\perpcompX_{T_{0}+1}}{\parcompX_{T_{0}+1}} \leq \frac{1.5}{\frac{1}{30\sqrt{\rho}}} \leq 50\sqrt{\rho}.
\]
\textbf{Induction step:} Suppose claim~\ref{claim2-proof-thm-nonlinear} holds for $T_{0} + 1\leq t \leq k$ for some $k \geq T_{0}+1$. We need prove claim~\ref{claim2-proof-thm-nonlinear} for $t=k+1$. Using $\frac{\perpcompX_{k}}{\parcompX_{k}} \leq 50\sqrt{rho}$ and applying Lemma~\ref{lemma2-good-region} for $t = k$ yields that
\[
	\frac{\perpcompX_{k+1}^{2}}{\parcompX_{k+1}^{2}} \leq \ratiomapbit \circ \ratiomapbit\left( \frac{\perpcompX_{k}^{2}}{\parcompX_{k}^{2}}\right) + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq (50\sqrt{\rho})^{2}.
\]
So we obtain $\frac{\perpcompX_{k+1}}{\parcompX_{k+1}} \leq 50\sqrt{\rho}$.

\paragraph{Proof of claim~\ref{claim3-proof-thm-nonlinear}:} We prove it by induction on $t$.\\
\textbf{Base case:} $t= T_{1}$. By definition we have that $\frac{\perpcompX_{t}}{\parcompX_{t}} \leq 10$.\\
\textbf{Induction step:} Suppose claim~\ref{claim3-proof-thm-nonlinear} holds for $T_{1}\leq t \leq k$ for some $k \geq T_{1}$. We need prove claim~\ref{claim3-proof-thm-nonlinear} for $t=k+1$. Using $\frac{\perpcompX_{k}}{\parcompX_{k}} \leq 10$ and applying Lemma~\ref{lemma2-good-region} for $t = k$ yields that
\[
	\frac{\perpcompX_{k+1}^{2}}{\parcompX_{k+1}^{2}} \leq \ratiomapbit \circ \ratiomapbit \left( \frac{\perpcompX_{k}^{2}}{\parcompX_{k}^{2}}\right) + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq  \frac{50\pi^{2}}{\rho} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq 100,
\]
where in the last step we use part $\2$ of Lemma~\ref{f-h-main-properties}. So we obtain $\frac{\perpcompX_{k+1}}{\parcompX_{k+1}} \leq 10$.























\subsection{Proof of Lemma~\ref{f-h-main-properties}}
We start with some useful definition.
\begin{definition}\label{h1-h2-definition} We define for $x>0$
\[
	h_{1}(x) = \EE\left\{ \frac{|W|  \int_{0}^{x \cdot |W|}  e^{-t^{2}/2} dt}{C(\oversamp) + W^{2}} \right\} \bigg/ \EE\left\{ \frac{W^{2}}{C(\oversamp) + W^{2}}\right\}, h_{2}(x) = \EE\left\{ \frac{|W|^{3}  \int_{0}^{x \cdot |W|}  e^{-t^{2}/2} dt}{(C(\oversamp) + W^{2})^{2}} \right\} \bigg/ \EE\left\{ \frac{W^{4}}{(C(\oversamp) + W^{2})^{2}} \right\}.
\]
\end{definition}
The proof requires the following techinical lemma which is proved at the end of this this subsection. 
\begin{lemma}\label{lemma1-proof-f-h-main-properties} There exists a universal positive constant $C$ such that for $x>0$,
	\begin{align*}
		\frac{x}{(1+x^{2})^{1.5}} &\leq h_{1}(x) \leq  x,\ h_{2}(x) \leq x , h_{1}(x) \leq 5, h_{2}(x) \leq C\\ 
		\frac{1}{(1+x^{2})^{1.5}} &\leq h_{1}'(x) \leq \frac{5}{(1+x^{2})^{1.5}}\; \text{and}\; 0 \leq h_{2}'(x) \leq \frac{30}{(1+x^{2})^{2.5}}.
	\end{align*}
\end{lemma}
\paragraph{Proof of Lemma~\ref{f-h-main-properties}:}
We start with part $\1$. If $(\parcompX',\perpcompX') = \statemapid(\parcompX,\perpcompX)$, then by definition we have that $\parcompX' = \parmapid(\parcompX,\perpcompX) = \frac{\parcompX}{\parcompX^{2}+\perpcompX^{2}}$ and $(\perpcompX')^{2} = \perpmapid(\parcompX,\perpcompX) = \frac{1+\sigma^{2}}{C(\oversamp)}\cdot \frac{\perpcompX^{2}}{(\parcompX^{2}+\perpcompX^{2})^{2}} + \frac{\sigma^{2}}{C(\oversamp)} \cdot \frac{\parcompX^{2}}{(\parcompX^{2}+\perpcompX^{2})^{2}}$. Consequently, we obtain that $\frac{(\perpcompX')^{2}}{(\parcompX')^{2}} = \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{\perpcompX^{2}}{\parcompX^{2}} + \frac{\sigma^{2}}{C(\oversamp)} = \ratiomapid(\perpcompX^{2}/\parcompX^{2})$.\\
If $(\parcompX',\perpcompX') = \statemapbit(\parcompX,\perpcompX)$, then by definition $\parcompX' = \parmapid(\parcompX,\perpcompX)$ and $(\perpcompX')^{2} = \perpmapbit(\parcompX,\perpcompX)$. Consequently, $\frac{(\perpcompX')^{2}}{(\parcompX')^{2}} = \frac{\perpmapbit(\parcompX,\perpcompX)}{\parmapbit(\parcompX,\perpcompX)^{2}} = \ratiomapbit(\perpcompX^{2}/\parcompX^{2})$.\\
Next we prove part $\2$. To reduce the notational burden, let $h(x) = \ratiomapbit(x)$. Recall $h_{1}(x)$ and $h_{2}(x)$ in definition~\ref{h1-h2-definition}. Using the definition of $\ratiomapbit$, we obtain that 
\begin{align*}
h(x) = \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{h_{1}(1/\sqrt{x})^{2}} + \frac{1}{C(\oversamp)} \cdot \frac{ \EE\left\{ \frac{W^{4}}{ (C(\oversamp)+W^{2} )^{2} } \right\} }{ \EE\left\{ \frac{W^{2}}{ (C(\oversamp)+W^{2})^{2}} \right\}} \cdot \left( 1 - 2\cdot \frac{h_{2}(1/\sqrt{x})}{h_{1}(1/\sqrt{x})} \right).
\end{align*}
Applying Lemma~\ref{lemma1-proof-f-h-main-properties} yields that for $x>0$
\[
	\frac{1}{\sqrt{x}} \cdot \frac{1}{(1+1/x)^{1.5}} \leq h_{1}(1/\sqrt{x}) \leq  \frac{1}{\sqrt{x}}\;\text{and}\; h_{2}(1/\sqrt{x}) \leq \frac{1}{\sqrt{x}}
\]
Consequently, we obtain that $h_{1}(1/\sqrt{x}) \geq \frac{1}{1.01^{1.5}\sqrt{x}}$ for $x\geq 100$. Note that 
\begin{align*}
	\frac{ \EE\left\{ \frac{W^{4}}{ (C(\oversamp)+W^{2} )^{2} } \right\} }{ \EE\left\{ \frac{W^{2}}{ (C(\oversamp)+W^{2})^{2}} \right\}} \leq \frac{ \EE\left\{ \frac{W^{4}}{ C(\oversamp)^{2} } \right\} }{ \EE\left\{ \frac{W^{2}}{ (C(\oversamp)+C(\oversamp)W^{2})^{2}} \right\}} \leq \frac{\EE\{W^{4}\} }{ \EE\left\{ \frac{W^{2}}{ (1+W^{2})^{2}} \right\} } \leq 20.
\end{align*}
Putting the pieces together yields that for $x\geq 100$
\begin{align*}
h(x) &\leq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot 1.01^{3} \cdot x + \frac{20}{C(\oversamp)} \leq \frac{\pi^{2}}{2} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot x + \frac{20}{C(\oversamp)} \quad \text{and} \\
h(x) &\geq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot x + \frac{1}{C(\oversamp)} \cdot \frac{ \EE\left\{ \frac{W^{4}}{ (C(\oversamp)+W^{2} )^{2} } \right\} }{ \EE\left\{ \frac{W^{2}}{ (C(\oversamp)+W^{2})^{2}} \right\}}\cdot (1-2\cdot1.01^{3/2}) \geq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot x - \frac{25}{C(\oversamp)} \\&\overset{\1}{\geq} \frac{\pi^{2}}{8}\cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot x + \frac{20}{C(\oversamp)},
\end{align*}
where step $\1$ follows since $x\geq 100$. Note that $h_{1}(x)$ is a monotone increasing function. So we deduce that $h_{1}(1/\sqrt{x}) \geq h_{1}(1/\sqrt{100})$ for $x \leq 100$. Using Lemma~\ref{lemma1-proof-f-h-main-properties} for $x = 100$ yields that $h(1/\sqrt{100}) \geq 0.1/1.01^{3/2}$. Consequently, we obtain that for $x\leq 100$
\[
h(x) \leq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{h_{1}(1/\sqrt{x})^{2}} + \frac{20}{C(\oversamp)} \leq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1.01^{3}}{0.01} + \frac{20}{C(\oversamp)} \leq 50 \pi^{2} \cdot \frac{1+\sigma^{2}}{C(\oversamp)}.
\]

\subsubsection{Proof of Lemma~\ref{lemma1-proof-f-h-main-properties}}
Taking the deriative of $h_{1}(x)$ and $h_{2}(x)$ yields that
\[
h_{1}'(x) = \EE\left\{ \frac{W^{2} e^{-x^{2}W^{2}/2}}{C(\oversamp) + W^{2}} \right\} \bigg/ \EE\left\{ \frac{W^{2}}{C(\oversamp) + W^{2}}\right\},\ h_{2}'(x) = \EE\left\{ \frac{W^{4}  e^{-x^{2}W^{2}/2}}{(C(\oversamp) + W^{2})^{2}} \right\} \bigg/ \EE\left\{ \frac{W^{4}}{(C(\oversamp) + W^{2})^{2}} \right\}.
\]
Using the fact $e^{-x^{2}W^{2}/2} \leq 1$, we obtan that $h_{1}'(x) \leq 1$ and $h_{2}'(x) \leq 1$. We next get lower bound of $h_{1}'(x)$. Using the fact that $W$ is a standard normal random variables yields that
\begin{align*}
\EE_{W\sim\mathcal{N}(0,1)}\left\{ \frac{W^{2} e^{-x^{2}W^{2}/2}}{C(\oversamp) + W^{2}} \right\} = \frac{ \EE_{W\sim\mathcal{N}(0,\frac{1}{1+x^{2}})}\left\{ \frac{W^{2}}{C(\oversamp) + W^{2}} \right\} }{\sqrt{1+x^{2}}}  = \frac{ \EE_{W\sim\mathcal{N}(0,1)}\left\{ \frac{W^{2}}{ C(\oversamp) + \frac{W^{2}}{1+x^{2}}} \right\} }{(1+x^{2})^{1.5}}.
\end{align*}
Similarly, we have that $\EE\left\{ \frac{W^{4}  e^{-x^{2}W^{2}/2}}{(C(\oversamp) + W^{2})^{2}} \right\} = \EE \left\{ \frac{W^{4}}{ (C(\oversamp) + W^{2}/(1+x^{2}) )^{2}} \right\} \bigg/ (1+x^{2})^{2.5}$. Consequently, we obtain that 
\begin{align}\label{h1'-h2'}
h_{1}'(x) = \frac{ \EE\left\{ \frac{W^{2}}{ C(\oversamp) + W^{2}/(1+x^{2}) } \right\} }{(1+x^{2})^{1.5} \cdot \EE\left\{ \frac{W^{2}}{C(\oversamp) + W^{2}}\right\} } \ \text{and}\ h_{2}'(x) = \frac{ \EE\left\{ \frac{W^{4}}{ ( C(\oversamp) + W^{2}/(1+x^{2}))^{2} } \right\} }{(1+x^{2})^{2.5} \cdot \EE\left\{ \frac{W^{4}}{(C(\oversamp) + W^{2} )^{2}}\right\} }.
\end{align}
We deduce that $h_{1}'(x) \geq 1/(1+x^{2})^{1.5}$ for $x>0$. Applying the lower and upper bounds of $h_{1}'(x)$ and $h_{1}(0)=0$ yields that for $x>0$.
\[
h_{1}(x) = h_{1}(0) + \int_{0}^{x} h_{1}'(t) dt \leq x \  \text{and} \ h_{1}(x) = h_{1}(0) + \int_{0}^{x} h'(t) dt \geq x/(1+x^{2})^{1.5}.
\]
Similarly, using $h_{2}'(x) \leq 1$ and $h_{2}(0)=0$ yields that $h_{2}(x) \leq x$ for $x>0$. Using $\int_{0}^{x \cdot |W|}  e^{-t^{2}/2} dt \leq \sqrt{\pi/2}$ for $x>0$ yields that
\begin{align*}
	h_{1}(x) &\leq \sqrt{\pi/2} \cdot \EE\left\{ \frac{|W|}{C(\oversamp) + W^{2}} \right\} \bigg/ \EE\left\{ \frac{W^{2}}{C(\oversamp) + W^{2}}\right\} \leq \sqrt{\pi/2} \cdot \EE\{|W|\}\bigg/ \EE\left\{ \frac{W^{2}}{1 + W^{2}}\right\} \leq 5\;\text{and}\\
	h_{2}(x) &\leq \sqrt{\pi/2} \cdot \EE\left\{ \frac{|W|^{3}}{(C(\oversamp) + W^{2})^{2}} \right\} \bigg/ \EE\left\{ \frac{W^{4}}{(C(\oversamp) + W^{2})^{2}} \right\} \leq \sqrt{\pi/2} \cdot \EE\{|W|^{3}\}\bigg/ \EE\left\{ \frac{W^{4}}{(1 + W^{2})^{2}}\right\}.
\end{align*}
Note that the right hand side of the inequality in the display above is a constant. So we conclude that $h_{1}(x) \leq 5$ and $h_{2}(x) \leq C$ for some constant $C$. Moreover,
\begin{align*}
	h_{1}'(x) &= \frac{ \EE\left\{ \frac{W^{2}}{ C(\oversamp) + W^{2}/(1+x^{2}) } \right\} }{(1+x^{2})^{1.5} \cdot \EE\left\{ \frac{W^{2}}{C(\oversamp) + W^{2}}\right\} } \leq \frac{ \EE\left\{ W^{2} \right\} }{(1+x^{2})^{1.5} \cdot \EE\left\{ \frac{W^{2}}{1 + W^{2}}\right\} } \leq \frac{5}{(1+x^{2})^{1.5}} \quad \text{and}\\
	h_{2}'(x) &= \frac{ \EE\left\{ \frac{W^{4}}{ ( C(\oversamp) + W^{2}/(1+x^{2}))^{2} } \right\} }{(1+x^{2})^{2.5} \cdot \EE\left\{ \frac{W^{4}}{(C(\oversamp) + W^{2} )^{2}}\right\} } \leq \frac{ \EE\left\{ W^{4} \right\} }{(1+x^{2})^{2.5} \cdot \EE\left\{ \frac{W^{4}}{(1 + W^{2} )^{2}}\right\} } \leq \frac{30}{(1+x^{2})^{2.5}}.
\end{align*}



















\subsection{Proof of Lemma~\ref{lemma2-good-region} for $\psi(x) = x$}
The proof requires the following auxilary lemma, which is proved at the end of this subsection.
\begin{lemma}\label{help-lemma2-GD-linear}
Let $\rho = \frac{C(\oversamp)}{1+\sigma^{2}}$. Suppose $a>0,b\geq0$ and $\frac{b}{a} \leq 50\sqrt{\rho}$. Let $a^{\mathsf{det}} = \parmapid(a,b)$ and $(b^{\mathsf{det}})^{2} = \perpmapid(a,b)$. Let $a',b' \in \mathbb{R}$ such that
\begin{align}\label{condition-help-lemma2-GD-linear}
	\left| a' - a^{\mathsf{det}}\right| \lesssim \frac{1}{\sqrt{a^{2}+b^{2}}} \cdot\sqrt{\frac{\log(n)}{n}} \; \text{and} \; \left| (b')^{2} - (b^{\mathsf{det}})^{2}\right| \lesssim \frac{1}{a^{2}+b^{2}}\cdot\frac{\sqrt{d}\log^{2}(n)}{n}.
\end{align}
Then there exists a universal constant $C$ such that for $C\leq \oversamp$ we have
\[
	\left| \left( \frac{b'}{a'} \right)^{2} - \ratiomapid\left(\frac{b^{2}}{a^{2}}\right) \right| \lesssim \max\left\{1,b^{2}/a^{2}\right\} \cdot \frac{\sqrt{d}\log^{2}(n)}{n} + \max\left\{1,b/a\right\}\cdot \sqrt{\frac{\log(n)}{n}}.
\]
\end{lemma}

\paragraph{Proof of Lemma~\ref{lemma2-good-region} for $\psi(x) = x$:} The proof takes two steps.\\
\textbf{First step:} On event $\mathcal{A}_{t+1}$, estimate $\perpcompZ_{t+1}/\parcompZ_{t+1}$.\\
Let $a = \parcompX_{t}$ and $b = \perpcompX_{t}$. By definition, $\parcompZ_{t+1}^{\mathsf{det}} = \parmapid(a,b)$ and $(\perpcompZ_{t+1}^{\mathsf{det}})^{2}=\perpmapid(a,b)$. On event $\mathcal{A}_{t+1}$, we obtain that
\[
		\left| \parcompZ_{t+1} - \parcompZ_{t+1}^{\mathsf{det}} \right| \lesssim \frac{1}{\sqrt{a^{2}+b^{2}}} \cdot\sqrt{\frac{\log(n)}{n}} \; \text{and} \; \left| (\perpcompZ_{t+1})^{2} - (\perpcompZ_{t+1}^{\mathsf{det}})^{2}\right| \lesssim \frac{1}{a^{2}+b^{2}}\cdot\frac{\sqrt{d}\log^{2}(n)}{n}.
\]
Using the condition $b/a = \perpcompX_{t}/\parcompX_{t} \leq 50\sqrt{\rho} \lesssim \sqrt{\oversamp}$ and applying Lemma~\ref{help-lemma2-GD-linear} for $a = \parcompX_{t},b = \perpcompX_{t},a' = \parcompZ_{t+1}$ and $b' = \perpcompZ_{t+1}$, we obtain that
\begin{align}\label{ineq1-lemma2-GD-linear}
\begin{split}
	\left| \left( \frac{\perpcompZ_{t+1}}{\parcompZ_{t+1}} \right)^{2} - \ratiomapid\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right| &\lesssim \max\left\{1,\perpcompX_{t}^{2}/\parcompX_{t}^{2}\right\} \cdot \frac{\sqrt{d}\log^{2}(n)}{n} + \max\left\{1,\perpcompX_{t}/\parcompX_{t}\right\}\cdot \sqrt{\frac{\log(n)}{n}} \\&\lesssim \oversamp \cdot \frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\oversamp} \cdot  \sqrt{\frac{\log(n)}{n}}.
\end{split}
\end{align}
Consequently, using $\perpcompX_{t}/\parcompX_{t} \leq 50\sqrt{\rho} \lesssim \sqrt{\oversamp}$, we obtain that there exists some universal constant $C_{1}$ such that
\begin{align*}
	\left( \frac{\perpcompZ_{t+1}}{\parcompZ_{t+1}} \right)^{2} &\leq \ratiomapid\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \\ &=
	\frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{\sigma^{2}}{C(\oversamp)} + \frac{C_{1}\log^{2}(d)}{\sqrt{d}} \leq
	50^{2}+1.
\end{align*}\\
\textbf{Second step:} On event $\mathcal{B}_{t+1}$, estimate $\perpcompX_{t+1}/\parcompX_{t+1}$.\\
Let $a = \parcompZ_{t+1}$ and $b = \perpcompZ_{t+1}$. By definition, $\parcompX_{t+1}^{\mathsf{det}} = \parmapid(a,b)$ and $(\perpcompX_{t+1}^{\mathsf{det}})^{2}=\perpmapid(a,b)$. On event $\mathcal{B}_{t+1}$, we obtain that
\[
		\left| \parcompX_{t+1} - \parcompX_{t+1}^{\mathsf{det}} \right| \lesssim \frac{1}{\sqrt{a^{2}+b^{2}}} \cdot\sqrt{\frac{\log(n)}{n}} \; \text{and} \; \left| (\perpcompX_{t+1})^{2} - (\perpcompX_{t+1}^{\mathsf{det}})^{2}\right| \lesssim \frac{1}{a^{2}+b^{2}}\cdot\frac{\log^{2}(n)}{n}.
\]
Using the condition $b/a = \perpcompZ_{t+1}/\parcompZ_{t+1} \leq 50+1$ and applying Lemma~\ref{help-lemma2-GD-linear} for $a = \parcompZ_{t+1},b = \perpcompZ_{t+1},a' = \parcompX_{t+1}$ and $b' = \perpcompX_{t+1}$, we obtain that
\begin{align}\label{ineq2-lemma2-GD-linear}
\left| \left( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \right)^{2} - \ratiomapid\left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) \right| \lesssim \frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\frac{\log(n)}{n}}.
\end{align}
Now, using the triangle inequality yields that
\begin{align*}
	\left| \left( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \right)^{2} - \ratiomapid \circ \ratiomapid\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right| &\leq
	\left| \left( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \right)^{2} - \ratiomapid\left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) \right| + 
	\left| \ratiomapid\left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) - \ratiomapid \circ \ratiomapid\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right| \\&\overset{\1}{=}
	\left| \left( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \right)^{2} - \ratiomapid\left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) \right| + 
	\frac{1+\sigma^{2}}{C(\oversamp)} \cdot \left| \left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) -  \ratiomapid\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right| \\&\overset{\2}{\lesssim}
	\frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\frac{\log(n)}{n}} + \frac{1}{\oversamp} \cdot \left( \oversamp \cdot \frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\oversamp} \cdot  \sqrt{\frac{\log(n)}{n}} \right) \\&\lesssim
	\frac{\log^{2}(n)}{\sqrt{n}}
\end{align*}
where in step $\1$ we use $\ratiomapid(x) = \frac{1+\sigma^{2}}{C(\oversamp)}\cdot x+\frac{\sigma^{2}}{C(\oversamp)}$ and step $\2$ follows from inequalities~\eqref{ineq1-lemma2-GD-linear} and~\eqref{ineq2-lemma2-GD-linear}.




\subsubsection{Proof of Lemma~\ref{help-lemma2-GD-linear}}
Using inequality~\eqref{condition-help-lemma2-GD-linear} yields that
\begin{align*}
	a' &\geq \parmapid(a,b) - \frac{C_{1}}{\sqrt{a^{2}+b^{2}}} \cdot\sqrt{\frac{\log(d)}{\oversamp \cdot d}} =
	\frac{a}{a^{2}+b^{2}} - \frac{C_{1}}{\sqrt{a^{2}+b^{2}}} \cdot\sqrt{\frac{\log(d)}{\oversamp \cdot d}} \\&=
	\frac{1}{\sqrt{a^{2}+b^{2}}}\cdot \left( \frac{1}{\sqrt{1+b^{2}/a^{2}}} - C_{1}\sqrt{\frac{\log(d)}{\oversamp \cdot d}} \right) \geq  \frac{0.5}{\sqrt{a^{2}+b^{2}}}\cdot  \frac{1}{\sqrt{1+b^{2}/a^{2}}},
\end{align*}
where $C_{1}$ is some universal constant and in the last step we use $\frac{1}{\sqrt{1+b^{2}/a^{2}}} \gtrsim \frac{1}{\sqrt{\oversamp}}$ since $b/a\leq50\sqrt{\rho} \lesssim \sqrt{\oversamp}$.
Using the triangle inequality yields that
\begin{align}\label{ineq1-help-lemma2-GD-linear}
	\begin{split}
		\left| \left( \frac{b'}{a'} \right)^{2} -\left( \frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} \right| &\leq \frac{\left| (b')^{2} - (b^{\mathsf{det}})^{2}\right|}{(a')^{2}} + 
		\left| \left( \frac{b^{\mathsf{det}}}{a'} \right)^{2} -\left( \frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} \right| \\&=
		\frac{\left| (b')^{2} - (b^{\mathsf{det}})^{2}\right|}{(a')^{2}} + \left(\frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} \cdot
		  \frac{\left| (a')^{2} - (a^{\mathsf{det}})^{2}\right|}{(a')^{2}} \\&\leq
		\frac{\left| (b')^{2} - (b^{\mathsf{det}})^{2}\right|}{(a')^{2}} + \left(\frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} \cdot
		  \left( \frac{ (a' - a^{\mathsf{det}})^{2}}{(a')^{2}} + \frac{2 \left| a' - a^{\mathsf{det}} \right| }{a'} \right).
	  \end{split}
\end{align}
Using part $\1$ of Lemma~\ref{f-h-main-properties} we obtain that
\[
	\left(\frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} = \ratiomapid\left(\frac{b^{2}}{a^{2}}\right) = \frac{1+\sigma^{2}}{C(\oversamp)}\cdot \frac{b^{2}}{a^{2}} + \frac{\sigma^{2}}{C(\oversamp)} \leq 50^{2} + 1,
\]
where in the last step we use $b/a \leq 50\sqrt{\rho}$. Using inequality~\eqref{condition-help-lemma2-GD-linear} and lower bound of $a'$, we obtain that
\begin{align*}
	\frac{\left| (b')^{2} - (b^{\mathsf{det}})^{2}\right|}{(a')^{2}} &\lesssim (1+b^{2}/a^{2}) \cdot \frac{\sqrt{d}\log^{2}(n)}{n} \lesssim \max\{1,b^{2}/a^{2}\} \cdot \frac{\sqrt{d}\log^{2}(n)}{n}\quad \text{and}\\
	\frac{ \left| a' - a^{\mathsf{det}} \right| }{a'} &\lesssim \sqrt{1+b^{2}/a^{2}} \cdot \sqrt{\frac{\log(n)}{n}} \lesssim \max\{1,b^{2}/a^{2}\} \cdot \sqrt{\frac{\log(n)}{n}}.
\end{align*}
Putting the pieces together yields that
\[
	\left| \left( \frac{b'}{a'} \right)^{2} -\left( \frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} \right| \lesssim \max\{1,b^{2}/a^{2}\} \cdot \frac{\sqrt{d}\log^{2}(n)}{n} +  \max\{1,b/a\} \cdot \sqrt{\frac{\log(n)}{n}}
\]
The desired result follows since $\left(\frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} =\ratiomapid\left(\frac{b^{2}}{a^{2}}\right)$.










































\subsection{Proof of Lemma~\ref{lemma2-good-region} for $\psi(x) = \mathsf{sign}(x)$}
The proof requires the following two lemmas, which are proved at the end of this subsection.

\begin{lemma}\label{f-h-properties-nonlinear}
Let $\parmapbit$ and $\perpmapbit$ be functions in definition~\ref{F-G-definition}.
\renewcommand{\theenumi}{\roman{enumi}}
\begin{enumerate}
	\item There exists a universal positive constants $C_{1}$ such that $| \ratiomapbit'(x) | \leq \frac{C_{1}(1+x^{1.5})}{C(\oversamp)}$ for $x > 0$.
	\item 
		\begin{align*}
			\parmapbit(\parcompX,\perpcompX) \geq \frac{1}{\sqrt{2}\pi} \cdot \frac{\min\{\frac{\parcompX}{\perpcompX},1\}}{(\parcompX^{2} + \perpcompX^{2})^{1/2}},\quad \text{if}\;\;\frac{\parcompX}{\perpcompX} \geq 0.
		\end{align*}
\end{enumerate}
\end{lemma}

\begin{lemma}\label{help-lemma2-GD-nonlinear}
Let $\rho = \frac{C(\oversamp)}{1+\sigma^{2}}$. Suppose $a>0,b\geq0$ and $\frac{b}{a} \leq 50\sqrt{\rho}$. Let $a^{\mathsf{det}} = \parmapbit(a,b)$ and $(b^{\mathsf{det}})^{2} = \perpmapbit(a,b)$. Let $a',b' \in \mathbb{R}$ such that
\begin{align}\label{condition-help-lemma2-GD-nonlinear}
	\left| a' - a^{\mathsf{det}}\right| \lesssim \frac{1}{\sqrt{a^{2}+b^{2}}} \cdot\sqrt{\frac{\log(n)}{n}} \; \text{and} \; \left| (b')^{2} - (b^{\mathsf{det}})^{2}\right| \lesssim \frac{1}{a^{2}+b^{2}}\cdot\frac{\sqrt{d}\log^{2}(n)}{n}.
\end{align}
Then there exists a universal constant $C$ such that for $\oversamp \geq C$ we have that
\[
	\left| \left( \frac{b'}{a'} \right)^{2} - \ratiomapbit\left(\frac{b^{2}}{a^{2}}\right) \right| \lesssim \max\{1,b^{2}/a^{2}\} \cdot \frac{\sqrt{d}\log^{2}(n)}{n} + \max\{1,b/a\} \cdot \sqrt{ \frac{\log(n)}{n}}.
\]
\end{lemma}

\paragraph{Proof of Lemma~\ref{lemma2-good-region} for $\psi(x) = \mathsf{sign}(x)$:}The proof takes two steps.\\
\textbf{First step:} On event $\mathcal{A}_{t+1}$, estimate $\perpcompZ_{t+1}/\parcompZ_{t+1}$.\\
Let $a = \parcompX_{t}$ and $b = \perpcompX_{t}$. By definition, $\parcompZ_{t+1}^{\mathsf{det}} = \parmapbit(a,b)$ and $(\perpcompZ_{t+1}^{\mathsf{det}})^{2}=\perpmapbit(a,b)$. On event $\mathcal{A}_{t+1}$, we obtain that
\[
		\left| \parcompZ_{t+1} - \parcompZ_{t+1}^{\mathsf{det}} \right| \lesssim \frac{1}{\sqrt{a^{2}+b^{2}}} \cdot\sqrt{\frac{\log(n)}{n}} \; \text{and} \; \left| (\perpcompZ_{t+1})^{2} - (\perpcompZ_{t+1}^{\mathsf{det}})^{2}\right| \lesssim \frac{1}{a^{2}+b^{2}}\cdot\frac{\sqrt{d}\log^{2}(n)}{n}.
\]
Using the condition $b/a = \perpcompX_{t}/\parcompX_{t} \leq 50\sqrt{\rho} \lesssim \sqrt{\oversamp}$ and applying Lemma~\ref{help-lemma2-GD-nonlinear} for $a = \parcompX_{t},b = \perpcompX_{t},a' = \parcompZ_{t+1}$ and $b' = \perpcompZ_{t+1}$, we obtain that
\begin{align}\label{ineq1-lemma2-GD-nonlinear}
\begin{split}
	\left| \left( \frac{\perpcompZ_{t+1}}{\parcompZ_{t+1}} \right)^{2} - \ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right| &\lesssim \max\{1,\perpcompX_{t}^{2}/\parcompX_{t}^{2}\} \cdot \frac{\sqrt{d}\log^{2}(n)}{n}+\max\{1,\perpcompX_{t}/\parcompX_{t}\} \cdot \sqrt{\frac{\log(n)}{n}} \\ &\lesssim
	\oversamp \cdot \frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\oversamp} \cdot \sqrt{\frac{\log(n)}{n}}.
\end{split}
\end{align}
Using part $\2$ of Lemma~\ref{f-h-main-properties} yields that
\[
	\ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \leq \max\left\{ \frac{\pi^{2}}{2} \cdot \frac{1}{\rho} \cdot \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}} + \frac{20}{C(\oversamp)}, \frac{50\pi^{2}}{\rho} \right\} \leq C,
\]
where $C$ is some universal constant and in the last step we use $\frac{\perpcompX_{t}}{\parcompX_{t}} \leq 50\sqrt{\rho}$.
Consequently, there exists some universal constant $C_{1}$ such that
\begin{align*}
	\left( \frac{\perpcompZ_{t+1}}{\parcompZ_{t+1}} \right)^{2} &\leq \ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) + C_{1}\oversamp \cdot \frac{\sqrt{d}\log^{2}(n)}{n} + C_{1}\sqrt{\oversamp} \cdot \sqrt{\frac{\log(n)}{n}} \leq C+1.
\end{align*}
\\
\textbf{Second step:} On event $\mathcal{B}_{t+1}$, estimate $\perpcompX_{t+1}/\parcompX_{t+1}$.\\
Let $a = \parcompZ_{t+1}$ and $b = \perpcompZ_{t+1}$. By definition, $\parcompX_{t+1}^{\mathsf{det}} = \parmapbit(a,b)$ and $(\perpcompX_{t+1}^{\mathsf{det}})^{2}=\perpmapbit(a,b)$. On event $\mathcal{B}_{t+1}$, we obtain that
\[
		\left| \parcompX_{t+1} - \parcompX_{t+1}^{\mathsf{det}} \right| \lesssim \frac{1}{\sqrt{a^{2}+b^{2}}} \cdot\sqrt{\frac{\log(n)}{n}} \; \text{and} \; \left| (\perpcompX_{t+1})^{2} - (\perpcompX_{t+1}^{\mathsf{det}})^{2}\right| \lesssim \frac{1}{a^{2}+b^{2}}\cdot\frac{\sqrt{d}\log^{2}(n)}{n}.
\]
Using the condition $b/a = \perpcompZ_{t+1}/\parcompZ_{t+1} \leq \sqrt{C+1}$ and applying Lemma~\ref{help-lemma2-GD-nonlinear} for $a = \parcompZ_{t+1},b = \perpcompZ_{t+1},a' = \parcompX_{t+1}$ and $b' = \perpcompX_{t+1}$, we obtain that
\begin{align}\label{ineq2-lemma2-GD-linear}
\left| \left( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \right)^{2} - \ratiomapbit\left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) \right| \lesssim \frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\frac{\log(n)}{n}}.
\end{align}
We obtain that
\begin{align*}
	&\left| \ratiomapbit\left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) - \ratiomapbit \circ \ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right| \\&\leq \max_{0 \leq \lambda \leq 1}\left| \ratiomapbit'\left( \lambda\cdot \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}} + (1-\lambda)\cdot \ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right)\right| \cdot \left| \left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) -  \ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right| \\&\lesssim 
	\frac{1}{\oversamp} \cdot \left| \left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) -  \ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right|,
\end{align*} 
where in the last step we use part $\1$ of Lemma~\ref{f-h-properties-nonlinear}, $\frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}} \lesssim 1$ and $\ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \lesssim 1$ to obtain that
\[
	\left| \ratiomapbit'\left( \lambda\cdot \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}} + (1-\lambda)\cdot \ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right)\right| \lesssim \frac{1}{C(\oversamp)} \lesssim \frac{1}{\oversamp}.
\]
Now, putting the pieces together yields that
\begin{align*}
	&\left| \left( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \right)^{2} - \ratiomapbit \circ \ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right| \\&\leq
	\left| \left( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \right)^{2} - \ratiomapbit\left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) \right| + 
	\left| \ratiomapbit\left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) - \ratiomapbit \circ \ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right| \\&\lesssim
	\left| \left( \frac{\perpcompX_{t+1}}{\parcompX_{t+1}} \right)^{2} - \ratiomapbit\left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) \right| + 
	\frac{1}{\oversamp} \cdot \left| \left( \frac{\perpcompZ_{t+1}^{2}}{\parcompZ_{t+1}^{2}}\right) -  \ratiomapbit\left( \frac{\perpcompX_{t}^{2}}{\parcompX_{t}^{2}}\right) \right| \\&\lesssim
	\frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\frac{\log(n)}{n}} + \frac{1}{\oversamp} \cdot \left( \oversamp \cdot \frac{\sqrt{d}\log^{2}(n)}{n} + \sqrt{\oversamp} \cdot \sqrt{\frac{\log(n)}{n}} \right) \\&\lesssim
	\frac{\log^{2}(n)}{\sqrt{n}}.
\end{align*}










\subsubsection{Proof of Lemma~\ref{f-h-properties-nonlinear}}
We start with part $\1$. Recall $h_{1}(x)$ and $h_{2}(x)$ from definition~\ref{h1-h2-definition} and $\ratiomapbit(x)$ from definition~\ref{definition-f-h}. By definition, we obtain that
\begin{align}\label{eq1-proof-f-h-properties-nonlinear}
\ratiomapbit(x) = \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{h_{1}(1/\sqrt{x})^{2}} + \frac{1}{C(\oversamp)} \cdot \frac{ \EE\left\{ \frac{W^{4}}{ (C(\oversamp)+W^{2} )^{2} } \right\} }{ \EE\left\{ \frac{W^{2}}{ (C(\oversamp)+W^{2})^{2}} \right\}} \cdot \left( 1 - 2\cdot \frac{h_{2}(1/\sqrt{x})}{h_{1}(1/\sqrt{x})} \right).
\end{align}
Note that 
\[
	\frac{ \EE\left\{ \frac{W^{4}}{ (C(\oversamp)+W^{2} )^{2} } \right\} }{ \EE\left\{ \frac{W^{2}}{ (C(\oversamp)+W^{2})^{2}} \right\}} \leq \EE\{W^{4}\}\bigg/\EE\left\{\frac{W^{2}}{(1+W^{2})^{2}}\right\} \leq 20.
\]
Computing the deriative of $\ratiomapbit(x)$ using equality~\eqref{eq1-proof-f-h-properties-nonlinear}, applying the triangle inequality and using the inequality in the display above yield that
\begin{align}\label{ineq1-h'-onebit-property-proof}
|\ratiomapbit'(x)| \leq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{|h_{1}'(1/\sqrt{x}) \cdot x^{-1.5}|}{h_{1}(1/\sqrt{x})^{3}} + \frac{20}{C(\oversamp)} \cdot \left( \frac{|h_{2}'(1/\sqrt{x}) \cdot x^{-1.5}|}{h_{1}(1/\sqrt{x})} +  \frac{h_{2}(1/\sqrt{x})|h_{1}'(1/\sqrt{x}) \cdot x^{-1.5}|}{h_{1}(1/\sqrt{x})^{2}} \right).
\end{align}
Using Lemma~\ref{lemma1-proof-f-h-main-properties} yields that 
\begin{align}\label{ineq2-h'-onebit-property-proof}
	|h_{1}'(1/\sqrt{x}) \cdot x^{-1.5}| \leq \frac{5x^{-1.5}}{(1+1/x)^{1.5}} \leq 5, \; |h_{2}'(1/\sqrt{x}) \cdot x^{-1.5}| \leq \frac{30x^{-1.5}}{(1+1/x)^{2.5}} \leq 30x\;\text{and}\; h_{2}(x) \leq C. 
\end{align}
Note that $h_{1}(x)$ is a monotone increasing function. So we deduce that $h_{1}(1/\sqrt{x}) \geq h_{1}(1/\sqrt{100})$ for $x \leq 100$. Using Lemma~\ref{lemma1-proof-f-h-main-properties} for $x = 100$ yields that $h(1/\sqrt{100}) \geq 0.1/1.01^{3/2}$. So we conclude that $h_{1}(1/\sqrt{x}) \geq 0.1/1.01^{3/2}$ for $x\leq 100$. Consequently, substituing inequalities~\eqref{ineq2-h'-onebit-property-proof}, $h_{1}(1/\sqrt{x}) \geq 0.1/1.01^{3/2}$ and $h_{2}(x) \leq C$ into inequality~\eqref{ineq1-h'-onebit-property-proof}, we obtain that for $x\leq100$
\[
|\ratiomapbit'(x)| \leq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{5}{(0.1/1.01^{3/2})^{3}} + \frac{20}{C(\oversamp)} \cdot \left( \frac{30x}{0.1/1.01^{3/2}} +  \frac{5C}{(0.1/1.01^{3/2})^{2}} \right) \leq \frac{C_{1}}{C(\oversamp)},
\]
where the last inequality follows since $x\leq100$ and let $C_{1}$ be a large enough constant. Using Lemma~\ref{lemma1-proof-f-h-main-properties} yields that $h_{1}(1/\sqrt{x}) \geq 1/(\sqrt{x}1.01^{1.5})$ for $x\geq 100$. Consequently, we obtain that for $x\geq 100$,
\[
|\ratiomapbit'(x)| \leq \frac{\pi^{2}}{4} \cdot \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{5}{(1/(\sqrt{x}1.01^{1.5}))^{3}} + \frac{20}{C(\oversamp)} \cdot \left( \frac{30x}{1/(\sqrt{x}1.01^{1.5})} +  \frac{5C}{(1/(\sqrt{x}1.01^{1.5}))^{2}} \right) \leq \frac{C_{1}x^{1.5}}{C(\oversamp)}.
\]
Putting the pieces together yields that $|h'(x)| \leq C_{1}(1+x^{1.5})/C(\oversamp)$ for $x>0$. We next prove part $\2$. Using definition~\ref{h1-h2-definition} and definition~\ref{F-G-definition}, we obtain that
\[
	\parmapbit(\parcompX,\perpcompX) = \frac{2}{\pi} \cdot (\parcompX^{2} + \perpcompX^{2})^{-1/2} \cdot h_{1}(\parcompX/\perpcompX).
\]
If $\parcompX/\perpcompX \geq 1$,then using the monotone increasing of $h_{1}(x)$ yields
\[
	h_{1}(\parcompX/\perpcompX) \geq h_{1}(1) \geq 2^{-1.5},
\] 
where the last step follows from Lemma~\ref{lemma1-proof-f-h-main-properties}. Consequently, we obtain that
\[
	\parmapbit(\parcompX,\perpcompX) \geq \frac{1}{\sqrt{2}\pi} \cdot (\parcompX^{2} + \perpcompX^{2})^{-1/2}, \quad \text{if}\;\frac{\parcompX}{\perpcompX} \geq 1.
\]
If $0 \leq \parcompX/\perpcompX \leq 1$, then using Lemma~\ref{lemma1-proof-f-h-main-properties} yields that
\[
	h_{1}(\parcompX/\perpcompX) \geq \frac{\parcompX/\perpcompX}{(1+\parcompX^{2}/\perpcompX^{2})^{1.5}} \geq \parcompX/\perpcompX \cdot 2^{-1.5},
\]
where in the last step we use $\parcompX/\perpcompX \leq 1$. Consequently, we obtain that
\[
	\parmapbit(\parcompX,\perpcompX) \geq \frac{1}{\sqrt{2}\pi} \cdot (\parcompX^{2} + \perpcompX^{2})^{-1/2} \cdot \frac{\parcompX}{\perpcompX}, \quad \text{if}\;0\leq\frac{\parcompX}{\perpcompX} \leq 1.
\]
To this end, we conclude that
\[
	\parmapbit(\parcompX,\perpcompX) \geq \frac{1}{\sqrt{2}\pi} \cdot (\parcompX^{2} + \perpcompX^{2})^{-1/2} \cdot \min\{\frac{\parcompX}{\perpcompX},1\}\quad \text{if}\;\frac{\parcompX}{\perpcompX} \geq 0.
\]


\subsubsection{Proof of Lemma~\ref{help-lemma2-GD-nonlinear}}
Using inequality~\eqref{condition-help-lemma2-GD-nonlinear} yields that
\begin{align*}
	a' &\geq \parmapbit(a,b) - \frac{C_{1}}{\sqrt{a^{2}+b^{2}}} \cdot\sqrt{\frac{\log(d)}{\oversamp \cdot d}} \geq 
	 \frac{1}{\sqrt{2}\pi} \cdot \frac{\min\{\frac{a}{b},1\}}{\sqrt{a^{2} + b^{2}}} - \frac{C_{1}}{\sqrt{a^{2}+b^{2}}} \cdot\sqrt{\frac{\log(d)}{\oversamp \cdot d}} \\&=
	\frac{1}{\sqrt{a^{2}+b^{2}}}\cdot \left( \frac{\min\{\frac{a}{b},1\}}{\sqrt{2}\pi}   - C_{1}\sqrt{\frac{\log(d)}{\oversamp \cdot d}} \right) \geq  \frac{1}{\sqrt{a^{2}+b^{2}}} \cdot  \frac{\min\{\frac{a}{b},1\}}{2\pi},
\end{align*}
where $C_{1}$ is some universal constant and in the last step we use $\frac{a}{b} \gtrsim \frac{1}{\sqrt{\oversamp}}$ since $b/a\leq50\sqrt{\rho} \lesssim \sqrt{\oversamp}$.
Using the triangle inequality yields that
\begin{align}\label{ineq1-help-lemma2-GD-nonlinear}
	\begin{split}
		\left| \left( \frac{b'}{a'} \right)^{2} -\left( \frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} \right| &\leq \frac{\left| (b')^{2} - (b^{\mathsf{det}})^{2}\right|}{(a')^{2}} + 
		\left| \left( \frac{b^{\mathsf{det}}}{a'} \right)^{2} -\left( \frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} \right| \\&=
		\frac{\left| (b')^{2} - (b^{\mathsf{det}})^{2}\right|}{(a')^{2}} + \left(\frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} \cdot
		  \frac{\left| (a')^{2} - (a^{\mathsf{det}})^{2}\right|}{(a')^{2}} \\&\leq
		\frac{\left| (b')^{2} - (b^{\mathsf{det}})^{2}\right|}{(a')^{2}} + \left(\frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} \cdot
		  \left( \frac{ (a' - a^{\mathsf{det}})^{2}}{(a')^{2}} + \frac{2 \left| a' - a^{\mathsf{det}} \right| }{a'} \right).
	  \end{split}
\end{align}
Using Lemma~\ref{f-h-main-properties} we obtain that
\[
	\left(\frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} = \ratiomapbit\left(\frac{b^{2}}{a^{2}}\right) \leq \max\left\{ \frac{\pi^{2}}{2} \cdot \frac{1}{\rho} \cdot \frac{b^{2}}{a^{2}} + \frac{20}{C(\oversamp)}, \frac{50\pi^{2}}{\rho} \right\} \leq C,
\]
where $C$ is some universal constant and in the last step we use $b/a \leq 50\sqrt{\rho}$. Using inequality~\eqref{condition-help-lemma2-GD-nonlinear} and the lower bound of $a'$, we obtain that
\begin{align*}
	\frac{\left| (b')^{2} - (b^{\mathsf{det}})^{2}\right|}{(a')^{2}} &\lesssim \max\{1,b^{2}/a^{2}\} \cdot \frac{\sqrt{d}\log^{2}(n)}{n} \quad \text{and}\\
	\frac{ \left| a' - a^{\mathsf{det}} \right| }{a'} &\lesssim \max\{1,b/a\} \cdot \sqrt{\frac{\log(n)}{n}}
\end{align*}
Putting the pieces together yields that
\[
	\left| \left( \frac{b'}{a'} \right)^{2} -\left( \frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} \right| \lesssim \max\{1,b^{2}/a^{2}\} \cdot \frac{\sqrt{d}\log^{2}(n)}{n} +  \max\{1,b/a\} \cdot \sqrt{\frac{\log(n)}{n}}
\]
The desired result follows since $\left(\frac{b^{\mathsf{det}}}{a^{\mathsf{det}}}\right)^{2} =\ratiomapid\left(\frac{b^{2}}{a^{2}}\right)$.


































\subsection{Proof of Lemma~\ref{lemma2-initialization-linear}}

To reduce the notational burden, let $\rho = \frac{C(\oversamp)}{1+\sigma^{2}}$, $r_{t} = \frac{\perpcompX_{t}}{\parcompX_{t}}$, $\Delta_{1} = \sqrt{\frac{\log d}{\oversamp \cdot d}}$ and $\Delta_{2} = \frac{\log^{2}(d)}{\oversamp \cdot \sqrt{d}}$. The proof takes two steps.\\
\textbf{First Step:} On event $\mathcal{A}_{t+1}$, estimate $\parcompZ_{t+1}$ and $\perpcompZ_{t+1}$.\\
By definition, $\parcompZ_{t+1}^{\mathsf{det}} = \parmapid(\parcompX_{t},\perpcompX_{t})$ and $(\perpcompZ_{t+1}^{\mathsf{det}})^{2} = \perpmapid(\parcompX_{t},\perpcompX_{t})$. Using definition~\ref{F-G-definition}, we obtain that
\[
	\parcompZ_{t+1}^{\mathsf{det}} = \frac{\parcompX_{t}}{\parcompX_{t}^{2} + \perpcompX_{t}^{2}}\quad \text{and} \quad (\perpcompZ_{t+1}^{\mathsf{det}})^{2} = \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{\perpcompX_{t}^{2}}{(\parcompX_{t}^{2} + \perpcompX_{t}^{2})^{2}} + \frac{\sigma^{2}}{C(\oversamp)} \cdot  \frac{\parcompX_{t}^{2}}{(\parcompX_{t}^{2} + \perpcompX_{t}^{2})^{2}}.
\]
Consequently, we obtain that
\begin{align}\label{ineq1-lemma1-initia-linear-proof}
	(1-1/r_{t}^{2}) \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} \leq \parcompZ_{t+1}^{\mathsf{det}} \leq \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} \quad \text{and} \quad 
	\rho^{-1} \cdot  \perpcompX_{t}^{-2} \cdot (1+1/r_{t}^{2})^{-2} \leq (\perpcompZ_{t+1}^{\mathsf{det}})^{2} \leq \rho^{-1} \cdot  \perpcompX_{t}^{-2}.
\end{align}
On event $\mathcal{A}_{t+1}$ and using $\parcompX_{t}^{2} + \perpcompX_{t}^{2} \geq 0.5$, we obtain that
\begin{align}\label{ineq2-lemma1-initia-linear-proof}
	\left| \parcompZ_{t+1} - \parcompZ_{t+1}^{\mathsf{det}} \right| \leq C_{1} \cdot \Delta_{1} \quad \text{and} \quad \left| \perpcompZ_{t+1}^{2} - (\perpcompZ_{t+1}^{\mathsf{det}})^{2} \right| \leq C_{1} \cdot \Delta_{2}.
\end{align}\\
\textbf{Second step:} On event $\mathcal{B}_{t+1}$, estimate $\parcompX_{t+1}$ and $\perpcompX_{t+1}$.\\
Using inequalities~\eqref{ineq1-lemma1-initia-linear-proof} and~\eqref{ineq2-lemma1-initia-linear-proof} yields that
\begin{align}\label{ineq3-lemma1-initia-linear-proof}
\begin{split}
	\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2} &\leq (\parcompX_{t}/\perpcompX_{t}^{2} + C_{1}\Delta_{1})^{2} + \rho^{-1} \cdot  \perpcompX_{t}^{-2} + C_{1}\Delta_{2} \\ &\overset{\1}{\leq} 2\parcompX_{t}^{2}\perpcompX_{t}^{-4}  + 2C_{1}^{2}\Delta_{1}^{2} + \rho^{-1} \cdot  \perpcompX_{t}^{-2}  + C_{1}\Delta_{2} \\&\leq 
	\perpcompX_{t}^{-2} \cdot (\rho^{-1} + 2/r_{t}^{2}) + 2C_{1}^{2}\Delta_{1}^{2} + C_{1}\Delta_{2} \quad \text{and} \\
	\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2} &\geq \perpcompX_{t}^{-2} \cdot \rho^{-1} \cdot 1/(1+1/r_{t}^{2})^{2} - C_{1}\Delta_{2},
\end{split}
\end{align} 
where in step $\1$ we use $(a+b)^{2} \leq 2a^{2} + 2b^{2}$. By definition, we obtain that
\begin{align}\label{eq1-lemma1-initia-linear-proof}
	\parcompX_{t+1}^{\mathsf{det}} = \frac{\parcompZ_{t+1}}{\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2}}\quad \text{and} \quad (\perpcompX_{t+1}^{\mathsf{det}})^{2} = \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{\perpcompZ_{t+1}^{2}}{(\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2})^{2}} + \frac{\sigma^{2}}{C(\oversamp)} \cdot  \frac{\parcompZ_{t+1}^{2}}{(\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2})^{2}}.
\end{align}
Now, using inequalities~\eqref{ineq1-lemma1-initia-linear-proof},~\eqref{ineq2-lemma1-initia-linear-proof} and~\eqref{ineq3-lemma1-initia-linear-proof} yields that
\[
	\parcompX_{t+1}^{\mathsf{det}} \geq \frac{\parcompX_{t}\perpcompX_{t}^{-2}(1-r_{t}^{-2}) - C_{1}\Delta_{1}}{\perpcompX_{t}^{-2} \cdot (\rho^{-1} + 2/r_{t}^{2}) + 2C_{1}^{2}\Delta_{1}^{2} + C_{1}^{2}\Delta_{2}} = \frac{\parcompX_{t}(1-r_{t}^{-2}) - C_{1}\Delta_{1}\perpcompX_{t}^{2}}{(\rho^{-1} + 2/r_{t}^{2}) + \perpcompX_{t}^{2} \cdot (2C_{1}^{2}\Delta_{1}^{2} + C_{1}^{2}\Delta_{2})}.
\]
Using $\parcompX_{t} \geq 1/(50\sqrt{d})$, $\perpcompX_{t}^{2} \leq 2$, $r_{t}^{2} \geq 20\rho$ and $\Lambda \geq C\log d$ yields 
\[
	\parcompX_{t}(1-r_{t}^{-2}) - C_{1}\Delta_{1}\perpcompX_{t}^{2} \geq 0.5 \cdot \parcompX_{t}.
\]
Using $\perpcompX_{t}^{2} \leq 2$ and $r_{t}^{2} \geq 20\rho$ yields that
\[
	(\rho^{-1} + 2/r_{t}^{2}) + \perpcompX_{t}^{2} \cdot (2C_{1}^{2}\Delta_{1}^{2} + C_{1}^{2}\Delta_{2}) \leq 2\rho^{-1}.
\]
Putting the pieces together yields that $\parcompX_{t+1}^{\mathsf{det}} \geq \frac{\rho}{4} \cdot \parcompX_{t}.$ Similarly, using inequalities~\eqref{ineq1-lemma1-initia-linear-proof},~\eqref{ineq2-lemma1-initia-linear-proof} and~\eqref{ineq3-lemma1-initia-linear-proof} yields that
\[
	\parcompX_{t+1}^{\mathsf{det}} \leq \frac{\parcompX_{t} \perpcompX_{t}^{-2} + C_{1} \Delta_{1}}{ \rho^{-1} \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-2} - C_{1}\Delta_{2}} = 
	\frac{\parcompX_{t} + C_{1}\Delta_{1}\perpcompX_{t}^{2} }{ \rho^{-1} \cdot (1+r_{t}^{-2})^{-2} - C_{1}\Delta_{2}\perpcompX_{t}^{2}}.
\]
Using $\parcompX_{t} \geq 1/(50\sqrt{d})$, $\perpcompX_{t}^{2} \leq 2$, and $\Lambda \geq C\log d$ yields 
\[
	\parcompX_{t} + C_{1}\Delta_{1}\perpcompX_{t}^{2} \leq 2 \parcompX_{t}.
\]
Using $\perpcompX_{t}^{2} \leq 2$ and $r_{t}^{2} \geq 20\rho$ yields that
\[
	\rho^{-1} \cdot (1+r_{t}^{-2})^{-2} - C_{1}\Delta_{2}\perpcompX_{t}^{2} \geq 0.5 \cdot \rho^{-1}.
\]
Putting the pieces together yields that $\parcompX_{t+1}^{\mathsf{det}} \leq 4\rho \cdot \parcompX_{t}$. To this end, we have obtained that
\begin{align}\label{ineq4-lemma1-initia-linear-proof}
 \frac{\rho}{4} \cdot \parcompX_{t} \leq \parcompX_{t+1}^{\mathsf{det}} \leq 4\rho \cdot \parcompX_{t}.
\end{align}
Now we start to bound $\perpcompX_{t+1}^{\mathsf{det}}$. Let $\widetilde{r}_{t+1} = \perpcompZ_{t+1}/\parcompZ_{t+1}$. Using equality~\eqref{eq1-lemma1-initia-linear-proof}, we obtain that
\[
	\rho^{-1} \cdot \perpcompZ_{t+1}^{-2} \cdot (1+\widetilde{r}_{t+1}^{-2})^{-2} \leq (\perpcompX_{t+1}^{\mathsf{det}})^{2} \leq \rho^{-1} \cdot \perpcompZ_{t+1}^{-2}.
\]
Now using inequalities~\eqref{ineq1-lemma1-initia-linear-proof} and~\eqref{ineq2-lemma1-initia-linear-proof}, we obtain that
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} &\geq \rho^{-1} \cdot \perpcompZ_{t+1}^{-2} \cdot (1+\widetilde{r}_{t+1}^{-2})^{-2} \\ &=
	\frac{1}{\rho} \cdot  \frac{1}{\rho^{-1} \cdot \perpcompX_{t}^{-2} + C_{1}\Delta_{2} } \cdot \frac{1}{(1+\widetilde{r}_{t+1}^{-2})^{2}} \\&=
	\perpcompX_{t}^{2} \cdot (1+C_{1}\Delta_{2} \cdot \rho \cdot \perpcompX_{t}^{2})^{-1} \cdot (1+\widetilde{r}_{t+1}^{-2})^{-2} \\&\geq
	\perpcompX_{t}^{2} \cdot (1-C_{1}\Delta_{2} \cdot \rho \cdot \perpcompX_{t}^{2}) \cdot (1-2\widetilde{r}_{t+1}^{-2}),
\end{align*} 
where in the last step we use $(1+a)^{-1}\geq 1-a$ and $(1+a)^{-2} \geq (1-2a)$. Continuing, using $\perpcompZ_{t+1}^{2} \geq \rho^{-1}\perpcompX_{t}^{-2}(1+r_{t}^{-2})^{2} - C_{1}\Delta_{2} \geq 0.5 \rho^{-1} \perpcompX_{t}^{-2}$ and $\parcompZ_{t+1}^{2} \leq 2\parcompX_{t}^{2}\perpcompX_{t}^{-4}+2C_{1}^{2}\Delta_{1}^{2}\leq 3\parcompX_{t}^{2}\perpcompX_{t}^{-4}$ yields that $\widetilde{r}_{t+1}^{2} \geq (6\rho)^{-1}r_{t}^{2}$. Putting the pieces together yields that
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} &\geq \perpcompX_{t}^{2} \cdot (1-C_{1}\Delta_{2} \cdot \rho \cdot \perpcompX_{t}^{2}) \cdot (1-2\widetilde{r}_{t+1}^{-2}) \\&\geq
	\perpcompX_{t}^{2} \cdot (1-2C_{1}\Delta_{2} \cdot \rho) \cdot (1-12\rho r_{t}^{-2}) \\&\geq
	\perpcompX_{t}^{2} \cdot (1-2C_{1}\Delta_{2}\rho -12 \rho r_{t}^{-2}) \\&\geq
	\perpcompX_{t}^{2} - 12\rho \parcompX_{t}^{2}-C_{1}'\frac{\log^{2}(d)}{\sqrt{d}},
\end{align*}
where in the last step we use $\perpcompX_{t}^{2} \cdot r_{t}^{-2} = \parcompX_{t}^{2}$ and $2C_{1}\Delta_{2}\rho =\frac{2C_{1}\log^{2}(d)}{\oversamp \cdot \sqrt{d}} \cdot \frac{C(\oversamp)}{1+\sigma^{2}} \leq \frac{2C_{1}'\log^{2}(d)}{\sqrt{d}}$ for some universal contant $C_{1}'$ since $\oversamp \asymp C(\oversamp)$. Similarly, we obtain that 
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} &\leq \rho^{-1} \cdot \perpcompZ_{t+1}^{-2} \leq \rho^{-1} \cdot (\rho^{-1}\perpcompX_{t}^{-2}(1+r_{t}^{-2})^{-2} - C_{1}\Delta_{2})^{-1} \\ &=
	\frac{\perpcompX_{t}^{2} \cdot (1+r_{t}^{-2})^{2}}{1-C_{1}\rho \Delta_{2} \perpcompX_{t}^{2} (1+r_{t}^{-2})^{2}} \\&\leq
	\perpcompX_{t}^{2} \cdot (1+r_{t}^{-2})^{2} \cdot (1+2C_{1}\rho \Delta_{2} \perpcompX_{t}^{2} (1+r_{t}^{-2})^{2}),
\end{align*}
where in the last step we use $(1-a)^{-1} \leq 1+2a$ for $0\leq a \leq 0.5$ and let $a = C_{1}\rho \Delta_{2} \perpcompX_{t}^{2} (1+r_{t}^{-2})^{2} \leq 0.5$. Continuing, using $r_{t}^{2}\geq 20 \rho$ and $\perpcompX_{t}^{2} \leq 2$ yields that
\[
	2C_{1}\rho \Delta_{2} \perpcompX_{t}^{2} (1+r_{t}^{-2})^{2} \leq 8C_{1} \cdot \frac{C(\oversamp)}{1+\sigma^{2}} \cdot \frac{\log^{2}(d)}{\oversamp \cdot \sqrt{d}} \leq \frac{C_{1}'\log^{2}(d)}{\sqrt{d}}.
\]
Consequently, we obtain that
\[
	(1+r_{t}^{-2})^{2} \cdot (1+2C_{1}\rho \Delta_{2} \perpcompX_{t}^{2} (1+r_{t}^{-2})^{2})\leq (1+3r_{t}^{-2})(1+\frac{C_{1}'\log^{2}(d)}{\sqrt{d}}) \leq 1+3r_{t}^{-2}+\frac{C_{1}''\log^{2}(d)}{\sqrt{d}},
\]
for some universal constant $C_{1}''$. Putting the pieces together yields that
\[
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} \leq \perpcompX_{t}^{2} \cdot (1+3r_{t}^{-2}+\frac{C_{1}''\log^{2}(d)}{\sqrt{d}}) \leq \perpcompX_{t}^{2} + 3\parcompX_{t}^{2} + \frac{2C_{1}''\log^{2}(d)}{\sqrt{d}}.
\]
To this end, we have obtained that
\begin{align}\label{ineq5-lemma1-initia-linear-proof}
	\perpcompX_{t}^{2} - 12\rho \parcompX_{t}^{2}-C_{1}'\frac{\log^{2}(d)}{\sqrt{d}} \leq (\perpcompX_{t+1}^{\mathsf{det}})^{2} \leq \perpcompX_{t}^{2} + 3\parcompX_{t}^{2} + \frac{2C_{1}''\log^{2}(d)}{\sqrt{d}}.
\end{align}
On event $\mathcal{B}_{t+1}$ and using $\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2} \geq \perpcompX_{t}^{-2} \cdot \rho^{-1} \cdot 1/(1+1/r_{t}^{2})^{2} - C_{1}\Delta_{2} \geq \rho^{-1}/4$, we obtain that
\begin{align*}
	\left| \parcompZ_{t+1} - \parcompZ_{t+1}^{\mathsf{det}} \right| \leq C_{1} \cdot \left( \parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2} \right)^{-1/2} \cdot \Delta_{1} \leq \frac{C_{1}'\log d}{\sqrt{d}} \quad \text{and}\\
	\left| \perpcompZ_{t+1}^{2}  - (\perpcompZ_{t+1}^{\mathsf{det}})^{2} \right| \leq C_{1} \cdot \left( \parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2} \right)^{-1} \cdot \Delta_{2} \leq \frac{C_{1}'\log^{2}(d)}{\sqrt{d}}
\end{align*}
Combining with inequalities~\eqref{ineq4-lemma1-initia-linear-proof} and~\eqref{ineq5-lemma1-initia-linear-proof}, we obtain that
\begin{align*}
	\parcompZ_{t+1} &\leq \parcompZ_{t+1}^{\mathsf{det}} + \frac{C_{1}'\log d}{\sqrt{d}} \leq 4\rho \cdot \parcompX_{t} + \frac{C_{1}'\log d}{\sqrt{d}} \leq 5\rho \cdot \parcompX_{t}, \\
	\parcompZ_{t+1} &\geq \parcompZ_{t+1}^{\mathsf{det}} - \frac{C_{1}'\log d}{\sqrt{d}} \geq \rho/4 \cdot \parcompX_{t} - \frac{C_{1}'\log d}{\sqrt{d}} \geq \rho/5 \cdot \parcompX_{t},\\
	\perpcompZ_{t+1}^{2} &\leq (\perpcompZ_{t+1}^{\mathsf{det}})^{2} + \frac{C_{1}'\log^{2}(d)}{\sqrt{d}} \leq \perpcompX_{t}^{2} + 3\parcompX_{t}^{2} + \frac{C_{1}''\log^{2}(d)}{\sqrt{d}}\quad \text{and}\\
	\perpcompZ_{t+1}^{2} &\geq (\perpcompZ_{t+1}^{\mathsf{det}})^{2} - \frac{C_{1}'\log^{2}(d)}{\sqrt{d}} \geq \perpcompX_{t}^{2} - 12\rho \parcompX_{t}^{2}-C_{1}''\frac{\log^{2}(d)}{\sqrt{d}}.
\end{align*}








































\subsection{Proof of Lemma~\ref{lemma2-initialization-nonlinear}}
To reduce the notational burden, let $\rho = \frac{C(\oversamp)}{1+\sigma^{2}}$, $r_{t} = \frac{\perpcompX_{t}}{\parcompX_{t}}$, $\Delta_{1} = \sqrt{\frac{\log d}{\oversamp \cdot d}}$ and $\Delta_{2} = \frac{\log^{2}(d)}{\oversamp \cdot \sqrt{d}}$. The proof takes two steps.\\
\textbf{First Step:} On event $\mathcal{A}_{t+1}$, estimate $\parcompZ_{t+1}$ and $\perpcompZ_{t+1}$.\\
By definition, we obtain that $\parcompZ_{t+1}^{\mathsf{det}} = \parmapbit(\parcompX_{t},\perpcompX_{t})$ and $(\perpcompZ_{t+1}^{\mathsf{det}})^{2} = \perpmapbit(\parcompX_{t},\perpcompX_{t})$. Using definition~\ref{F-G-definition}, we obtain that
\begin{align}\label{eq1-lemma1-init-nonlinear-proof}
	\begin{split}
		\parcompZ_{t+1}^{\mathsf{det}} &= \frac{2}{\pi} \cdot \frac{1}{\sqrt{\parcompX_{t}^{2} + \perpcompX_{t}^{2}}} \cdot \EE\left\{ \frac{|W| \cdot \int_{0}^{\frac{\parcompX_{t}}{\perpcompX_{t}} \cdot |W|}  e^{-t^{2}/2} dt}{C(\oversamp) + W^{2}} \right\}  \bigg/  \EE\left\{ \frac{W^{2}}{C(\oversamp) + W^{2}}\right\} \;\; \text{ and } \;\; \\
		(\perpcompZ_{t+1}^{\mathsf{det}})^{2} &= \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2} + \perpcompX_{t}^{2}} + \frac{(\parcompZ_{t+1}^{\mathsf{det}})^{2}}{C(\oversamp)}  \cdot \EE\left\{ \frac{W^{4}}{(C(\oversamp) + W^{2})^{2}} \right\} \bigg/ \EE\left\{ \frac{W^{2}}{(C(\oversamp) + W^{2})^{2}}\right\} 
		\\&- \frac{4}{\pi} \cdot \frac{\parcompZ_{t+1}^{\mathsf{det}}}{C(\oversamp)\sqrt{\parcompX_{t}^{2} + \perpcompX_{t}^{2}}} \cdot \EE\left\{ \frac{|W|^{3} \cdot \int_{0}^{\frac{\parcompX_{t}}{\perpcompX_{t}} \cdot |W|}  e^{-t^{2}/2} dt}{(C(\oversamp) + W^{2})^{2}} \right\}  \bigg/ \EE\left\{  \frac{W^{2}}{(C(\oversamp) + W^{2})^{2}} \right\}.
	\end{split}
\end{align}
Using $\int_{0}^{\frac{\parcompX_{t}}{\perpcompX_{t}} \cdot |W|}  e^{-t^{2}/2} dt \leq \frac{\parcompX_{t}}{\perpcompX_{t}} \cdot |W|$ yields that
\[
	\parcompZ_{t+1}^{\mathsf{det}} \leq \frac{2}{\pi} \cdot \frac{1}{\sqrt{\parcompX_{t}^{2} + \perpcompX_{t}^{2}}} \cdot  \frac{\parcompX_{t}}{\perpcompX_{t}} \leq \frac{2}{\pi} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}}.
\]
Applying part $\2$ of Lemma~\ref{f-h-properties-nonlinear} since $\parcompX_{t}/\perpcompX_{t} \leq 1$ yields that
\[
	\parcompZ_{t+1}^{\mathsf{det}} \geq \frac{1}{\sqrt{2\pi}} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}} \cdot \frac{1}{\sqrt{\parcompX_{t}^{2} + \perpcompX_{t}^{2}}} = \frac{1}{\sqrt{2\pi}} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} \cdot \frac{1}{(1 + r_{t}^{-2})^{1/2}}.
\]
Now we turn to bound $(\perpcompZ_{t+1}^{\mathsf{det}})^{2}$. Note that for $W\sim \mathcal{N}(0,1)$,
\[
	\EE\left\{ \frac{W^{4}}{(C(\oversamp) + W^{2})^{2}} \right\} \bigg/ \EE\left\{ \frac{W^{2}}{(C(\oversamp) + W^{2})^{2}}\right\} \leq \EE\{W^{4}\} \bigg/ \EE\left\{ \frac{W^{2}}{(1 + W^{2})^{2}}\right\} \leq 20.
\] 
Using equality~\eqref{eq1-lemma1-init-nonlinear-proof} and the upper bound of $\parcompZ_{t+1}^{\mathsf{det}}$ yields that 
\begin{align*}
	(\perpcompZ_{t+1}^{\mathsf{det}})^{2} &\leq \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} + \frac{20(\parcompZ_{t+1}^{\mathsf{det}})^{2}}{C(\oversamp)} \leq 
	\frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} + \frac{20}{C(\oversamp)} \cdot \frac{4}{\pi^{2}} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}}\cdot \frac{\parcompX_{t}^{2}}{\perpcompX_{t}^{2}} \\&\leq \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} \cdot (1+9r_{t}^{-2})\;\;\text{and}\\
	(\perpcompZ_{t+1}^{\mathsf{det}})^{2} &\geq  \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} - \frac{4}{\pi} \cdot \frac{\parcompZ_{t+1}^{\mathsf{det}}}{C(\oversamp)\sqrt{\parcompX_{t}^{2} + \perpcompX_{t}^{2}}} \cdot 20 \geq \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} - \frac{160}{\pi^{2}C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2} + \perpcompX_{t}^{2}} \cdot \frac{\parcompX_{t}^{2}}{\perpcompX_{t}^{2}} \\&\geq\frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} \cdot (1-18r_{t}^{-2}).
\end{align*}
To this end, we have obtained
\begin{align}\label{ineq1-lemma1-init-nonlinear-proof}
	\frac{1}{\sqrt{2\pi}} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} \cdot \frac{1}{(1 + r_{t}^{-2})^{1/2}} \leq \parcompZ_{t+1}^{\mathsf{det}} \leq \frac{2}{\pi} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}}\;\;\text{and}\;\; 
	\frac{1}{\rho} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} \cdot (1-18r_{t}^{-2}) \leq (\perpcompZ_{t+1}^{\mathsf{det}})^{2} \leq \frac{1}{\rho} \cdot \frac{1}{\parcompX_{t}^{2}+\perpcompX_{t}^{2}} \cdot (1+9r_{t}^{-2})
\end{align}
On event $\mathcal{A}_{t+1}$, using $\parcompX_{t}^{2} + \perpcompX_{t}^{2} \geq 0.5$ yields that
\begin{align}\label{ineq2-lemma1-init-nonlinear-proof}
	\left| \parcompZ_{t+1} - \parcompZ_{t+1}^{\mathsf{det}}\right| \leq C_{1}\Delta_{1} \quad \text{and} \quad \left| \perpcompZ_{t+1}^{2} - (\perpcompZ_{t+1}^{\mathsf{det}})^{2} \right| \leq C_{1}\Delta_{2},
\end{align}
where $C_{1}$ is some universal constant.\\
\textbf{Second step:} On event $\mathcal{B}_{t+1}$, estimate $\parcompX_{t+1}$ and $\perpcompX_{t+1}$.\\
We start with the upper bound of $\parcompX_{t+1}^{\mathsf{det}}$. By definition, $\parcompX_{t+1}^{\mathsf{det}} = \parmapbit(\parcompZ_{t+1},\perpcompZ_{t+1})$. Using definition of $\parmapbit$, we obtain that
\begin{align}\label{ineq2.5-lemma1-init-nonlinear-proof}
	\parcompX_{t+1}^{\mathsf{det}} = \frac{2}{\pi} \cdot \frac{1}{\sqrt{\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2}}} \cdot \frac{\EE\left\{ \frac{|W| \cdot \int_{0}^{\frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}} \cdot |W|}  e^{-t^{2}/2} dt}{C(\oversamp) + W^{2}} \right\}}{\EE\left\{ \frac{W^{2}}{C(\oversamp) + W^{2}}\right\}} \leq \frac{2}{\pi} \cdot \frac{1}{\sqrt{\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2}}} \cdot \frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}} \leq \frac{2}{\pi} \cdot \frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}^{2}}. 
\end{align}
Using inequalities~\eqref{ineq1-lemma1-init-nonlinear-proof} and~\eqref{ineq2-lemma1-init-nonlinear-proof}, we obtain that
\begin{align}\label{ineq3-lemma1-init-nonlinear-proof}
	\parcompZ_{t+1} &\leq \frac{2}{\pi} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} + C_{1}\cdot \Delta_{1} \overset{\1}{\leq} \frac{3}{\pi} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} \quad \text{and}\\
	\perpcompZ_{t+1}^{2} &\geq \rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-1} \cdot (1-18r_{t}^{-2}) - C_{1}\Delta_{2} \overset{\2}{\geq} 0.5\cdot \rho^{-1}\cdot \perpcompX_{t}^{-2},
\end{align}
where in step $\1$ we use $\parcompX_{t} \geq 1/(50\sqrt{d})$, $\perpcompX_{t}^{2}\leq2$, $\Delta_{1} \asymp \sqrt{\log d}/\sqrt{\oversamp \cdot d}$ and $\oversamp \geq C\log d$, and in step $\2$ we use $r_{t}^{2} \geq 50 \rho$, $\rho \asymp \oversamp$ and $\Delta_2 \asymp \log^{2}(d)/(\oversamp \cdot \sqrt{d})$. Putting the pieces together yields that
\[
	\parcompX_{t+1}^{\mathsf{det}} \leq \frac{2}{\pi} \cdot \frac{\frac{3}{\pi} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}}}{0.5\cdot \rho^{-1}\cdot \perpcompX_{t}^{-2}} \leq 2\rho \cdot \parcompX_{t}.
\]
We next derive the lower bound of $\parcompX_{t+1}^{\mathsf{det}}$. Let $\widetilde{r}_{t+1} = \parcompZ_{t+1}/\perpcompZ_{t+1}$. Using inequality~\eqref{ineq3-lemma1-init-nonlinear-proof} yields that
\[
	\widetilde{r}_{t+1} \geq \frac{\left(0.5\cdot \rho^{-1}\cdot \perpcompX_{t}^{-2}\right)^{1/2}}{\frac{3}{\pi} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}}} \geq \frac{\pi}{6} \cdot \rho^{-1/2} \cdot r_{t}.
\]
Since $r_{t}\geq \sqrt{20\rho}$, we obtain that $\widetilde{r}_{t+1} \geq 1$. Using part $\2$ of Lemma~\ref{f-h-properties-nonlinear} with $\frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}} = 1/\widetilde{r}_{t+1} \leq 1$ yields that 
\begin{align}\label{ineq3.5-lemma1-init-nonlinear-proof}
	\parcompX_{t+1}^{\mathsf{det}} \geq \frac{1}{\sqrt{2\pi}}\cdot \frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}} \cdot \frac{1}{(\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2})^{1/2}} = \frac{1}{\sqrt{2\pi}}\cdot \frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}^{2}} \cdot \frac{1}{(1+\widetilde{r}_{t+1}^{-2})^{1/2}} \geq \frac{1}{2\sqrt{\pi}} \cdot \frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}^{2}}.
\end{align}
Using inequalities~\eqref{ineq1-lemma1-init-nonlinear-proof} and~\eqref{ineq2-lemma1-init-nonlinear-proof}, we obtain that
\begin{align}\label{ineq4-lemma1-init-nonlinear-proof}
	\parcompZ_{t+1} &\geq \frac{1}{\sqrt{2\pi}} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} \cdot \frac{1}{(1 + r_{t}^{-2})^{1/2}} - C_{1}\Delta_{1} \overset{\1}{\geq} \frac{1}{4\sqrt{\pi}} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}}\quad \text{and}\\
	\perpcompZ_{t+1}^{2} &\leq \rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-1} \cdot (1+9r_{t}^{-2}) + C_{1}\Delta_{2} \overset{\2}{\leq} 2\rho^{-1} \cdot \perpcompX_{t}^{-2},
\end{align}
where in step $\1$ and step $\2$ we use $\parcompX_{t} \geq 1/(50\sqrt{d})$, $\perpcompX_{t}^{2}\leq2$, $\Delta_{1} \asymp \sqrt{\log d}/\sqrt{\oversamp \cdot d}$, $\oversamp \geq C\log d$, $r_{t}^{2} \geq 50 \rho$, $\rho \asymp \oversamp$ and $\Delta_2 \asymp \log^{2}(d)/(\oversamp \cdot \sqrt{d})$. Putting the pieces together yields that
\[
	\parcompX_{t+1}^{\mathsf{det}} \geq \frac{1}{2\sqrt{\pi}} \cdot \frac{\parcompZ_{t+1}}{\perpcompZ_{t+1}^{2}} \geq \frac{1}{2\sqrt{\pi}} \cdot \frac{ \frac{1}{4\sqrt{\pi}} \cdot \frac{\parcompX_{t}}{\perpcompX_{t}^{2}} }{ 2\rho^{-1} \cdot \perpcompX_{t}^{-2} } \geq \frac{\rho}{16\pi} \cdot \parcompX_{t}. 
\]
Next, we next derive the upper bound $(\perpcompX_{t+1}^{\mathsf{det}})^{2}$. By definition, $(\perpcompX_{t+1}^{\mathsf{det}})^{2} = \perpmapbit(\parcompZ_{t+1},\perpcompZ_{t+1})$. Consequently, we obtain that
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} &\leq \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompZ_{t+1}^{2}+\perpcompZ_{t+1}^{2}} + \frac{20(\parcompX_{t+1}^{\mathsf{det}})^{2}}{C(\oversamp)} \overset{\1}{\leq} 
	\frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompZ_{t+1}^{2}+\perpcompZ_{t+1}^{2}} + \frac{20}{C(\oversamp)} \cdot \frac{4}{\pi^{2}} \cdot \frac{1}{\parcompZ_{t+1}^{2}+\perpcompZ_{t+1}^{2}}\cdot \frac{\parcompZ_{t+1}^{2}}{\perpcompZ_{t+1}^{2}} \\&\leq \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompZ_{t+1}^{2}+\perpcompZ_{t+1}^{2}} \cdot (1+9\widetilde{r}_{t+1}^{-2}) \leq \rho^{-1} \cdot \perpcompZ_{t+1}^{-2}\cdot (1+9\widetilde{r}_{t+1}^{-2}),
\end{align*}
where in step $\1$ we plug in inequality~\eqref{ineq2.5-lemma1-init-nonlinear-proof}. Using inequalities~\eqref{ineq1-lemma1-init-nonlinear-proof} and~\eqref{ineq2-lemma1-init-nonlinear-proof} yields 
\[
	\perpcompZ_{t+1}^{2} \geq \rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-1} \cdot (1-18r_{t}^{-2}) - C_{1}\Delta_{2}.
\]
Putting the two pieces together yields that
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} &\leq \frac{1}{\rho}\cdot \frac{ (1+9\widetilde{r}_{t+1}^{-2})}{\rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-1} \cdot (1-18r_{t}^{-2}) - C_{1}\Delta_{2}} \\&=
	\frac{\perpcompX_{t}^{2}\cdot (1+r_{t}^{-2})\cdot (1-18r_{t}^{-2})^{-1} \cdot (1+9\widetilde{r}_{t+1}^{-2}) }{ 1-C_{1}\cdot \rho \cdot \perpcompX_{t}^{2}\cdot (1+r_{t}^{-2})\cdot (1-18r_{t}^{-2})^{-1} \cdot \Delta_{2}} \\& \overset{\1}{\leq}
	\frac{\perpcompX_{t}^{2}\cdot (1+r_{t}^{-2})\cdot (1-18r_{t}^{-2})^{-1} \cdot (1+9\widetilde{r}_{t+1}^{-2}) }{ 1-10C_{1}\cdot \rho \cdot \Delta_{2}} \\&\overset{\2}{\leq}
	\perpcompX_{t}^{2}\cdot (1+r_{t}^{-2})\cdot (1-18r_{t}^{-2})^{-1} \cdot (1+9\widetilde{r}_{t+1}^{-2}) \cdot (1+20C_{1}\rho\Delta_{2}),
\end{align*}
where in step $\1$ we use $\perpcompX_{t}^{2}\cdot (1+r_{t}^{-2})\cdot (1-18r_{t}^{-2})^{-1} \leq 10$ since $\perpcompX_{t}^{2} \leq 2$ and $r_{t}^{2} \geq 50\rho$, and in step $\2$ we use $(1-a)^{-1} \leq 1+2a$ for $0 \leq a\leq 0.5$ and set $a = 10C_{1}\cdot \rho \cdot \Delta_{2} \asymp \log^{2}(d)/\sqrt{d}$. Continuing, using $\widetilde{r}_{t+1} \geq \frac{\pi}{6} \cdot \rho^{-1/2} \cdot r_{t}$ yields that
\begin{align*}
	(1+r_{t}^{-2})\cdot (1-18r_{t}^{-2})^{-1} \cdot (1+9\widetilde{r}_{t+1}^{-2}) \leq (1+r_{t}^{-2})\cdot(1+36r_{t}^{-2})\cdot(1+36\rho r_{t}^{-2}) \leq 1+40\rho r_{t}^{-2}.
\end{align*}
Putting the pieces together yields that
\[
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} \leq \perpcompX_{t}^{2} \cdot (1+40\rho r_{t}^{-2}) \cdot (1+20C_{1}\rho\Delta_{2}) \leq \perpcompX_{t}^{2} + 40\rho\parcompX_{t}^{2} + \frac{C_{1}'\log^{2}(d)}{\sqrt{d}}.
\]
Next we derive the lower bound of $(\perpcompX_{t+1}^{\mathsf{det}})^{2}$. We obtain that
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} &\geq  \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompZ_{t+1}^{2}+\perpcompZ_{t+1}^{2}} - \frac{4}{\pi} \cdot \frac{\parcompX_{t+1}^{\mathsf{det}}}{C(\oversamp)\sqrt{\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2}}} \cdot 20 \\&\overset{\1}{\geq} \frac{1+\sigma^{2}}{C(\oversamp)} \cdot \frac{1}{\parcompZ_{t+1}^{2}+\perpcompZ_{t+1}^{2}} - \frac{160}{\pi^{2}C(\oversamp)} \cdot \frac{1}{\parcompZ_{t+1}^{2} + \perpcompZ_{t+1}^{2}} \cdot \frac{\parcompZ_{t+1}^{2}}{\perpcompZ_{t+1}^{2}} \\&\geq \rho^{-1} \cdot \perpcompZ_{t+1}^{-2} \cdot (1+\widetilde{r}_{t+1}^{-2})^{-1} \cdot (1-18\widetilde{r}_{t+1}^{-2}),
\end{align*}
where in step $\1$ we use inequality~\eqref{ineq2.5-lemma1-init-nonlinear-proof}. Using inequalities~\eqref{ineq1-lemma1-init-nonlinear-proof} and~\eqref{ineq2-lemma1-init-nonlinear-proof} yields 
\[
	\perpcompZ_{t+1}^{2} \leq \rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-1} \cdot (1+9r_{t}^{-2}) + C_{1}\Delta_{2} \leq \rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+9r_{t}^{-2}) + C_{1}\Delta_{2} .
\]
Putting the two pieces together yields that
\begin{align*}
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} &\geq \frac{1}{\rho} \cdot \frac{(1+\widetilde{r}_{t+1}^{-2})^{-1} \cdot (1-18\widetilde{r}_{t+1}^{-2})}{\rho^{-1} \cdot \perpcompX_{t}^{-2}  \cdot (1+9r_{t}^{-2}) + C_{1}\Delta_{2}} 
	\\&= \frac{\perpcompX_{t}^{2}\cdot(1+9r_{t}^{-2})^{-1}\cdot(1+\widetilde{r}_{t+1}^{-2})^{-1} \cdot (1-18\widetilde{r}_{t+1}^{-2})}{1 + C_{1}\perpcompX_{t}^{2}(1+9r_{t}^{-2})^{-1}\rho\Delta_{2}} \\& \overset{\1}{\geq} \frac{\perpcompX_{t}^{2}\cdot(1+9r_{t}^{-2})^{-1}\cdot(1+\widetilde{r}_{t+1}^{-2})^{-1} \cdot (1-18\widetilde{r}_{t+1}^{-2})}{1 + 10C_{1}\rho\Delta_{2}} \\ &\geq
	\perpcompX_{t}^{2}\cdot(1+9r_{t}^{-2})^{-1}\cdot(1+\widetilde{r}_{t+1}^{-2})^{-1} \cdot (1-18\widetilde{r}_{t+1}^{-2}) \cdot (1 - 10C_{1}\rho\Delta_{2}),
\end{align*}
where in step $\1$ we use $\perpcompX_{t}^{2}(1+9r_{t}^{-2})^{-1} \leq 10$ since $\perpcompX_{t}^{2} \leq 2$ and $r_{t}^{2}\geq 20\rho$, and in last step we use $(1+a)^{-1} \geq 1-a$ by setting $a = 10C_{1}\rho\Delta_{2}$. Continuing, using $\widetilde{r}_{t+1} \geq \frac{\pi}{6} \cdot \rho^{-1/2} \cdot r_{t}$, we obtain that
\[
	(1+9r_{t}^{-2})^{-1}\cdot(1+\widetilde{r}_{t+1}^{-2})^{-1} \cdot (1-18\widetilde{r}_{t+1}^{-2}) \geq (1-9r_{t}^{-2})\cdot(1-\widetilde{r}_{t+1}^{-2}) \cdot (1-18\widetilde{r}_{t+1}^{-2}) \geq 1-100\rho\cdot r_{t}^{-2}.
\]
Putting the pieces together yields that
\[
	(\perpcompX_{t+1}^{\mathsf{det}})^{2} \geq \perpcompX_{t}^{2}\cdot (1-100\rho\cdot r_{t}^{-2})\cdot (1 - 10C_{1}\rho\Delta_{2}) \geq \perpcompX_{t}^{2} - 100\rho \cdot \parcompX_{t}^{2} - \frac{C_{1}'\log^{2}(d)}{\sqrt{d}}.
\]
To this end, we have obtained the following upper and lower bound of $\parcompX_{t+1}^{\mathsf{det}}$ and $(\perpcompX_{t+1}^{\mathsf{det}})^{2}$:
\begin{align*}
	\frac{\rho}{16\pi} \cdot \parcompX_{t} &\leq \parcompX_{t+1}^{\mathsf{det}} \leq 2\rho \cdot \parcompX_{t} \quad \text{and}\\
	\perpcompX_{t}^{2} - 100\rho \cdot \parcompX_{t}^{2} - \frac{C_{1}'\log^{2}(d)}{\sqrt{d}} &\leq (\perpcompX_{t+1}^{\mathsf{det}})^{2} \leq \perpcompX_{t}^{2} + 40\rho\parcompX_{t}^{2} + \frac{C_{1}'\log^{2}(d)}{\sqrt{d}}.
\end{align*}
Note that 
\[
	\parcompZ_{t+1}^{2}+\perpcompZ_{t+1}^{2} \geq \perpcompZ_{t+1}^{2} \geq \rho^{-1} \cdot \perpcompX_{t}^{-2} \cdot (1+r_{t}^{-2})^{-1} \cdot (1-18r_{t}^{-2}) - C_{1}\Delta_{2} \geq \rho^{-1}/4 \gtrsim \oversamp^{-1},
\]
where the last step follows since $\rho \asymp \oversamp$. Consequently, on event $\mathcal{B}_{t+1}$, we obtain that
\begin{align*}
	\left| \parcompX_{t+1} - \parcompX_{t+1}^{\mathsf{det}}\right| \lesssim \sqrt{\frac{\log d}{d}} \quad \text{and} \quad \left| \perpcompX_{t+1}^{2} - (\perpcompX_{t+1}^{\mathsf{det}})^{2} \right| \lesssim \frac{\log^{2}(d)}{\sqrt{d}}.
\end{align*}
Putting the pieces together yields that
\begin{align*}
	\parcompZ_{t+1} &\leq \parcompZ_{t+1}^{\mathsf{det}} + \frac{C_{1}'\log d}{\sqrt{d}} \leq 2\rho \cdot \parcompX_{t} + \frac{C_{1}'\log d}{\sqrt{d}} \leq 3\rho \cdot \parcompX_{t}, \\
	\parcompZ_{t+1} &\geq \parcompZ_{t+1}^{\mathsf{det}} - \frac{C_{1}'\log d}{\sqrt{d}} \geq \frac{\rho}{16\pi}  \cdot \parcompX_{t} - \frac{C_{1}'\log d}{\sqrt{d}} \geq \frac{\rho}{20\pi} \cdot \parcompX_{t},\\
	\perpcompZ_{t+1}^{2} &\leq (\perpcompZ_{t+1}^{\mathsf{det}})^{2} + \frac{C_{1}'\log^{2}(d)}{\sqrt{d}} \leq \perpcompX_{t}^{2} + 40\rho\parcompX_{t}^{2} + \frac{C_{1}''\log^{2}(d)}{\sqrt{d}}\quad \text{and}\\
	\perpcompZ_{t+1}^{2} &\geq (\perpcompZ_{t+1}^{\mathsf{det}})^{2} - \frac{C_{1}'\log^{2}(d)}{\sqrt{d}} \geq \perpcompX_{t}^{2} - 100\rho \parcompX_{t}^{2}-C_{1}''\frac{\log^{2}(d)}{\sqrt{d}}.
\end{align*}
















































==> commands.tex <==
%auto-ignore
%!TEX root = main-paper-template.tex

% The command above makes the PDF compilable from this file if you're using SublimeText

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Some basic packages

\usepackage{comment}
\usepackage{epsf}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{bbm}
\usepackage{color}
\usepackage{nicefrac}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amsmath, bm}
\usepackage{amssymb}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{float}
\usepackage[ruled, vlined, lined, commentsnumbered]{algorithm2e}

\RequirePackage[colorlinks,citecolor={blue!60!black},urlcolor={blue!70!black},linkcolor={red!60!black},breaklinks,hypertexnames=false]{hyperref} %Adds links to references (without boxes)


% Alternative minipage environment, renders better in terms of spacing

\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}
  
\newenvironment{algbox}[0]{\vskip 0.2in
\noindent 
\begin{fminipage}{6.3in}
}{
\end{fminipage}
\vskip 0.2in
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MACROS BELOW

%%%%%%%

% {Theorem, Proposition, Lemma, Corollary} numbered sequentially
% throughout the paper, not by section number and not combined


\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem{claim}{Claim}

%%%%%%%%%%%
%References (natbib): Use \citet and \citep to take full advantage

\usepackage{natbib}
\setcitestyle{round}

%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Widebar command
\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
 \settowidth{\widebarargwidth}{\ensuremath{#1}}%
 \settoheight{\widebarargheight}{\ensuremath{#1}}%
 \settodepth{\widebarargdepth}{\ensuremath{#1}}%
 \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
 \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
 \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
   \hspace{0.3\widebarargdepth}%
   \addtolength{\widebarargheight}{0.3ex}%
   \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
 {#1}}



%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
\makeatletter
\long\def\@makecaption#1#2{
       \vskip 0.8ex
       \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
       \parindent 1.5em 
       \dimen0=\hsize
       \advance\dimen0 by -3em
       \ifdim \wd\@tempboxa >\dimen0
               \hbox to \hsize{
                       \parindent 0em
                       \hfil 
                       \parbox{\dimen0}{\def\baselinestretch{0.96}\small
                               {\bf #1.} #2
                               %%\unhbox\@tempboxa
                               } 
                       \hfil}
       \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
       \fi
       }
\makeatother



%% COMMENTING commands: insert more for more than two collaborators
\long\def\comment#1{}

\newcommand{\revision}[1]{\textcolor{black}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\apcomment}[1]{{\bf{{\blue{{AP --- #1}}}}}}

%\newcommand{\olive}[1]{\textcolor{olive}{#1}}
%\newcommand{\kaccomment}[1]{{\bf{{\olive{{KAC --- #1}}}}}
  
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\kaccomment}[1]{{\bf{{\red{{KAC --- #1}}}}}}



% Some vector/matrix norms. Convention is that we use triple lines for matrix 
% norms and double lines for vector norms.
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\| #1\|_{#2}}

% Some useful and common operators
% Independence symbol
\newcommand\indpt{\protect\mathpalette{\protect\independenT}{\perp}} 
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\defn}{\coloneqq} %This is a properly aligned definition symbol
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator{\modd}{mod}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator{\floor}{floor}
% \DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\dist}{\rho}
\DeclareMathOperator{\trace}{\mathsf{tr}}
\DeclareMathOperator{\op}{\mathsf{op}}
\DeclareMathOperator{\sign}{\mathsf{sgn}}



% Specific norms
\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{nuc}}}}}
\newcommand{\fronorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{F}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{op}}}}}
\newcommand{\eucnorm}[1]{\left\|#1 \right\|}
\newcommand{\linfnorm}[1]{\left\|#1 \right\|_\infty}

% Bracket notation to make life easier when writing long expressions
\newcommand{\paren}[1]{\left\{ #1 \right\} }
% Inner product
\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}

% The macros below are useful if you see these quantities changing over the course of writing
\newcommand{\numdim}{\ensuremath{d}}
\newcommand{\numobs}{\ensuremath{n}}

% Distances between distributions
\newcommand{\kull}[2]{\ensuremath{D_{\mathsf{KL}}(#1\; \| \; #2)}}
\newcommand{\KL}{\ensuremath{D_{\mathsf{KL}}}}
\newcommand{\TV}{\ensuremath{d_{\mathsf{TV}}}}
\newcommand{\Hel}{\ensuremath{d_{\mathsf{hel}}}}

% Probability
\newcommand{\EE}{\ensuremath{{\mathbb{E}}}}
\newcommand{\real}{\ensuremath{{\mathbb{R}}}}
\newcommand{\Prob}{\ensuremath{{\mathbb{P}}}}
\newcommand{\ind}[1]{\ensuremath{{\mathbb{I}\left\{ #1 \right\}}}}

%Numbering (use with \overset to label steps)
\newcommand{\1}{\ensuremath{{\sf (i)}}}
\newcommand{\2}{\ensuremath{{\sf (ii)}}}
\newcommand{\3}{\ensuremath{{\sf (iii)}}}
\newcommand{\4}{\ensuremath{{\sf (iv)}}}
\newcommand{\5}{\ensuremath{{\sf (v)}}}
\newcommand{\6}{\ensuremath{{\sf (vi)}}}
\newcommand{\7}{\ensuremath{{\sf (vii)}}}

%Eigenvector / eigenvalue related notation
\newcommand{\eig}[1]{\ensuremath{\lambda_{#1}}}
\newcommand{\eigmax}{\ensuremath{\eig{\max}}}
\newcommand{\eigmin}{\ensuremath{\eig{\min}}}


% Distributions
\newcommand{\NORMAL}{\ensuremath{\mathsf{N}}}
\newcommand{\BER}{\ensuremath{\mbox{\sf Ber}}}
\newcommand{\BIN}{\ensuremath{\mbox{\sf Bin}}}
\newcommand{\Hyp}{\ensuremath{\mbox{\sf Hyp}}}

% Script letters
\newcommand{\Aspace}{\ensuremath{\mathcal{A}}}
\newcommand{\Xspace}{\ensuremath{\mathcal{X}}}
\newcommand{\Yspace}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zspace}{\ensuremath{\mathcal{Z}}}
\newcommand{\Fspace}{\ensuremath{\mathcal{F}}}

% Population and sample loss functions
\newcommand{\loss}{\ensuremath{\mathcal{L}}}
\newcommand{\lossn}[1]{\ensuremath{\mathcal{L}^n \left( #1 \right)}}

% True parameter
\newcommand{\thetastar}{\ensuremath{\theta^*}}
% Estimates
\newcommand{\thetahat}{\ensuremath{\widehat{\theta}}}
\newcommand{\thetabar}{\ensuremath{\overline{\theta}}}
\newcommand{\thetatil}{\ensuremath{\widetilde{\theta}}}

% Order notation
\newcommand{\order}{\ensuremath{\mathcal{O}}}
\newcommand{\ordertil}{\ensuremath{\widetilde{\order}}}
\newcommand{\Omegatil}{\ensuremath{\widetilde{\Omega}}}

% Macros for blind deconvolution
\newcommand{\parcompZ}{\widetilde{\alpha}}
\newcommand{\parcompdetZ}{\widetilde{\alpha}^{\mathsf{det}}}
\newcommand{\perpcompZ}{\widetilde{\beta}}
\newcommand{\perpcompdetZ}{\widetilde{\beta}^{\mathsf{det}}}
\newcommand{\parcompX}{\alpha}
\newcommand{\parcompdetX}{\alpha^{\mathsf{det}}}
\newcommand{\parcompdetbarX}{\widebar{\alpha}^{\mathsf{det}}}
\newcommand{\perpcompX}{\beta}
\newcommand{\perpcompbarX}{\widebar{\beta}}
\newcommand{\perpcompdetX}{\beta^{\mathsf{det}}}
\newcommand{\oversamp}{\Lambda}
\newcommand{\parsigma}{1+\sigma}
\newcommand{\perpsigma}{1+\sigma^{2}}
\newcommand{\pardevn}{\sqrt{\frac{\log(n)}{n}}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bSig}{\boldsymbol{\Sigma}}
\newcommand{\beps}{\boldsymbol{\epsilon}}
\newcommand{\perpX}{\beta}
\newcommand{\parX}{\alpha}
\newcommand{\perpZ}{\iota}
\newcommand{\parZ}{\gamma}
\newcommand{\coefX}{\mu}
\newcommand{\bcoefX}{\boldsymbol{\mu}}
\newcommand{\coefZ}{\nu}
\newcommand{\bcoefZ}{\boldsymbol{\nu}}
\newcommand{\epsilondn}{\epsilon_{d,n}}
\newcommand{\Cdm}{C_{d,m}}
\newcommand{\K}{100}
\newcommand{\ratiomapid}{h_{\mathsf{id}}}
\newcommand{\ratiomapbit}{h_{\mathsf{sgn}}}
\newcommand{\ratiomappsi}{h_{\psi}}
\newcommand{\parmapid}{F_{\mathsf{id}}}
\newcommand{\parmapbit}{F_{\mathsf{sgn}}}
\newcommand{\perpmapid}{G_{\mathsf{id}}}
\newcommand{\perpmapbit}{G_{\mathsf{sgn}}}
\newcommand{\statemapid}{\mathcal{S}_{\mathsf{id}}}
\newcommand{\statemapbit}{\mathcal{S}_{\mathsf{sgn}}}
\newcommand{\perplogd}{\log^{8}(d)}
\newcommand{\perplogn}{\log^{8}(n)}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}

% constants for convergence proof
\newcommand{\Alam}{A(\Lambda)}
\newcommand{\Blam}{B(\Lambda)}


% Leave one out notation
\newcommand{\Xcol}[1]{\bX^{(#1)}}
\newcommand{\Xloco}[1]{\bX_{\backslash #1}}
\newcommand{\coefXloco}[1]{\widehat{\coefX}^{(\backslash#1)}}
\newcommand{\bSk}[1]{\bS_{\backslash #1}}

% Notation for deviation lemmas
\newcommand{\numexpect}{XXX}
%\newcommand{\denomexpect}{(\parcompZ_{t+1}^2 + \perpcompZ_{t+1}^2) \EE\Bigl\{ \frac{G^2}{1 + \tau G^2}\Bigr\}}
\newcommand{\denomexpect}{YYY}
\newcommand{\intermediateperp}{ZZZ}
\newcommand{\fdown}{f^{\downarrow}}
\newcommand{\fup}{f^{\uparrow}}
\newcommand{\bmuG}{\widebar{\boldsymbol{\mu}}}
